On Compositions of Transformations in Contrastive Self-Supervised Learning

In the image domain, excellent representations can be learned by inducing invariance to content-preserving transformations via noise contrastive learning. In this paper, we generalize contrastive learning to a wider set of transformations, and their compositions, for which either invariance or distinctiveness is sought. We show that it is not immediately obvious how existing methods such as SimCLR can be extended to do so. Instead, we introduce a number of formal requirements that all contrastive formulations must satisfy, and propose a practical construction which satisfies these requirements. In order to maximise the reach of this analysis, we express all components of noise contrastive formulations as the choice of certain generalized transformations of the data (GDTs), including data sampling. We then consider videos as an example of data in which a large variety of transformations are applicable, accounting for the extra modalities -- for which we analyze audio and text -- and the dimension of time. We find that being invariant to certain transformations and distinctive to others is critical to learning effective video representations, improving the state-of-the-art for multiple benchmarks by a large margin, and even surpassing supervised pretraining.

==> 7_broader_impact.tex <==
\clearpage
\section*{Broader impact}

We see the research presented in this work to have a potential broader impact in three main areas over the short and long term.
\paragraph{Reduce bias on less curated data}
The promise of self-supervised methods is to learn ever more robust and general visual representation models without manual annotations. 
Indeed, training on ever larger datasets with ever better methods has continued to increase performance on downstream tasks and we have presented similar findings in this paper.
This shows the potential and benefit of self-supervised learning compared to supervised or weakly-supervised learning, and also has the added potential to reduce the risk of incorporating biases present in the training data.
As biases start in the data collection process, using less curated data and significantly more of it might be useful in having less biased models as these will be trained with more diversity. 
We should also note that biases present in these models might disappear once the network is fine-tuned on a target task (on which biases should, also be avoided or known).
However, it is still crucial to understand this aspect in detail when it comes to deployment and we believe that research should be encouraged probing self-supervised models with regards to their underlying data distributions, in a similar way to \citep{jahanian2020On,voynov2020unsupervised} for images, and as has been done more rigorously in the NLP domain for some time, e.g. \cite{bolukbasi2016man,qian2019reducing,park2018reducing,zhao2019gender}.

\paragraph{Applications in medical imaging.} Using pretrained visual feature representations, such as those obtained by training on ImageNet LSVRC-12 and finetuning these on specific medical imaging tasks has been very successful~\cite{xie2018pre,schlegl2014unsupervised,litjens2017survey}.
Models obtained in such a manner outperform those trained from scratch and vice versa require less expert time for human annotation~\cite{overviewmedical}. 
Thus far, these mostly 2D CNN models were used for transfer learning, but there are applications were the temporal dimension is key, such as heart imaging with ultra sound~\cite{huang2017temporal}. 
It is likely that self-supervised video representation models, such as the one presented in this paper will be useful for these applications, with the implications of a) increasing the accuracy of the physician's diagnosis,  b) reducing the time-cost of diagnosis, and c) facilitating remote diagnostics in places with not enough trained staff.
However, a risk with algorithms in unsupervised learning is that users may put too much blind trust on the results of the algorithm (in our case a network initialization). 
In practice, there are no guarantees that the algorithm would find a solution fit for any particular downstream application.
This needs to be carefully validated a posteriory.

\paragraph{Harmful content detection.}
The number of uploaded videos to online platforms only keeps increasing, yet automatically detecting harmful content is still in its infancy. 
As content is now increasingly moving towards videos, self-supervisedly trained video models may be especially useful for transfer learning. 
The benefits are a) the models can be more accurately detect harmful content, leading to both higher recall and precision, and b) training good classifiers requires less annotations from humans, which are in this case not just expensive but psychologically harmful.

Furthermore we encourage ways of getting the research community to participate in these developments in ways that do not require the release and distribution of such material. 
One recent such initiative is the hateful memes competition\footnote{\url{https://www.drivendata.org/competitions/64/hateful-memes/}}, which although based on image understanding captures the difficulties of multi-modal learning and the nuances of understanding intention.


==> GDT (ICCV 2021)/1_introduction.tex <==
\section{Introduction}

Works such as MoCo~\citep{he2019momentum}, SimCLR~\citep{Chen2020ASF}, SwAV~\citep{caron2020unsupervised} and BYOL~\citep{grill2020bootstrap} have shown that it is possible to pre-train state-of-the-art image representations without the use of any manually-provided labels.
Furthermore, many of these approaches use variants of noise contrastive learning~\citep{gutmann2010noise, Hadsell2006DimensionalityRB}.
Their idea is to learn a representation that is \emph{invariant} to transformations that leave the meaning of an image unchanged (e.g.~geometric distortion or cropping) and \emph{distinctive} to changes that are likely to alter its meaning (e.g.~replacing an image with another chosen at random).

\input{figs/splash_update}

These prior works have also shown that the choice of transformations is of primary importance for performance~\citep{Chen2020ASF, caron2020unsupervised}.
This is not just a matter of selecting a certain type of transformation, but also to specify how different transformations should be composed, and how these compositions should be sampled to from batches for training the model.
So far, these choices have been mostly driven by intuition, with little formal understanding of why certain choices may be preferable, and how these choices can be generalized.

In this work, we answer some of these questions via a formal analysis of \emph{composable transformations in contrastive learning}.
Our analysis shows how invariance and distinctiveness to individual transformations can be meaningfully incorporated in the same learning formulation.
It also provides some principles to guide the construction of the training batches.
We interpret existing sampling schemes, such as the one in SimCLR, as special cases with certain potential advantages and disadvantages.
We do so by showing how these constructions can be extended systematically to any composition of invariant and distinctive transformations.

Furthermore, we demonstrate the utility of our analysis by exploring contrastive methods for learning representations of video data.
Compared to images, videos contain a time dimension and multiple modalities, which have been shown to provide effective learning cues; for instance
% \citep{owens2016ambient,Arandjelovic17} leverages multiple modalities, and \citep{avts,Chung16a,owens2018audio} the time dimension.
\citep{owens2016ambient} leverages multiple modalities, and \citep{avts,Chung16a} the time dimension.
We show how these effects can be incorporated in a uniform manner in contrastive learning by considering a suitable class of \emph{generalized data 
transformations} (GDTs).
GDTs capture standard augmentations, as well as temporal transformations, modality slicing and data sampling.
The advantages of using GDTs is that they allow us to base the entire design of the learning formulation (e.g., how to write a coherent learning objective and how to sample batches) on a small number of design principles that our analysis has identified.

% Then, based on our g

% Based on the analysis above, we show that these ad-hoc approaches can be reduced to a standard contrastive learning formulation that is a direct generalization of SimCLR.
% In order to do so, we reduce all effects, including data sampling, modality slicing, and time manipulation, to \emph{generalized data 
% transformations} (GDTs).

% An analysis of such works shows that a dominant factor for performance is the choice of the transformations applied to the data.
% So far, authors have explored standard ad-hoc image augmentations such as random scale changes, crops, or contrast changes.
% Videos further allow to leverage the time dimension and multiple modalities.
% For example, {}\cite{owens2016ambient,Arandjelovic17} learn representations by matching visual and audio streams, as a proxy for objects that have a coherent appearance and sound.
% Their formulation is similar to noise contrastive ones, but does not quite follow the pattern of expressing the loss in terms of invariance to data transformations.
% Others~\citep{avts,Chung16a,owens2018audio} depart further from standard contrastive schemes by learning representations that can tell whether visual and audio streams are in sync or not; the difference here is that the representation is encouraged to be distinctive rather than invariant to a time shift.

% An analysis of such works shows that a dominant factor for performance is the choice of the transformations applied to the data.
% So far, authors have explored standard ad-hoc image augmentations such as random scale changes, crops, or contrast changes.
% Videos further allow to leverage the time dimension and multiple modalities.
% For example, {}\cite{owens2016ambient,Arandjelovic17} learn representations by matching visual and audio streams, as a proxy for objects that have a coherent appearance and sound.
% Their formulation is similar to noise contrastive ones, but does not quite follow the pattern of expressing the loss in terms of invariance to data transformations.
% Others~\citep{avts,Chung16a,owens2018audio} depart further from standard contrastive schemes by learning representations that can tell whether visual and audio streams are in sync or not; the difference here is that the representation is encouraged to be distinctive rather than invariant to a time shift.

% Overall, it seems that finding an optimal noise contrastive formulation for videos will require combining several transformations while accounting for time and multiple modalities, and understanding how invariance and distinctiveness should relate to the transformations.
% However, the ad-hoc nature of these choices in previous contributions make a systematic exploration of this space rather difficult.

% In this paper, we propose a solution to this problem by introducing the Generalized Data Transformations (GDT;~\cref{fig:splash}) framework.
% GDTs reduce most previous methods, contrastive or not, to a noise contrastive formulation that is expressed in terms of data transformations only, making it simpler to systematically explore the space of possible combinations.
% This is true in particular for multi-modal data, where the space of possible contrastive pairs and transformations is not just combinatorially larger, but also vastly under-explored compared to the image domain.
%separating different modalities can also be seen as a transformation of an input video.
% \todo{Why do we apply GDT to multi-modal learning?}
% To facilitate a thorough analysis of data transformation based pretraining, the formalism shows \emph{which} combinations of different transformations are valid and how to enumerate them.
% It also clarifies how invariance and distinctiveness to different effects can be incorporated in a simple noise contrastive loss based formulation and when doing so leads to a valid learning objective.
% These two aspects allows the search space of potentially optimal transformations to be significantly constrained, making it amenable to grid-search or more sophisticated methods such as Bayesian optimisation.

With this, we make some notable findings for contrastive video representation learning.
% First, we find that using our framework, most previous pretext representation learning tasks can be formulated in a noise-contrastive manner, unifying previously distinct domains.
% Second, 
First, we show that using this wider class of transformations greatly exceeds the performance that can be obtained by a vanilla applications of image-centric methods such as SimCLR to video data.
By leveraging time and multiple modalities, we obtain large performance gains, almost \emph{doubling} the performance.
% that by investigating factors to be variant to, it is possible to observe large gains in numerous downstream tasks, far outperforming a simple SimCLR extension to video data.
Second, we show that just learning representations that are invariant to more and more transformations is \emph{not} optimal, at least when it comes to video data; instead, combining invariance to certain factors with distinctiveness to others performs better.
To the best of our knowledge, this is the first time such an effect has been demonstrated in contrastive learning.

% By using GDTs, we make several findings.
% First, we find that using our framework, most previous pretext representation learning tasks can be formulated in a noise-contrastive manner, unifying previously distinct domains.
% Second, we show that just learning representations that are invariant to more and more transformations is \emph{not} optimal, at least when it comes to video data; instead, balancing invariance to certain factors with distinctiveness to others performs best.
% Third, we find that by investigating factors to be variant to, it is possible to observe large gains in numerous downstream tasks, far outperforming a simple SimCLR extension to video data.
%what to be variant to can lead to large gains in numerous downstream performances. % , for both visual and audio tasks.

We also set the new state of the art in audio-visual representation learning, with both  small and large video pretraining datasets on a variety of downstream tasks.
In particular, we achieve $94.1\%$ and $67.4\%$ on the standardized UCF-101~\citep{UCF101} and HMDB-51~\citep{kuehne2011hmdb} action recognition benchmarks, when pretrained on HowTo100M~\citep{miech2019howto100m}, and $95.2\%$ and $72.8\%$ respectively when pretrained on IG65M~\citep{Ghadiyaram2019}.

% Compared to images, videos allow for pretraining methods exploiting time- and multi-modality based transformations~\citep{ShuffleNet,avts,arandjelovic17look}.
% An example is cross-modal supervision~\citep{owens2016ambient, arandjelovic17look}, where one learns to match the visual and audio components extracted from the same video.
% The latter is an excellent proxy for abstraction as it encourages the representation to learn objects with a characteristic appearance and sound.
% Others~\cite{avts,Chung16a,owens2018audio} have proposed to look at the temporal correlation between the audio and visual streams, learning to tell whether they are in sync or not.
% Notably, these methods are usually \emph{not} formulated in a noise contrastive manner.
% Overall, we can paint a complex picture, with different methods learning from a different combination of cues and learning schemes.

% While the best-performing methods differ in several ways
% By comparing the best-performing noise contrastive methods available, it seems that a dominant factor for performance is the choice of which transformations are used during learning.
% In computer vision, most formulations seek invariance to \emph{photo-geometric} data transformations, in the form of random 2D image distortions such as scale changes, crops, or contrast changes.
% While these only approximate real nuisance factors such as a viewpoint change, object deformations or intra-class variations, the key advantage is that they can be trivially implemented.
% For distinctiveness, these formulations seek to discriminate different image samples, assuming that the probability that two random images have the same `meaning' is very low.

% Compared to images, videos allow for pretraining methods exploiting time- and multi-modality based transformations~\citep{ShuffleNet,avts,arandjelovic17look}.
% An example is cross-modal supervision~\citep{owens2016ambient, arandjelovic17look}, where one learns to match the visual and audio components extracted from the same video.
% The latter is an excellent proxy for abstraction as it encourages the representation to learn objects with a characteristic appearance and sound.
% Others~\cite{avts,Chung16a,owens2018audio} have proposed to look at the temporal correlation between the audio and visual streams, learning to tell whether they are in sync or not.
% Notably, these methods are usually \emph{not} formulated in a noise contrastive manner.
% Overall, we can paint a complex picture, with different methods learning from a different combination of cues and learning schemes.

% In this paper, we introduce the method of \emph{generalized data transformation} (GDT) which clarifies, unifies and improves these different methodological approaches.
% A GDT absorbs in one object effects such as data sampling, choice of a modality, time shift, and photo-geometric augmentation.
% Given this, one can reduce most existing self-supervised learning schemes to (1) choosing how GDTs are sampled in a batch and (2) which GDT pairs are contrasted positively, negatively, or are ignored.
% This concept is exemplified in~\Cref{fig:splash} in a typical instantiation for audio-visual learning.
% A set of GDTs are constructed hierarchically, starting from sampling videos from a dataset down to splitting modalities and applying augmentations (A).
% Then, different pairs of transformations are contrasted with a positive (attractive) or negative (repulsive) effect (B).
% This learns corresponding invariances or distinctiveness in the representation (C).

% The importance of our reduction is that it extends to cues that have been so far given only in a non-contrastive manner, and allows for novel combinations previously unexplored, such as distinctiveness to time shift and time reversal across modalities, yielding state-of-the-art feature representations.
% We also derive formal conditions to tell which combinations are valid.
% Furthermore, most contrastive formulations are concerned with the choice of invariances, fixing distinctiveness to the discrimination of different samples.
% The GDT framework shows that both design choices can be changed, leading to better results.

% In short, a key benefit of GDTs is that they allow to systematically explore  and test novel \emph{hypotheses} on which invariances and distinctivenesses are most beneficial for pretraining data representations.
% Because of this added flexibility, we can \emph{improve} the performance of existing approaches.
% To demonstrate this, we apply our framework to multi-modal (video) data, as it offers a rich space of combinations to search.
% Using our framework, we explore the space of such combinations and determine which ones are optimal for downstream performance.
% With this, we are able to set the new state of the art in audio-visual representation learning, with both  small and large video pretraining datasets on a variety of visual and audio downstream tasks.
% In particular, we achieve $95.2\%$ and $72.8\%$ on the standardized UCF-101 and HMDB-51 action recognition benchmarks.

%\todo{are we happy w/ this splash?}


==> GDT (ICCV 2021)/2_related_work.tex <==
\section{Related work}

% \textbf{Early unsupervised representation learning}.
% Learning representations from unlabelled data has been an active area of computer vision research for decades.
% Early works such as auto-encoders \citep{hinton2006reducing}, deep belief networks \citep{hinton2006fast}, shift-invariant decoders \citep{ranzato2007unsupervised}, sparse coding algorithms \citep{lee2007efficient} and stacked ISAs \citep{le2011learning} learned image and video representations by reconstructing inputs.
% Recently, however, a number of works have instead focused on self-supervised learning approaches to learn representations by developing \emph{pretext tasks} to encourage networks to learn semantics from the free supervision signals available in images and videos.

\textbf{Self-supervised learning from images and videos.}
A variety of pretext tasks have been proposed to learn representations from unlabelled \textbf{images}.
Some tasks leverage the spatial context in images \citep{doersch2015unsupervised, noroozi2016unsupervised} to train CNNs, while others create pseudo classification labels via artificial rotations \citep{gidaris2018unsupervised}, or clustering features \citep{ji2018invariant,caron2018deep, caron2019unsupervised,caron2020unsupervised,asano2020self,gidaris2020learning}.
Colorization~\citep{zhang16colorful,zhang2017split},
%predicting features~\citep{oord2018representation,henaff2019data,bachman2019learning,anand2019unsupervised},
inpainting~\citep{pathak2016context}, solving jigsaw puzzles~\citep{noroozi2017representation}, as well as the contrastive methods detailed below, have been proposed for self-supervised image representation learning.
Some of the tasks that use the space dimension of images have been extended to the space-time dimensions of \textbf{videos} by crafting equivalent tasks.
These include jigsaw puzzles \citep{kim2019self}, and predicting rotations~\citep{jing2018self} or future frames~\citep{han2019video}.
Other tasks leverage the temporal dimension of videos to learn representations by predicting shuffled frames~\citep{misra2016shuffle}, the direction of time~\citep{wei2018learning}, motion \citep{motion_statistics}, temporal ordering~\citep{clip_order, lee2017unsupervised}, and playback speed \citep{benaim2020speednet, cho2020selfsupervised,fernando17self-supervised}.
These pretext-tasks can be framed as GDTs.
%and used as learning signals in our framework.

\textbf{Multi-modal learning.}
Videos, unlike images, are a rich source of a variety of modalities such as speech, audio, and optical flow, and their correlation can be used as a supervisory signal.
This idea has been present as early as 1994~\citep{NIPS1993_831}.
Only recently, however, has multi-modal learning been used to successfully learn effective representations by leveraging the natural correspondence~\citep{owens2016ambient, aytar2016soundnet, Arandjelovic17, morgado2020avid, alwassel2019self, asano2020labelling} and synchronization~\citep{Chung16a, avts, owens2018audio} between the audio and visual streams.
%Other methods use a modality distillation framework to learn video~\citep{owens2016ambient, piergiovanni2020evolving} and sound representations~\citep{aytar2016soundnet}.
%With the release of the recent HowTo100M dataset~\citep{miech19howto100m}, a large-scale instructional video dataset,
A number of recent papers have leveraged speech as a weak supervisory signal to train video representations \citep{sun2019videobert, sun2019contrastive, miech2019endtoend, li2020learning, nagrani2020} and recently \cite{alayrac2020selfsupervised}, who use speech, audio and video.
%These ASR models are, however, supervised models and thus implicitly contain more information than obtained from the training video datasets.
Other works incorporate optical flow and other modalities~\citep{zhao2019sound, piergiovanni2020evolving, Han2020SelfsupervisedCF, Han_2020} to learn representations.
In CMC~\citep{tian2019contrastive}, representations are learned with different views such as different color channels or modalities to solely induce multi-view invariance.
In contrast, our work extends this to and analyses multi-modal transformations and examines their utility as an invariant \textit{or} distinctive learning signal.

%Futhermore, multi-modal learning has been used for several applications such as lip reading~\citep{Chung16a, Chung_2017_lip_reading, afouras2018deep_lip_reading}, audio-visual source separation and localization~\citep{arandjelovic2018objects, zhao2018sound, afouras2018conversation, zhao2019sound, harwath2018jointly}, speech recognition~\citep{potamianos2003recent, afouras2018deep}, efficient inference~\citep{gao2019listen, korbar2019scsampler}, egocentric action recognition~\citep{kazakos2019epicfusion} and navigation~\citep{chen2019audiovisual}.
%Futhermore, multi-modal learning has been used for several applications such as lip reading~\citep{Chung_2017_lip_reading, afouras2018deep_lip_reading, afouras2020asr}, audio-visual source separation~\citep{gao2018learning, owens2018audio, afouras2018conversation, zhao2019sound, rouditchenko2019self}, audio-visual speech recognition~\citep{potamianos2003recent, ngiam2011multimodal, afouras2018deep, chung2018voxceleb2}, sound-source localization~\citep{arandjelovic2018objects, Senocak_2018, zhao2018sound, hu2018deep, Ephrat_2018, casanovas2010blind, gao2019co, gan2019self}, audio-visual question answering~\citep{alamri2018audio}, binaural audio generation~\citep{gao20192}, biometric matching~\citep{nagrani2018learnable, nagrani2018seeing}, multi-modal video retrieval~\citep{liu2019use},  controllable face generation~\citep{wiles2018x2face}, efficient inference~\citep{gao2019listen, korbar2019scsampler}, egocentric action recognition~\citep{kazakos2019epicfusion} and navigation~\citep{chen2019audiovisual}.
% Recent works have also found that multi-modal learning can lead to more robust representations as they can partly account for the different learning speeds of the different modalities~\citep{alwassel2019self, xiao2020audiovisual, wang2019makes}.
% In another recent, concurrent work~\citep{morgado2020avid}, hard-negative two-stage training is combined with a momentum-based contrastive loss.
%
% \paragraph{Multi-Modal transformations.}
%The space for \textbf{transformations} is much richer in video than images due to the audio and visual streams.
%Crucially, videos have high frame rates, which allows for a large combinatorial space of cropping in time \textit{and} space ~\citep{simonyan2014,alwassel2019self,avts,han2019video,arandjelovic17look,Tran18}.
%Videos also contain useful multi-modal signals such as audio-visual synchronization~\citep{Chung16a, avts, arandjelovic17look, owens2018audio}.
%yielding semantically strongly aligned transformations.
%{\color{red} These transformations, when combined with our general, hierarchical data sampling framework and the learning signal provided by a noise-contrastive loss, allow us to train state-of-the-art self-supervised video and audio encoders, beating even supervised baselines.}
%\todo{not sure if good. sounds like we only use default transformations. plus we don't compare against our method in the other paragraphs in this section.}

\textbf{Noise Contrastive Loss.}
Noise contrastive losses~\citep{Hadsell2006DimensionalityRB, gutmann2010noise} measure the similarity between sample pairs in a representational space and are at the core of several recent works on unsupervised feature learning.
They yield good performance for learning image~\citep{Wu_2018_CVPR, oord2018representation,hjelm2018learning, tian2019contrastive, he2019momentum, misra2019selfsupervised,henaff2019data,Chen2020ASF, li2020prototypical,tian2020makes} and video~\citep{sohn2016improved, miech2019endtoend, han2019video, sun2019contrastive, li2020learning, morgado2020avid, yao2021seco, anand2019unsupervised, hjelm2020representation} representations, and circumvent the need to explicitly specify what information needs to be discarded via a designed task.

We leverage the noise contrastive loss as a learning framework to encourage the network to learn desired invariance and distinctiveness to data transformations.
% The combination of data augmentations and noise-contrastive re-identification is enough to train networks effectively.
The GDT framework can be used to combine and extend many of these cues, contrastive or not, in a single noise contrastive formulation.

% Our \textit{Generalized Data Transformations} framework simplifies and contains the recent advances in self-supervised representation learning, by extending the core idea (learning desirable invariances and distinctiveness via transformations) from images~\citep{dosovitskiy2015discriminative, ji2018invariant, misra2019selfsupervised, he2019momentum, tian2019contrastive}, to multi-modal audio and visual streams and enabling our network to train with new learning signals whilst naturally incorporating cross-modal and noise-contrastive training.

% Some of the transformations used in GDT were considered in prior work by means of binary classifiers~\citep{wei2018learning,arandjelovic17look, owens2018audio} or margin-contrastive losses~\cite{avts}; here we use or approach to combine all of them in a single noise-contrastive formulation~\citep{gutmann2010noise,Wu_2018_CVPR,tian2019contrastive,Chen2020ASF,he2019momentum,misra2019selfsupervised,henaff2019data,hjelm2018learning}.


==> GDT (ICCV 2021)/3_methods.tex <==
\input{figs/splash}

\section{Method}\label{s:method-new}

We generalize contrastive methods such as CPC~\citep{oord2018representation}, PIRL~\citep{misra2019selfsupervised}, MoCo~\citep{he2019momentum}, SimCLR~\citep{Chen2020ASF}, and SwAV~\citep{caron2020unsupervised} to learn representations that can be invariant or distinctive to any number of transformations.
% We generalize them for learning data representations that are not just variant to the image index and invariant to augmentations but can instead be invariant or variant to any transformation provided. 

Given a collection $x$ of data such as images or videos, we generate training samples
$$
   x(t_1,\dots,t_M) \in \mathcal{X}.
$$
by applying a sequence of $M$ transformations \mbox{$T=(t_1,\dots,t_M)$} to the collection.
We consider typical transformations such as data augmentations (e.g., randomly cropping an image).
We also find it useful to express in the same manner other operations such as extracting a specific image or video from the collection or extracting a specific modality from a video.
We call these \emph{generalized data transformations} (GDTs).

% While this notation is unusual, it supports useful generalizations of existing contrastive formulations.
% For most the discussion, the nature of the transformations is unimportant; it only matters that they index training samples.
To provide a concrete example, in a standard contrastive learning formulation such as SimCLR, the first transformation $t_1=i\in\{1,\dots,|x|\}$ extracts an image $x_i$ from the collection $x$ and the second transformation $t_2=g$ applies to it a random augmentation, so that we can write
$
   x(t_1,t_2) = g(x_i).
$
The goal is to learn a representation $\Phi : \mathcal{X}\rightarrow \mathbb{R}^d$ that identifies the image regardless of the augmentation;
in other words, $\Phi$ should be invariant to the choice of $t_2$ and distinctive for the choice of $t_1$.

We wish to generalize this construction to richer data such as videos.
Compared to images, videos contain multiple modalities and additional dimensions, which allows to consider qualitatively different transformations such as time shift, time reversal, and modality slicing.
This generalization is however non-trivial.
First, when considering $M>2$ transformations, we have a choice of making the representation invariant or distinctive to each of them independently.
For instance, video representations may benefit from being distinctive to time shift and/or time reversal rather than invariant to them.
It is not immediately obvious how contrastive learning should be modified to incorporate these different choices.
%
Another less apparent but important issue is how training data batches should be formed.
Contrastive learning formulations minimize, in fact, a loss that involves comparing (contrasting) the representations of different samples, and is thus \emph{not decomposable}.
In practice, the loss is approximated by sampling batches of data, and how this is done has a major effect on the performance.
In the previous example of SimCLR, if transformation $(t_1,t_2)$ is included in the batch, so must be a complementary transformation $(t_1,t_2')$ that differs only in the second factor $t_2\not=t'_2$.
This is required in order to learn the desired invariance.
It also means that transformations in a batch cannot be sampled independently.
A way to guarantee that both $(t_1,t_2)$ and $(t_1,t_2')$ are in the batch is to consider all possible combinations
$
\mathcal{T}_1\times\mathcal{T}_2
$
of two sets of transformations $\mathcal{T}_1$ and $\mathcal{T}_2$.
However this is statistically inefficient because it applies the same augmentations $\mathcal{T}_2$  to all images in the batch.
Instead, SimCLR samples at random $B/2$ images and then applies to them $B$ independently sampled augmentations.
%\todo{shouldn't it be 2B?}
This is better than the scheme above that would only use $B / |\mathcal{T}_1| = 2$ different augmentations.
However, it is unclear how this strategy for sampling diverse transformations can be extended to $M\! >\! 2$ factors.
This is studied next. %in the next section.
% it is unclear how to e in terms of sampling order and permissible combinations.
%\todo{give example why not clear?}

\subsection{Compositional contrastive learning}\label{s:main-method}

Given a batch $\mathcal{T}$ of data transformations, we consider the learning objective:
\begin{multline}\label{e:contrastive}
\footnotesize
\mathcal{L}(\Phi; \mathcal{T})
=
-
\sum_{\mathclap{T,T' \in \mathcal{T}}}
c(T,T')w(T,T') 
\\
\cdot \log
\left(
\frac{
e^{\langle \Phi(x(T)), \Phi(x(T')) \rangle/\rho}
}{
\sum\limits_{\mathrlap{T'' \in \mathcal{T}}}
w(T,T'')~
e^{\langle \Phi(x(T)), \Phi(x(T'')) \rangle/\rho}
}
\right).
\end{multline}
where $\rho > 0$ is a temperature parameter.
The \emph{contrast function} $c(T,T')\in\{0,1\}$ has the following interpretation:
when $c(T,T')=1$, then the representations $\Phi(x(T))$ and $\Phi(x(T'))$ are pulled together (invariance), and when $c(T,T')=0$ they are pushed apart (distinctiveness).
For example, in SimCLR, we set $c(T,T') = c((i,g),(i',g')) = \delta_{i=i'}$ to push apart the representations of different images $(i,i')$ while remaining invariant to a transformation pair $(g,g')$.
The \emph{weight function} $w$ is a second binary function that focuses learning on more informative transformation pairs; for instance, SimCLR sets $w(T,T')=\delta_{T\not=T'}$ to avoid focusing learning invariance to identical transformation $T=T'$ as this is trivially satisfied.
Next, we provide a semi-formal analysis of this formulation, leaving the details to~\cref{s:theory}.

\paragraph{Multiple invariances and distinctiveness.}

The key to extending~\cref{e:contrastive} to $M>2$ transformation is to build the function $c(T,T')$.
We do this one factor a time.
% \todo{ref to eq is not correct} Y: think it's fine
If we wish the representation to be distinctive to factor $t_m$, we set $c(t_m,t_m')=\delta_{t_m=t_m'}$.
If we wish it to be invariant to it, we set $c(t_m,t_m')=1$.
In \cref{l:prod,l:prod2} (\cref{s:theory}), we show that, given these choices, the only consistent definition of $c(T,T')$ is the product $\prod_{m=1}^M c(t_m,t_m')$.
The intuition is as follows:
The representation $\Phi$ should distinguish samples $x(T)$ and $x(T')$ if, and only if, at least one of the distinctive factors in $T$ and $T'$ differs.

\paragraph{Forming a batch.}

Given $c$, the remaining challenge is to sample training batches $\mathcal{T}$ appropriately.
We start by deriving some requirements for $\mathcal{T}$ and then develop a sampling scheme that satisfies them (none of these are guaranteed by sampling $T$ and $T'$ independently).
(i) First, in order for~\cref{e:contrastive} not to be identically zero, $c(T,T')$ should be non-zero for at least \emph{some} choices of $T$ and $T'$ in the batch.
(ii) Furthermore, when $c(T,T')=1$, this should not be for the trivial case $T=T'$ (the one that SimCLR discounts by setting $w(T,T')=0$).
Based on the discussion above, the condition $c(T,T')=1~\wedge~T\not=T'$ means that all distinctive factors in $T$ and $T'$ agree and that at least an invariant factor differs. 
(iii) Additionally, for the fraction in~\cref{e:contrastive} not to be a constant, if $c(T,T')=1$, there should be another $T''$ in the batch such that $c(T,T'')=0$.
The latter means that at least one distinctive factor in $T$ and $T''$ differs.%, a requirement to form a contrast based loss.

Short of considering all possible combinations of transformations (which, as explained 
above, can be statistically inefficient), we can sample a batch $\mathcal{T}$ that satisfies these constraints as follows.
We describe this process for the case of $M=3$ transformations, but note that it extends immediately to any $M$ (this is done in~\cref{s:composition,s:batches}).
First, we sample $K_1$ versions of the first distinctive transformations $t_1$.
Then, for each $t_1$, we sample $K_2$ transformations $t_2$, also distinctive.
Finally, for each choice of $(t_1,t_2)$, we sample $K_3$ invariant transformations $t_3$.\footnote{Note that the sampling ordering is arbitrary; in particular, it needs not to be the same as the ordering in which transformations are applied to the data.}
We thus obtain a batch of $|\mathcal{T}|=K_1 K_2 K_3$ transformations.

This scheme has several desirable properties.
First, for every $T=(t_1,t_2,t_3)$, there is another $T'=(t_1,t_2,t_3')$ that agrees on the distinctive factors and differs in the invariant one (properties (i) and (ii)).
Second, there is a $T''=(t_1,t_2',t_3')$ or $T''=(t_1',t_2',t_3')$ that differs in one or more distinctive factors (property (iii)).
Third, the construction is balanced, in the sense that the number of transformations that share a particular factor value $t_m$ is the same for all values of $t_m$ (this number is $|\mathcal{T}|/(K_1\cdots K_m)$).
Furthermore, SimCLR is obtained as a special case.
Please see~\cref{l:count1,l:count2} (\cref{s:theory}) for an in-depth discussion.

\paragraph{Limitations.}

Despite the benefits, this scheme has also some limitations.
The main issue is that a difference in factor $t_m$ generally implies a difference in all subsequent factors as well, meaning that the representation may be unable to observe and thus learn to discriminate changes in all individual factors.
In~\cref{s:limitations}, we show why this is unlikely to be an issue for the practical cases considered here and in the literature.
However, we also suggest other practical cases where this \emph{can} be a significant issue, affecting even methods such as SimCLR\@.

\subsection{Properties of Generalized Data Transformations\label{s:theorems}}

In this section, we show that GDT's batch sampling strategy is statistically more efficient than naively-sampled pairs for contrastive learning. 
We do this by showing that GDT's objective has the same mean but a lower variance than sampling batches with eq. \ref{e:contrastive} directly, which would either enumerate all possible pairs of transformations (which is prohibitively expensive) or subsample it by sampling transformations independently. 
We assume that the distinctive transformations are injective. 
This must be approximately true, otherwise it is impossible for any method to be distinctive to such transformations. 
% We are then able to interpret GDT as a pairwise extension of stratified sampling \cite{mcbook} (ch. 8). 
In fact, we can prove the following result:
\begin{theorem}
\label{thm:variance}Given a set of transformations $\mathcal{T}$, of which the distinctive transformations are injective, GDT is an unbiased estimate $\hat{\mathcal{L}}$ of the generalized contrastive loss (eq. \ref{e:contrastive}), i.e. $\mathbb{E}[\hat{\mathcal{L}}]=\mathcal{L}(\Phi;\mathcal{T})$. Furthermore, consider a batch of sampled compositions of $M$ transformations, with size $\prod_{j}^{M}K_{j}$, where $K_{m}$ is the number of samples for the $m$th transformation. Define $K_{I}=\prod_{j\in I}K_{j}$ and $K_{V}=\prod_{j\in V}K_{j}$, where $I$ and $V$ are the subsets of indices corresponding to invariant and distinctive transformations, respectively. Denote by $\mathcal{L}_{jj'}$ and $\sigma_{jj'}^{2}$ the mean and variance of the partial sum of the objective (eq. \ref{e:contrastive}) on the set $\mathcal{X}_{j}\times\mathcal{X}_{j'}$, with $\mathcal{X}_{j}=\{x(T^{I},T_{j}^{V}):T^{I}\in\mathcal{T}_{I}\}$, i.e. the sample pairs corresponding to distinctive transformations with indices $j$ and $j'$. Then, the variance of the GDT estimate is
\[
\mathbb{V}[\hat{\mathcal{L}}]=\frac{1}{K_{V}^{4}K_{I}^{2}}\sum_{jj'}^{K_{V},K_{V}}\sigma_{jj'}^{2}.
\]
The naive estimate's variance, on the other hand, is
\[
\mathbb{V}[\hat{\mathcal{L}}_{\textrm{d}}]=\frac{1}{K_{V}^{2}K_{I}^{2}}\sum_{jj'}^{K_{V},K_{V}}\sigma_{jj'}^{2}+\frac{1}{K_{V}^{2}}\sum_{jj'}^{K_{V},K_{V}}\left(\mathcal{L}_{jj'}-\mathcal{L}\right)^{2},
\]
which is larger by a multiplicative factor of $K_{V}^{2}$ and a further additive factor.
\, Proof: {\normalfont See Appendix A. \qed}  % inline proof uses less space
\end{theorem}

% We can prove (see Appendix 1.3, \cref{thm:variance}) 
This states that sampling data with GDT yields reduced variance, resulting in higher-quality gradients for learning the \emph{same} objective (since the estimate is unbiased), which is reflected empirically in our strong performance on numerous datasets and benchmarks. % experiments. 
We note that this may apply to other methods built on the same sampling strategy but which compose transformations in different ways than GDT, as long as the requirements (i-iii) for forming a batch (sec. \ref{s:main-method}) are satisfied.

\subsection{Application to video data}
% \todo{Why video??}
As a concrete instantiation of our framework, we consider video data and transformations of the type $T=(t_1,t_2,t_3,t_4,t_5) = (i,\tau,m,r,g)$, as shown in \cref{f:theory}, as follows.
The first component $i$ \textbf{selects} a video in the dataset.
% \todo{ordering??}
We sample $K_i \gg 2$ indices/videos and assume distinctiveness, so that~$c(i,i') = \delta_{i=i'}$.
%
The second component $\tau$ contrasts different \textbf{temporal shifts}.
We sample $K_\tau=2$ different values of a delay $\tau$ uniformly at random, extracting a 1s clip $x_{i\tau}$ starting at time $\tau$.
For this contrast, we will test the distinctiveness and invariance hypotheses, as \cite{avts} indicate that the former may be preferable.
%
The third component $m$ contrasts \textbf{modalities}, projecting the video $x_{i\tau}$ to either its visual or audio component $m(x_{i\tau})$.
We assume invariance $c(m,m')=1$ and always sample two such transformations $m_v$ and $m_a$ to extract both modalities, so $K_m = 2$.
%
The fourth component $r$ contrasts \textbf{time reversal}~\citep{pickup2014seeing, wei2018learning}, which has not previously been explored in a contrastive or cross-modal setting.
This is given by a transformation $r\in\mathcal{R}=\{r_0, r_1\}$, where $r_0$ is the identity and $r_1$ flips the time dimension of its input tensor, so $K_r = 2$.
%
The final component $g$ applies a spatial and aural \textbf{augmentation} $x(T) = g(r(m(x_{i\tau})))$, also normalizing the data.
We assume invariance $c(g,g')=1$ and pick $K_g=1$, i.e.~augment each datum at this level in the sampling hierarchy.
These choices lead to  $K=K_i K_\tau K_m K_r K_g = 8K_i$ transformations $T$ in the batch $\mathcal{T}$ (in ablations, we also test a subset of these choices).

While we focus on modality splitting, time reversal and shift, note that we could use any transformation that can yield a useful learning signal, such as speed~\citep{benaim2020speednet, cho2020selfsupervised, wang2020self, jenni2020video, yang2020video, epstein2020oops} and temporal ordering~\citep{misra2016shuffle, clip_order, lee2017unsupervised, fernando2017self}.

\paragraph{Modality splitting.}

The modality splitting transformation $m$ is useful to capture correlation between modalities~\citep{avts,Arandjelovic17,owens2016ambient,aytar2016soundnet,wei2018learning}.
Modality splitting means that the nature of the sample $x(i,\tau,m,r,g)$ is either a sequence of frames ($m=m_v$) or a sound ($m=m_a$).
Formally, this means that $x(i,\tau,m,r,g)$ is an element of the direct sum $\mathcal{X}_v \oplus \mathcal{X}_a$ of visual and audio signals; likewise $g$, $r$ and $\Phi$ are defined on this direct sum.
In practice, this means that the transformation $g$ comprises a pair of augmentations $(g_v,g_a)$, where $g_v(v)$ extracts a fixed-size tensor by resizing to a fixed resolution of a random spatial crop of the input video $v$, and $g_a(a)$ extracts a spectrogram representation of the audio signal followed by SpecAugment~\citep{Park_2019} with frequency and time masking.
Likewise, $\Phi=(\Phi_v,\Phi_a)$ comprises a pair of neural networks, one for each modality, both valued in $\mathbb{R}^d$ (refer to~\Cref{s:appx:traindetails} for architectural details).
In the \cref{s:appx:cross-vs-within-modal}, we show that modality splitting is key for performance; thus, we extend SimCLR weight function $w$ to focus learning on only cross-modal pairs:
$w(T,T)=\delta_{i\not= i} \cdot \delta_{m\not=m'}$.

\subsection{Discussion: utility of GDT}

With our framework, we can now generalize current state of the art contrastive learning approaches such as SimCLR in a systematic and practical manner.
The theory above and in~\cref{s:theory} tells us what is the meaning of composing transformations, how a batch should be sampled and why, how this can be achieved by using a hierarchical sampling scheme that extends SimCLR, and what are the limitations of doing so.
A particular benefit is to allow to specify individually, for each transformation, if invariance or distinctiveness is sought,
% generalization allows the composition of any arbitrary transformations, while specifying the choice of learning either invariances and variances simultaneously for each transformation,
whereas previous works lack this distinction and largely considered learning only invariances (SimCLR~\citep{Chen2020ASF}, AVID~\citep{morgado2020avid}), or distinctiveness (AoT~\citep{wei2018learning}) to all factors.
This property allows the flexible utilization of dataset specific transformations in the case of prior knowledge, or, as we have shown in this study, the exploration of useful signals by enumeration. Finding the best transformation signals can even be further optimized by methods such as Bayesian optimization.
Finally, compared to a direct application of previous state-of-the-art methods image-based methods such as SimCLR~\citep{Chen2020ASF}, PIRL~\cite{misra2019selfsupervised}, and MoCo~\citep{he2019momentum}, we can also seamlessly incorporate important cues such as cross-modal correlation, greatly improving downstream performance (see \cref{tab:appx:ablation:modality}).

% A particular benefit is to extend incorporate multiple modalities, compared to previous contrastive formulations, such as   which work only on images. 

% Benefits of GDT formulation, particularly applied to video? Why apply GDT to multi-modal representation learning?  Key differences (novelty) in formulation relative to SimCLR (for images), CMC (multi-view learning), and AVID (audio-visual contrastive training)?

% Our method can also be used to investigate any future transformations that can yield a useful signal.
% If we use this transformation, we always sample both, setting $K_r=2$.

% With this formulation, we can now generate new learning signals by choosing the transformations to be invariant and distinctive to. %We now apply the framework to generalize the multi-modal contrastive scheme described above.
% Taking, for example  $\ast=0$, a noise-contrastive version of~\cite{avts} can be constructed, or by setting $\ast= \cdot$, we generate a novel, cross-modal SimCLR-like loss. %  resulting scheme is illustrated in~\cref{fig:splash}.


==> GDT (ICCV 2021)/4_experiments.tex <==
\section{Experiments}\label{sec:experiments}

We compare self-supervised methods on pretraining audio-visual representations.
Quality is assessed based on how well the pretrained representation transfers to downstream tasks.
We conduct a study on video-audio, as well as video-text unsupervised representation learning to show the generality of our framework and then compare our best setup to the state of the art.
%to determine the best learning transformations and setup.
%Then, we use the latter to compare to the state of the art.

\paragraph{Self-supervised pretraining.}

For pretraining, we consider two standard pretraining datasets: Kinetics-400 ~\citep{kinetics} and HT100M~\citep{miech2019howto100m} and use R(2+1)D-18~\citep{tran2018closer} and a 2D ResNet~\citep{KaimingHe16} as encoders (see Appendix for further details). 
We also explore how our algorithm scales to even larger, less-curated datasets and train on IG65M~\citep{Ghadiyaram2019} as done in XDC~\citep{alwassel2019self}.
%AudioSet~\citep{AudioSet}, and additionally, the recently released, VGG-Sound dataset~\citep{VGGSound}.
%The videos in Kinetics are about 10-seconds long, each depicting one of 400 different actions.
%VGG-Sound and AudioSet are both audio-visual datasets consisting of short clips of audio events, extracted from videos uploaded to YouTube, each depicting one of 300 and 632  different acoustic audio events respectively.
%After removing samples without audio, we are left with around $230$K videos for Kinetics, $170$k videos for VGG-Sound and $1.8$M videos for AudioSet, which we use for pretraining completely without labels.
% Finally, we also explore how our algorithm scales to even larger, less-curated datasets and train on IG65M~\citep{Ghadiyaram2019} as done in XDC~\citep{alwassel2019self}.

% Our method learns a pair of representations $f=(f_v,f_a)$ for visual and audio information respectively and we refer to~\Cref{s:appx:traindetails} for architectural details.

\paragraph{Downstream tasks.}
To assess the pretrained representation $f_v$, we consider standard action recognition benchmark datasets, UCF-101~\citep{UCF101} and HMDB-51~\citep{kuehne2011hmdb}.
%UCF-101 contains about 13K videos from 101 human action classes, and HMDB-51 consists of 7K clips spanning 51 different human activities.
We test the performance of our pretrained models on the tasks of finetuning the pretrained representation, conducting few-shot learning and video action retrieval.
%To assess the \textbf{audio} representation $f_a$, we train a linear classifier on frozen features for the common ESC-50~\citep{esc50} and DCASE2014~\citep{DCASE} benchmarks.% and finetune for VGG-Sound~\citep{VGGSound}.
The full details are given in the Appendix.

\subsection{Analysis of generalized data transformations}\label{s:exp.hypothesis}

\input{tabs/t2_hypothesis-res}

In this section, we conduct an extensive study on each parameter of the GDT transformation studied here, $T = (i, \tau, m, r, g)$, and evaluate the performance by finetuning our network and conduncting video retrieval on the HMDB-51 action recognition benchmark.

\paragraph{SimCLR-like baseline.}

First, we use the framework to test a direct extension of SimCLR to video data, as shown in \Cref{tab:hypotheses_results}(a)-(d).
By this, we mean utilizing only the visual modality (V), and only invariance to transformations, which is standard in all recent self-supervised methods~\citep{Wu_2018_CVPR,he2019momentum,Chen2020ASF}.
For this, we consider GDTs of the type $T = (i, m_, \tau, r, g)$ described above and set $K_i=512$ (the largest we can fit in our setup).
In row (a), we pick only the video modality ($m=m_v$ so $K_m=1$).
We also sample a single shift $\tau$ (so $K_\tau=1$), which results in data augmentation but does not learn shift invariance, and no time reversal $r=1$ (so $K_r=1$) --- these are denoted with a $\cdot$ in the table.
However, we do sample two visual augmentations $g$ ($K_g=2$), emulating SimCLR and learning invariance to that factor.
We also set all transformation components to invariance ($c(t_m,t'_m)=1$) except the first that does sample selection.
In row (b-d) we also experiment with adding invariance to \emph{time shift} (TS) and \emph{time reversal} (TR), by setting $K_\tau=2$ and $K_r=2$.
We find that doing so consistently degrades the finetuning accuracy performance, but increases the retrieval performance somewhat, indicating that the model is not able to fully leverage these augmentation signals in a meaningful way.

\paragraph{Cross-modal learning.}

Next, in rows (e-h) we repeat this experiment, but using both audio-visual modalities (AV) by setting $K_m=2$.
In this case, as explained above, we set the weight $w$ to only consider cross-modal interactions and set $K_g=1$.
We note two facts:
First, the performance increases substantially (+7.8\% (e) vs (a-d)).
Second, now TS and TR invariance leads to significant improvements (up to +7.5\%).

\paragraph{Invariance vs distinctiveness.}

Next, in rows (i-l), we explore the effect of being invariant or distinctive to individual transformations, which is unique to our method.
Comparing row (h) to rows (k) and (l), we see that switching to distinctiveness to one of TS or TR further improves performance (up to +1.5\%).
On the other hand, `ignoring' either ($\cdot$ symbols in lines (g) and (j)) is worse than learning invariance ((h) and (l)), with a difference of around 2.5\%.
Finally, in row (m) we find that being distinctive for both TS and TR at the same time is worse, suggesting that a mix of distinctiveness and invariance is preferable.
This is particularly true for the retrieval metric (column R@1).

\subsection{Textual modality}\input{tabs/queryd}

In~\cref{t:text}, we demonstrate the generality of our approach by using ASR captions as an alternative modality (instead of audio) for the HowTo100M dataset~\citep{miech2019howto100m}. 
For the text encoder, we use a simple Word2Vec~\citep{mikolov2013efficient} embedding with a MLP (further details are provided in the Appendix).
Comparing \cref{t:text}(a) with (b), we find that switching from SimCLR to a cross-modal baseline increases performance by more than +22\%. 
Furthermore, we find gains of 3.7\% when switching from data-sampling distinctiveness only (row (b)) to incorporating further distinctivenesses (rows c-d). 
Finally, we find that -- as in the video-audio case -- combining time-shift distinctiveness with time-reversal invariance leads to particularly strong representations (row (f)), yielding benefits of over +5\% compared to data-sampling distinctiveness alone.
Compared to video-audio learning (\cref{tab:hypotheses_results}(m)), we find the case of distinctive-only for video-text learning (\cref{tab:queryd-av}(g)) to be highly competitive, highlighting the need to explore the set of possible transformation signals to achieve the best downstream performance.

\paragraph{Intuition.}
While we only analyse a subset of possible transformations for video data, we nevertheless find consistent signals across both video-audio and video-text learning:
Inclusion of further distinctivenesses to TS and TR always improve upon the basecase and the best setup is achieved for TS distinctiveness and TR invariance. 
%help for all setups, and the furthermore we found 
%While both TR and TS could function as a meaningful invariance transformation to provide the model with more difficult positives \textit{a-priori}, we find that using them instead to force \textit{distinctiveness} can work better, especially when combined with invariance.
One explanation for this might be that there is useful signal in both of these transformations that are not captured by previous ``augmentation-only'' naive noise-contrastive formulations.
For example, for time-shift (TS), the model profits from having to differentiate different points in time, e.g. between an athlete running vs an athlete landing in a sandpit, which could be both in the same video. 
This intuitively serves as a hard negative for the model, increasing its discriminative power.
For time reversal (TR), many actions depicted such as moving an object are inherently invariant to reversing time, as shown in~\citep{price2019_RetroActionsLearning}, therefore yielding a gain when used as an augmentation. 
In ~\citep{wei2018learning}, they show that humans have a $20\%$ error-rate when classifying a video’s direction of time in Kinetics-400, thus demonstrating that Kinetics-400 has subsets of videos that look realistic even when reversed. 
These findings that additional distinctiveness combined with invariances improve video representation learning are noteworthy, as they contradict results from the image self-supervised learning domain, where learning pretext-invariance can lead to more transferable representations~\citep{misra2019selfsupervised}. 
%This is likely due to the fact that TS and TR are useful signals that both require learning strong video representations to pick up on.
Even when compared to previous self-supervised learning approaches for video-data, such as predicting the arrow of time~\citep{wei2018learning}, our method yields new insights by showing that a unique combination of distinctivenesses and invariances performs best, at least on the training sets considered.
Combining these points, the strong performance of GDT is founded in its ability to leverage highly informative, yet ``free'', signal that we have from construction of the transformations.

\subsection{Qualitative analysis}
\begin{figure}[!t]
    \centering
\includegraphics[width=0.9\columnwidth]{figs/timeshifts.pdf}
    \caption{Learning distinctiveness to time-shifts: our GDT model from Tab.1(j) is able to differentiate features from the same video at different times better than a simple SimCLR variant (Tab.1(a)).
    \label{fig:histogram}}
\end{figure}
Here, we study what effect the different transformations we let our model be invariant and distinctive to have on our learned representations.
For this, we compare against the SimCLR baseline of Tab.1(a) and compare the average standard deviation of the normalized features for 10 time-shifted clips per video for 3000 randomly selected Kinetics-400 validation set.

\subsection{Comparison to the state of the art}

\input{tabs/t45_ret-few-aud}

\input{tabs/t3_video-sota}

Given one of our best learning setups from~\cref{s:exp.hypothesis} (row (l)), we train for longer and compare our feature representations to the state of the art on standard downstream benchmarks. %common visual and aural downstream benchmarks.

\subsubsection{Downstream benchmarks}

For \textbf{few-shot classification}, as shown in ~\cref{tab:few-shot-ret}, we significantly beat the 3D-Rotnet~\citep{jing2018self} baseline on UCF-101 by more than $10\%$ on average for each shot with our Kinetics-400 pretrained model.

For \textbf{video retrieval}, we report recall at 1 and 5  retrieved samples for split-1 of the HMDB-51 and UCF-101 datasets in~\cref{tab:few-shot-ret}.% (the results for recall at 10 and 50 are provided in the Appendix).
Using our model trained on Kinetics-400, \methodname~significantly beats all other self-supervised methods. 
In particular, we outperform CoCLR~\citep{Han2020SelfsupervisedCF}, a recent state-of-the-art self-supervised method, that uses optical flow as another view to mine hard positive to improve instance discrimination learning for video representations. 
Moreover, we surpass SeLaVi, an audio-visual clustering and representation learning method, by $2\%$ and $10\%$ on average on recall at 1 and 5 for HMDB-51 and UCF-101.  

For \textbf{video action recognition}, we finetune our \methodname~pretrained network for UCF-101 and HMDB-51 video classification, and compare against state-of-the-art self-supervised methods in~\cref{tab:sota}.
When pretrained on the Kinetics datasets, we find that our \methodname~pretrained model achieves very good results, outperforming all recent methods. 
In particular, we outperform audio-visual pretraining methods, AVTS~\citep{avts}, SeLaVi~\citep{asano2020labelling} and XDC~\citep{alwassel2019self}, by large margins using the same architecture (R(2+1)D-18) and dataset (Kinetics-400), showing the effectiveness of our GDT pre-training approach.
We also surpass AVID~\cite{morgado2020avid}, the state-of-the-art audio-visual representation learning method, by $1.5\%$ on HMDB-51 and $3.8\%$ on UCF-101. 
AVID uses a variant of the pre-training scheme of our baseline approach that extends noise contrastive learning to the audio-visual domain as in \Cref{tab:hypotheses_results}, row (e). 
However, while AVID simply encodes sample distinctiveness and invariance to modality in its visual representations, we are able to encode invariances and distinctiveness to additional transformations, which significantly improves our performance. 
Our approach is also more sample efficient, as we are able to achieve our results with 300 less epochs of training. 
Finally, when pretrained on HT100M, we achieve strong gains of $+6.4\%$ on HMDB-51 and $+2.8\%$ on UCF-101 compared to the state-of-the-art video text method, MIL-NCE~\cite{miech2019endtoend}. 
Similar to AVID, MIL-NCE uses a variant of the baseline cross-modal contrastive framework to learn representations, while we are able to improve upon this baseline by learning invariance and distinctiveness to additional transformations such as time reversal and time shift. 
Moreover, with HT100M pre-training, we outperform the Kinetics supervised baseline using the same architecture when finetuned on HMDB-51 ($67.4$ vs $65.1$) and are on par for UCF-101 ($94.1$ vs $94.2$). 
We further show the scalability and flexibility of our GDT framework by pretraining on the IG65M dataset~\citep{Ghadiyaram2019}.
With this, our visual feature representation sets a new state of the art among all self-supervised methods, particularly by a margin of $> \!4\%$ on the HMDB-51 dataset.
On UCF-101, we set similar state-of-the-art performance with XDC.
Along with XDC, we beat the Kinetics supervised pretraining baseline using the same architecture and finetuning protocol.

% and UCF-101 action recognition datasets. 
    
%among all self-supervised approaches on both downstream action recognition datasets, also surpassing the CPD~\citep{li2020learning} method on HMDB-51 and UCF-101 which uses weak supervision of video titles for pretraining a network.
%When constrained to pretraining on the AudioSet~\citep{AudioSet} dataset, we also find state-of-the-art performance among all self-supervised methods, particularly on HMDB-51. We get similar performance to XDC on UCF-101. 
%Lastly, we show the scalability and flexibility of our GDT framework by pretraining on the IG65M dataset~\citep{Ghadiyaram2019}.
% With this, our visual feature representation sets a new state of the art among all self-supervised methods, particularly by a margin of $> \!4\%$ on the HMDB-51 dataset.
% On UCF-101, we set similar state-of-the-art performance with XDC.
% Along with XDC, we beat the Kinetics supervised pretraining baseline using the same architecture and finetuning protocol.

% \subsubsection{Downstream audio benchmarks.}
% For \textbf{audio classification}, we find that we achieve  state-of-the-art performance among all self-supervised methods on both DCASE2014 and ESC-50.
%, and also surpass supervised performance when finetuning on VGG-Sound with $54.8\%$ mAP.



==> GDT (ICCV 2021)/5_conclusion.tex <==
\section{Conclusion}

We introduced the framework of Generalized Data Transformations (GDTs), which allows one to capture, in a single noise-contrastive objective, cues used in several prior contrastive and non-contrastive learning formulations, as well as easily incorporate new ones.
The framework shows how new meaningful compositions of transformations can be obtained, encoding valuable invariance and distinctiveness that we want our representations to learn.
% Following this methodology, we achieved state-of-the-art results for self-supervised pretraining on standard downstream video action recognition benchmarks, even surpassing supervised pretraining on HMDB-51.
Following this methodology, we achieved state-of-the-art results for self-supervised pretraining on standard downstream video action recognition benchmarks, even surpassing supervised pretraining.
Overall, our method significantly increases the expressiveness of contrastive learning for self-supervision, making it a flexible tool for many multi-modal settings, where a large pool of transformations exist and an optimal combination is sought. 

%for further research in the area.

% In this work, we have introduced a framework for data transformations in a multi-modal setting that extends the recent advances in self-supervised learning of images and videos.
% We show empirically that the data transformations, how they are sampled and contrasted, are the key ingredient in contrastive formulations because it encodes the valuable invariances and distinctiveness we want our representations to learn.
% By means of ablations, we validate that our Generalized Data Transformation framework is well suited for training representations in a self-supervised manner when combined with a noise contrastive loss and report state-of-the-art results for self-supervised pretraining on standard downstream video action recognition tasks, even surpassing supervised pretraining.`'



==> GDT (ICCV 2021)/7_broader_impact.tex <==
\clearpage
\section*{Broader impact}

We see the research presented in this work to have a potential broader impact in three main areas over the short and long term.
\paragraph{Reduce bias on less curated data}
The promise of self-supervised methods is to learn ever more robust and general visual representation models without manual annotations. 
Indeed, training on ever larger datasets with ever better methods has continued to increase performance on downstream tasks and we have presented similar findings in this paper.
This shows the potential and benefit of self-supervised learning compared to supervised or weakly-supervised learning, and also has the added potential to reduce the risk of incorporating biases present in the training data.
As biases start in the data collection process, using less curated data and significantly more of it might be useful in having less biased models as these will be trained with more diversity. 
We should also note that biases present in these models might disappear once the network is fine-tuned on a target task (on which biases should, also be avoided or known).
However, it is still crucial to understand this aspect in detail when it comes to deployment and we believe that research should be encouraged probing self-supervised models with regards to their underlying data distributions, in a similar way to \citep{jahanian2020On,voynov2020unsupervised} for images, and as has been done more rigorously in the NLP domain for some time, e.g. \cite{bolukbasi2016man,qian2019reducing,park2018reducing,zhao2019gender}.

\paragraph{Applications in medical imaging.} Using pretrained visual feature representations, such as those obtained by training on ImageNet LSVRC-12 and finetuning these on specific medical imaging tasks has been very successful~\cite{xie2018pre,schlegl2014unsupervised,litjens2017survey}.
Models obtained in such a manner outperform those trained from scratch and vice versa require less expert time for human annotation~\cite{overviewmedical}. 
Thus far, these mostly 2D CNN models were used for transfer learning, but there are applications were the temporal dimension is key, such as heart imaging with ultra sound~\cite{huang2017temporal}. 
It is likely that self-supervised video representation models, such as the one presented in this paper will be useful for these applications, with the implications of a) increasing the accuracy of the physician's diagnosis,  b) reducing the time-cost of diagnosis, and c) facilitating remote diagnostics in places with not enough trained staff.
However, a risk with algorithms in unsupervised learning is that users may put too much blind trust on the results of the algorithm (in our case a network initialization). 
In practice, there are no guarantees that the algorithm would find a solution fit for any particular downstream application.
This needs to be carefully validated a posteriory.

\paragraph{Harmful content detection.}
The number of uploaded videos to online platforms only keeps increasing, yet automatically detecting harmful content is still in its infancy. 
As content is now increasingly moving towards videos, self-supervisedly trained video models may be especially useful for transfer learning. 
The benefits are a) the models can be more accurately detect harmful content, leading to both higher recall and precision, and b) training good classifiers requires less annotations from humans, which are in this case not just expensive but psychologically harmful.

Furthermore we encourage ways of getting the research community to participate in these developments in ways that do not require the release and distribution of such material. 
One recent such initiative is the hateful memes competition\footnote{\url{https://www.drivendata.org/competitions/64/hateful-memes/}}, which although based on image understanding captures the difficulties of multi-modal learning and the nuances of understanding intention.


==> GDT (ICCV 2021)/figs/splash.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.7\linewidth]{figs/NCE.pdf}
    \caption{\textbf{Example instantiation.}
    % \textbf{A}: Hierarchical sampling process of generalized transformations $T=t_M \circ ... \circ t_1$ for the multi-modal training study case. 
    % %\textbf{B}: Subset of the $c(T,T')$ contrast matrix which shows which pairs are repelling (0) and attracting (1) (see text for details).
    % \textbf{B}: With generalized data transformations (GDT), the network learns a meaningful embedding via learning desirable invariances and distinctiveness to transformations (realigned here for clarity) across modalities and time.
    The embedding is learned via noise contrastive (NCE) learning. Here we show the case of audio-visual sample and time-shift distinctiveness: video-audio embeddings from the same video at the same time are pulled together, while audio-visual sample pairs from different videos and different starting times are pushed apart. 
    % Illustrational videos taken from YouTube~\citep{vidsource}.
    \label{fig:nce}}
%  \vspace{-12pt}
\end{figure}

==> GDT (ICCV 2021)/figs/splash_source.tex <==
  \begin{figure}
   \newcommand{\Tone}{\colorbox{blue!30}{$T_1$}\xspace}
   \newcommand{\Ttwo}{\colorbox{blue!20}{$T_2$}\xspace}
   \newcommand{\Tthree}{\colorbox{blue!10}{$T_3$}\xspace}
   \newcommand{\Tfour}{\colorbox{blue!5}{$T_4$}\xspace}
   \newcommand{\Tfive}{\colorbox{red!30}{$T_5$}\xspace}
   \newcommand{\Tsix}{\colorbox{red!20}{$T_6$}\xspace}
   \newcommand{\Tseven}{\colorbox{red!10}{$T_7$}\xspace}
   \newcommand{\Teight}{\colorbox{red!5}{$T_8$}\xspace}
   \fboxsep1pt
   \footnotesize
   \begin{tikzpicture}[grow'=right,
     edge from parent/.style={draw,-latex},
     label distance = 0.1cm,
     level 1/.style = {level distance=1cm, sibling distance=4mm},
     level 2/.style = {level distance=1cm, sibling distance=8mm},
     level 3/.style = {level distance=1cm, sibling distance=4mm},
     level 4/.style = {level distance=1cm, sibling distance=4mm},
     level 5/.style = {level distance=0.5cm, sibling distance=4mm, edge from parent/.style={}},
     ]
   \node (X) {1}
   child { node[label={$t_1$}] at ($(X)+(1,+1.6)$) {$i_1$}
       child { node[label={$t_2$}]{$\tau_1$}
           child { node[label={$t_3$}]{$m_v$}
               child { node[label={$t_4$}]{$g_1$} child { node{\Tone}} }
           }
           child { node{$m_a$}
               child { 
                    child { nchild { node{\Ttwo}} } node{$g_2$}
                    child { node{\Ttwo}} }
           }
       }
       child { node{$\tau_2$}
           child { node{$m_v$}
               child { node{$g_3$} child { node{\Tthree}} }
           }
           child { node{$m_a$}
               child { node{$g_4$} child { node{\Tfour}} }
           }
       }
   }
   child { node at ($(X)+(1,0)$) {$i_2$}
       child { node{$\tau_3$}
           child { node{$m_v$}
               child { node{$g_5$} child { node{\Tfive}} }
           }
           child { node{$m_a$}
               child { node{$g_6$} child { node{\Tsix}} }
           }
       }
       child { node{$\tau_4$}
           child { node{$m_v$}
               child { node{$g_7$} child { node{\Tseven}} }
           }
           child { node{$m_a$}
               child { node{$g_8$} child { node{\Teight}} }
           }
       }
   }
   child { node at ($(X)+(1,-0.5)$) {$\dots$} }
   child { node at ($(X)+(1,-1)$) {$i_{M_i}$}
       child { node{$\dots$} }
   }
   ;
   \end{tikzpicture}
   \hfill
   \newcommand{\zp}{$\cdot$}
   \newcommand{\0}{$\cdot$}
   \newcommand{\m}{$0$}
   \newcommand{\as}{$\ast$}
   % \newcommand{\1}{\fcolorbox{LimeGreen!100}{white}{\bf{1}}}
   \newcommand{\1}{$1$}
   \newcommand{\ld}[1]{\ldelim\{{2}{*}[\parbox{2mm}{\rotatebox[origin=c]{90}{\tiny #1}}]}
   % \newcommand{\ld}[1]{}
   \begin{tabular}[b]{c@{\,}c|cccc|cccc}
       \multicolumn{2}{c}{}
       & \multicolumn{4}{c}{\tiny video $i_1$}
       & \multicolumn{4}{c}{\tiny video $i_2$} \\[-.5em]
       \multicolumn{2}{c}{}
       & \multicolumn{4}{c}{\tiny \downbracefill}
       & \multicolumn{4}{c}{\tiny \downbracefill}\\[-.5em]
       \multicolumn{2}{c}{}
       & \multicolumn{2}{c}{\tiny visual}
       & \multicolumn{2}{c}{\tiny audio}
       & \multicolumn{2}{c}{\tiny visual}
       & \multicolumn{2}{c}{\tiny audio} \\[-.5em]
       \multicolumn{2}{c}{}
       & \multicolumn{2}{c}{\downbracefill}
       & \multicolumn{2}{c}{\downbracefill}
       & \multicolumn{2}{c}{\downbracefill}
       & \multicolumn{2}{c}{\downbracefill} \\
               & $c$     & \Tone & \Tthree & \Ttwo & \Tfour & \Tfive & \Tseven & \Tsix & \Teight \\
   \cline{2-10}
   \ld{audio}  & \Ttwo   & \1    & \as     & \0    & \zp    & \m     & \zp      & \zp   & \zp  \\
               & \Tfour  & \as   & \1      & \zp   & \0     & \zp     & \m      & \zp   & \zp \\
   \ld{visual} & \Tone   & \0    & \zp     & \1    & \as    & \zp    & \zp     & \m    & \zp \\
               & \Tthree & \zp   & \0      & \as   & \1     & \zp    & \zp     & \zp    & \m \\
   \cline{2-10}
   \ld{audio}  & \Tsix   & \m    & \zp      & \zp   & \zp    & \1     & \as     & \0    & \zp \\
               & \Teight & \zp    & \m      & \zp   & \zp    & \as    & \1      & \zp   & \0 \\
   \ld{visual} & \Tfive  & \zp   & \zp     & \m     & \zp     & \0     & \zp     & \1    & \as \\
               & \Tseven & \zp   & \zp     & \zp    & \m     & \zp    & \0      & \as   & \1 \\
   \end{tabular}
   \caption{
       \textbf{Left}: Hierarchical sampling process of generalized transformations for the multimodal training study case.
       All transformations are contrastive except $t_4$ which is augmentative.
       \textbf{Right}: Subset of the $c(T,T')$ matrix illustrating its pattern.
       The matrix has a block-diagonal structure (transformations have been reordered to highlight the pattern).
       The diagonal contrasts different modalities subject to the same time shift (e.g.~\Tone vs \Ttwo), for which we assume invariance ($1$).
       Identical (e.g.~\Tone vs \Tone) or within modality (\Tone vs \Tthree) comparisons are ignored, setting $w(T,T')=0$ (denoted by a $\cdot$). % in the table).
       The major off-diagonal blocks are set to $0$ as we assume sample distinctiveness (e.g.~\Tone vs \Tsix). %, except for within modality comparisons that we still ignore.
       Contrasting time shifts (e.g.~\Tone vs \Tfour) can be used for invariance, distinctiveness or ignored (baseline), so $\ast \in \{+1,0,\cdot\}$.
   }\label{f:theory}
   \end{figure}

==> GDT (ICCV 2021)/figs/splash_update.tex <==
\begin{figure}
%   \renewcommand{\Tone}{\colorbox{blue!30}{$T_{01}$}\xspace}
%   \renewcommand{\Ttwo}{\colorbox{blue!20}{$T_{02}$}\xspace}
%   \renewcommand{\Tthree}{\colorbox{blue!10}{$T_{03}$}\xspace}
%   \renewcommand{\Tfour}{\colorbox{blue!5}{$T_{04}$}\xspace}
%   \renewcommand{\Tfive}{\colorbox{red!30}{$T_{05}$}\xspace}
%   \renewcommand{\Tsix}{\colorbox{red!20}{$T_{06}$}\xspace}
%   \renewcommand{\Tseven}{\colorbox{red!10}{$T_{07}$}\xspace}
%   \renewcommand{\Teight}{\colorbox{red!5}{$T_{08}$}\xspace}
%   \newcommand{\Tnine}{\colorbox{blue!30}{$T_{09}$}\xspace}
%   \newcommand{\Tten}{\colorbox{blue!20}{$T_{10}$}\xspace}
%   \newcommand{\Televen}{\colorbox{blue!10}{$T_{11}$}\xspace}
%   \newcommand{\Ttwelve}{\colorbox{blue!5}{$T_{12}$}\xspace}
%   \newcommand{\Tthirteen}{\colorbox{red!30}{$T_{13}$}\xspace}
%   \newcommand{\Tfourteen}{\colorbox{red!20}{$T_{14}$}\xspace}
%   \newcommand{\Tfifteen}{\colorbox{red!10}{$T_{15}$}\xspace}
%   \newcommand{\Tsixteen}{\colorbox{red!5}{$T_{16}$}\xspace}

\renewcommand{\Tone}{{$T_{01}$}\xspace}
\renewcommand{\Ttwo}{{$T_{02}$}\xspace}
\renewcommand{\Tthree}{{$T_{03}$}\xspace}
\renewcommand{\Tfour}{{$T_{04}$}\xspace}
\renewcommand{\Tfive}{{$T_{05}$}\xspace}
\renewcommand{\Tsix}{{$T_{06}$}\xspace}
\renewcommand{\Tseven}{{$T_{07}$}\xspace}
\renewcommand{\Teight}{{$T_{08}$}\xspace}
\newcommand{\Tnine}{{$T_{09}$}\xspace}
\newcommand{\Tten}{{$T_{10}$}\xspace}
\newcommand{\Televen}{{$T_{11}$}\xspace}
\newcommand{\Ttwelve}{{$T_{12}$}\xspace}
\newcommand{\Tthirteen}{{$T_{13}$}\xspace}
\newcommand{\Tfourteen}{{$T_{14}$}\xspace}
\newcommand{\Tfifteen}{{$T_{15}$}\xspace}
\newcommand{\Tsixteen}{{$T_{16}$}\xspace}

\fboxsep0.5pt
\footnotesize
\begin{tikzpicture}[grow'=right,
  edge from parent/.style={draw,-latex},
  node distance=10mm,
  label distance = 0.2cm,
  %level 1/.style = {level distance=1cm, sibling distance=4mm},
  % level 2/.style = {level distance=1cm, sibling distance=mm},
  level 3/.style = {level distance=1cm, sibling distance=7mm},
  level 4/.style = {level distance=1cm, sibling distance=3mm},
%   level 5/.style = {level distance=1cm, sibling distance=250mm},
  %level 6/.style = {level distance=0.5cm, sibling distance=5mm, edge from parent/.style={}},
  ]
\node (X) {1}
child { node[label={$t_1$}] at ($(X)+(1,+0.5)$) {$i_1$}
    child { node[label={$t_2$}] {$\tau_1$} 
        child { node[label={$t_3$}] {$m_v$}
            child { node[label={$t_4$}]{$r_0$} 
                 child { node[label={$t_5$}]{$g_{01}$} child { node{\Tone}} } }
            child { node{$r_1$} 
                 child { node{$g_{02}$} child { node{\Ttwo}} } }
        }
        child { node {$m_a$}
            child { node {$r_0$} child { node{$g_{03}$} child { node{\Tthree}} } }
            child { node {$r_1$} child { node{$g_{04}$} child { node{\Tfour}} } }
        }
    }
    child { node  {$\tau_2$}
        child { node {$m_v$}
            child { node{$r_0$} child { node{$g_{05}$} child { node{\Tfive}} } }
            child { node{$r_1$} child { node{$g_{06}$} child { node{\Tsix}} } }
        }
        child { node {$m_a$}
            child { node{$r_0$} child { node{$g_{07}$} child { node{\Tseven}} } }
            child { node{$r_1$} child { node{$g_{08}$} child { node{\Teight}} } }
        }
    }
}
child { node at ($(X)+(1,-2.75)$) {$i_2$}
    child { node {$\tau_3$}
        child { node {$m_v$}
            child { node{$r_0$} child { node{$g_{09}$} child { node{\Tnine}} } }
            child { node{$r_1$} child { node{$g_{10}$} child { node{\Tten}} } }
        }
        child { node {$m_a$}
            child { node{$r_0$} child { node{$g_{11}$} child { node{\Televen}} } }
            child { node{$r_1$} child { node{$g_{12}$} child { node{\Ttwelve}} } }
        }
    }
    child { node{$\tau_4$}
        child { node {$m_v$} 
            child { node{$r_0$} child { node{$g_{13}$} child { node{\Tthirteen}} } }
            child { node{$r_1$} child { node{$g_{14}$} child { node{\Tfourteen}} } }
        }
        child { node {$m_a$}
            child { node{$r_0$} child { node{$g_{15}$} child { node{\Tfifteen}} } }
            child { node{$r_1$} child { node{$g_{16}$} child { node{\Tsixteen}} } }
        }
    }
}
child { node at ($(X)+(1,-4.0)$) {$\quad \dots$} }
child { node at ($(X)+(1,-4.8)$) {$i_{M_i}$}
    child { node{$\dots$} }
};
\end{tikzpicture}
\hfill
\caption{
    Hierarchical sampling process of generalized data transformations (GDTs).
    Shown here are the five transformations analyzed for the audio-visual training case and their compositions: data-sampling ($t_1$), time-shift  ($t_2$), modality splicing ($t_3$), time-reversal ($t_4$), and augmentation transformations, $g$ ($t_5$) to learn video representations via noise contrastive learning.
}\label{f:theory}
\end{figure}

==> GDT (ICCV 2021)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{d}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> GDT (ICCV 2021)/scratch.tex <==

\subsection{The general case: contrastive and augmentative transformations}

In order to instantiate~\cref{e:contrastive}, we require not only a definition of the function $c(T,T')$, but also a way of sampling transformations in the batch.
Differently from most learning formulations, in contrastive learning, one \emph{must} ensure that the batch contains transformations that can be meaningfully contrasted, so transformations cannot be sampled independently.

We propose the following \emph{hierarchical} sampling scheme.
Each generalized transformation $T=t_M \circ \dots \circ t_1$ is constructed as a sequence of $M$ transformations $t_m$.
First, we sample  $K_1$ versions of transformation $t_1$; then, for each sample $t_1$, we sample $K_2$ versions of transformation $t_2$ and so on, obtaining a total of $K=\prod_{m=1}^M K_m$ different transformations $T$ for the batch.

We distinguish between two types of transformations, depending on how we sample them.
For a \emph{contrastive transformation} $t_m$, we always sample \emph{two or more versions} of the same transformation, i.e.~$K_m \geq 2$.
For an \emph{augmentative transformation}, we only sample a single version, i.e.~$K_m=1$.
As the name suggests, contrastive transformations lead to explicit comparisons in the loss~\cref{e:contrastive}, whereas augmentative ones do not.\todo{This distinction actually does not make sense. Will likely remove.}

Given two generalized transformations $T=t_M\circ\dots\circ t_1$ and $T'=t'_M\circ\dots\circ t'_1$ sampled in this manner, we must also define $c(T,T')$.
For individual transformations, we set:
\begin{equation}
c(t_m,t_m')
=
\begin{cases}
1, & \text{if $t_m$ is augmentative or invariant contrastive},\\
2\delta_{t_m=t_m'}-1, & \text{if $t_m$ is distinctive contrastive.}
\end{cases}
\end{equation}
Then, if any $c(t_m,t_m')=-1$, we set $c(T,T')=-1$ for the overall transformation, otherwise we set $c(T,T')=1$.
In practice, we consider slightly refined definitions of $c(T,T')$ to allow for some comparisons to be ignored ($c(T,T')=0$), as suggested above and further detailed below.

\subsection{Learning hypotheses}
\begin{figure}[!tb]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/GDT_template.pdf}
    \caption{\textbf{The GDT loss template.}
    xxx.
    }\label{fig:template}
\end{figure}

Next, we describe the learning hypotheses explored in the paper.
These correspond to different definitions of the function $c(T,T')$, coding for invariance or distinctiveness to various transformations.
The function defaults to $c(T,T')=1$ (invariance), with the following modifications:

\paragraph{Sample distinctiveness.}

The representation must distinguish different videos, so that $i \not = i' \Rightarrow c(T,T')=0$.
This is the baseline on which the other hypotheses build upon.

\paragraph{Modality invariance (AV correspondence).}

The representation must be invariant to the selected modality, so $c(T,T')$ is not affected by $m$ or $m'$.
Combined with sample distinctiveness, this means that the representation must be able to identify the same video from either the visual or audio components.
Stated differently, the representation must be able to put in correspondence visual and audio tracks from the same video.

\paragraph{Augmentation invariance.}

The representation should be invariant to data augmentation.
Hence $c(T,T')$ is not affected by $t$ or $t'$.

\paragraph{Time shift invariance/distinctiveness (synchronization).}

The representation might be either invariant or distinctive to a temporal shift.
The latter, captured by $\tau \not= \tau' \Rightarrow c(T,T')=0$, means that the representation can tell if two clips from the same video are synchronized or not.
Combined with modality invariance, this also means deciding if the visual and audio components are in sync.

\paragraph{Time reversal invariance/distinctiveness (arrow of time).}

Similar to before, in order to train a representation sensitive to time reversal, we set $r \not= r' \Rightarrow c(T,T')=0$.

Distinctiveness to the arrow of time~\citep{wei2018learning} and synchronization~\citep{avts,owens2018audio,arandjelovic2018objects} were explored before, albeit in a different setup that requires either a binary classifier or a curriculum; furthermore, here we also test whether invariance to either effects is preferable to distinctivenesses as a learning cue.

{\color{red} motivation: need to also explain how our formulation can encode for combination of hypotheses and why the GDT formation is advantageous / key}

{\color{red} need to also explain how our formulation can encompass other papers: 3D Rotnet, Jigsaw, Sync, AVC, in a table -> extensibility}

{\color{red} also need to concretize notation to hypothesis table}

\section{Multi-modal self-supervision}

We apply our framework to multi-modal self-supervision where the data $x$ are \emph{videos}.
We learn representations using invariance or distinctiveness to several types of transformations, with each setting corresponding to a different \textit{learning hypothesis}.
This requires to decide how transformations $T$ are sampled in the contrastive loss~\cref{e:contrastive} and which transformation pairs $c(T,T')$ are considered positive or negative, thus leading to different invariance/distinctiveness requirements.

\subsection{Sampling transformation}

First, we discuss how transformations are sampled.
In order for the batch to contain a mix of positive and negative transformation pairs, we sample them in pairs.
Specifically, we start by sampling $K$ generalized transformations $T_1,\dots,T_m$ i.i.d.~at random.
Then, for each $T_m$, we randomly sample a second transformation $T_m' | T_m$ condition on the first.
This second, related transformation $T_m'$ does \emph{not} necessarily constitute a positive pairing with $T_m$; instead, we will choose $c(T_m,T_m')=1$ for invariance or $c(T_m,T_m')=0$ for distinctiveness.

In more detail, let the pair of transformations be the tuples $T_m= A_k \circ H_k$ and we will focus on formulating different choices of $H_k = (i,\tau,m,t,r)$ and $H_k'=(i',\tau',m',r')$ constructed as follows.

\paragraph{Sample selection.}
$H_k$ selects first a random video $x_i$ from the dataset $D$.
The paired transformation $H'_k$ always selects the same sample $i'=i$.\footnote{While we do not explore this case here, it is meaningful to also consider pairs where $i'\not=i$ --- this could be used, for example, to test whether two different images are rotated by different amounts, similar to RotNet.}

\paragraph{Temporal clipping.}
After selecting a video, $H_k$ extracts a 1s clip $x_{i\tau}$ from it, where the the starting time $\tau$ is selected uniformly at random.
$H'_k$ then picks either the same start time $\tau=\tau'$ or another uniformly randomly start time. % $\tau' \sim \mathcal{N}(\tau,\sigma^2)$.

\paragraph{Modality slicing.}
Next, $H_k$ slices a modality $m(x_{i\tau})$ at random, where $m\in\mathcal{M}$ extracts either the visual $v_{i\tau}$ or the audio $a_{i\tau}$ component from the video, as explained before.
$H'_k$ either samples a modality $m'$ independently of $m$, or always picks the opposite modality $m'\not =m$.

\paragraph{Augmentation and normalization.}
Following video selection, clipping and slicing, we apply a random augmentation.
For the visual component, $H_k$ extracts a fixed-size tensor $t(v_{i\tau})$ where $t$ picks a random spatial crop and resizes it to a fixed resolution.
For the audio component, $t(a_{i\tau})$ is a spectrogram representation of the audio signal followed by SpecAugment~\cite{Park_2019}.
The transformation $t'$ in $T'_k$ is sampled in the same way, independently of $t$.

\paragraph{Time reversal.}
Finally, $H_k$ applies a time reversal operator $r\in\mathcal{R}=\{r_0, r_1\}$, where $r_0$ is the identity (do nothing) and $r_1$ flips the time dimension of its input tensor.
The transformation $r'$ in $H'_k$ is sampled independently.

\subsection{Learning hypotheses}
\begin{figure}[!tb]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/GDT_template.pdf}
    \caption{\textbf{The GDT loss template.}
    xxx.
    }\label{fig:template}
\end{figure}

Next, we describe the learning hypotheses explored in the paper.
These correspond to different definitions of the function $c(T,T')$, coding for invariance or distinctiveness to various transformations.
The function defaults to $c(T,T')=1$ (invariance), with the following modifications:

\paragraph{Sample distinctiveness.}

The representation must distinguish different videos, so that $i \not = i' \Rightarrow c(T,T')=0$.
This is the baseline on which the other hypotheses build upon.

\paragraph{Modality invariance (AV correspondence).}

The representation must be invariant to the selected modality, so $c(T,T')$ is not affected by $m$ or $m'$.
Combined with sample distinctiveness, this means that the representation must be able to identify the same video from either the visual or audio components.
Stated differently, the representation must be able to put in correspondence visual and audio tracks from the same video.

\paragraph{Augmentation invariance.}

The representation should be invariant to data augmentation.
Hence $c(T,T')$ is not affected by $t$ or $t'$.

\paragraph{Time shift invariance/distinctiveness (synchronization).}

The representation might be either invariant or distinctive to a temporal shift.
The latter, captured by $\tau \not= \tau' \Rightarrow c(T,T')=0$, means that the representation can tell if two clips from the same video are synchronized or not.
Combined with modality invariance, this also means deciding if the visual and audio components are in sync.

\paragraph{Time reversal invariance/distinctiveness (arrow of time).}

Similar to before, in order to train a representation sensitive to time reversal we set $r \not= r' \Rightarrow c(T,T')=0$.

Distinctiveness to the arrow of time~\citep{wei2018learning} and synchronization~\citep{avts,owens2018audio,arandjelovic2018objects} were explored before, albeit in a different setup that requires either a binary classifier or a curriculum; furthermore, here we also test whether invariance to either effects is preferable to distinctivenesses as a learning cue.

Another line of work in self-supervision uses multiple data modalities instead of using only images.
In this case, the task is to predict one modality from the other, such as predicting properties of the audio track in a video from images extracted from it~\citep{owens2016ambient}.
Cross-modal self-supervision is, in practice, also very powerful, although in these cases, data augmentations have been considered as useful but not key elements of the formulations.

In this paper, we argue that transformations are in fact \emph{central} to self-supervision.
% By this, we mean that the specific learning formulation, contrastive or not, is not as crucial.
We develop a clear framework for semantics preserving data augmentations for multi-modal training.
In particular, we view multi-modal training as a \emph{special case} of data transformation and thus, any recent method in self-supervised learning can be applied to this case without changes.

This can be explained succinctly as follows.
In self-supervision in the image domain, one starts from an image $x$ and generates a second, congruous image $t(x)$ by applying a nuisance transformation $t$ to $x$.
These transformations leave the semantic content mostly intact but can introduce noise as variance or make the task more difficult by masking parts of the inputs.
The goal is then to learn a representation $\Phi$ which is approximately invariant to $t$,
i.e.~$\Phi(x) \approx \Phi(t(x))$.
The latter must be paired with a constraint that the representation should also be distinctive, i.e.~$\Phi(x)\not=\Phi(x')$ if $x$ and $x'$ are different images.

In multi-modal learning, one starts instead from composite data $z=(a,v)$.
For example, $a$ could be the audio stream and $v$ the video stream in a video.
Then, instead of directly learning to predict the audio $a$ from the video $v$ (or vice-versa), which is an ill-posed problem, one might instead wish to learn  a pair of representations $\Phi_\mathrm{a}(a) \approx \Phi_\mathrm{v}(v)$, one for each stream.
In this case, distinctiveness means that  $\Phi_\mathrm{a}(a) \not= \Phi_\mathrm{v}(v')$ if $(a,v)\not=(a',v')$ are two different videos.

It is then easy to combine these two approaches under the same formulation as shown in Figure~\ref{fig:splash}.
The first step is to consider transformations $t(x)$ applied to the composite data.
These \emph{generalized transformations} play two roles: (a) to \emph{slice} (selecting \emph{which} modality to observe) and (b) to \emph{augment} (applying a random perturbation to the modality) the data.
The second step is to consider a representation $\Phi$ that can take as input any modality.
This is trivially achieved by considering a pair of networks $\Phi =(\Phi_\mathrm{a},\Phi_\mathrm{v})$ as before, with the convention that $\Phi(t(x))$ amounts to running either $\Phi_\mathrm{a}$ or $\Phi_\mathrm{v}$ depending on which modality is sliced by $t$.

Since transformations on videos can be applied in the time dimension as well, this results in a \emph{combinatorial} space of possible transformations that can be used to slice and augment multi-modal data.
A second contribution of the paper is to study this space, demonstrating the power of searching for better sets of transformations.
We show empirically the power of these intuitions by building them into MoCo~\citep{he2019momentum}, an off-the-shelf self-supervised method for learning from static images, extending it to a state-of-the-art method for learning from multi-modal data.

\subsection{Semantic video augmentations \label{sec:transforms}}
\begin{figure}[!tb]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/aug.pdf}
    \caption{\textbf{GDT augmentation space for videos.} For visual clips, we apply cropping, flipping and temporal jittering. 
    For auditory clips, we use SpecAugment~\cite{Park_2019} along with temporal jittering. 
    In addition, both clips can be independently sampled yielding asynchronization.}
    \label{fig:transformation}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%% 
\paragraph{Implementation.}
For learning robust representations, the applied within-modal augmentations are shown in Figure~\ref{fig:transformation}. 

For $\mathcal{A}_\mathrm{a}$, the audio-level augmentations, we use one second clips using log mel bank features with 40 MEL filters and 99 audio frames and apply SpecAugment~\citep{Park_2019}.

The visual augmentations $\mathcal{A}_\mathrm{v}$ are borrowed from~\citep{avts} and consist of first sampling one second of video at the original frame rate, applying a resizing to $(128\times171)$, random cropping to $(112\times112)$ and random horizontal flipping. 
For both modalities, we explore the effect of sampling clips from the source videos at different times each epoch, which we refer to as temporal jittering. 
We show examples of how these transformations affect the input in Figure~\ref{fig:transformation}.

\subsection{Generalized Data Transformations}
%While previous works have utilized hand-crafted losses for videos such as colorization~\citep{vondrick2018tracking} or detecting rotations in clips~\citep{jing2018self}, we apply a contrastive loss function, which has recently been shown to yield good performance for images and videos~\citep{sohn2016improved,he2019momentum,Wu_2018_CVPR,oord2018representation,Chen2020ASF,miech2019endtoend,han2019video,sun2019contrastive,li2020learning} without the need to implicitly specify what information needs to be discarded via a designed task.

For training our network in a self-supervised manner, we utilize the above semantics preserving video augmentations and combine them with various other task-specific transforms $\mathcal{T}$, which we will call \textit{learning hypotheses}. 
Each hypothesis constitutes a prior on what the network should learn via specifying desirable invariances or variances.
As such, they can encode previously proposed pretext tasks and we select a subset of those to include in our framework:
\begin{itemize}
   \item  Audio-Visual correspondence: this is our basecase and the transformation is the identity function, $\mathcal{T}(z)=z$, where $z$ is the audio or video input.
   \item  (In)Variance to temporal synchronization. The transformation asynchronizes the input: $\mathcal{T}(z(t_n))= z(t_m), t_m\neq t_n$.
   \item  (In)Variance to the arrow of time. The transformation reverses the arrow of time. $\mathcal{T}(\vec{z})=\cev{z}$, where $\cev{z}$ represents the reversing of the frames for visual input and the left-right flipping of the spectrogram for audio.
\end{itemize}
Note that we do not only choose the hypotheses chosen in previous works (variant to arrow of time ~\citep{wei2018learning}, variant to synchronization ~\citep{avts, owens2018audio}), but also their reversals to investigate the performance when treating these task-specific transforms as semantics preserving augmentations.

For each of these hypotheses, applying them as a desired variance requires treating them differently than the augmentations described in Sec~\ref{sec:transforms}.
While the papers that have proposed these tasks use binary classifiers~\citep{wei2018learning,arandjelovic17look, owens2018audio} or margin constrastive losses~\cite{avts}, we accommodate these various hypotheses in a noise contrastive loss formulation~\citep{gutmann2010noise, Wu_2018_CVPR,tian2019contrastive,Chen2020ASF,he2019momentum,misra2019selfsupervised,henaff2019data,hjelm2018learning} by specifying the positives and the negatives accordingly, as shown in Table~\ref{tab:hypotheses}.
\input{tabs/pos-neg}

\paragraph{Two sets of composed transforms.}
Given the within-modality augmentations $\mathcal{A}$, we construct two composed transformations:

First, the base set of augmented data can be defined as applying an operator 
\begin{align}
t_1 & =\mathcal{I} \circ \mathcal{M} \circ \mathcal{A}
\end{align}
on the dataset $D$,
where $\mathcal{I}$ selects a source video with a random index and $\mathcal{M}$ select the modality.
The second transformation $t_2$ can be used to define additional variances (e.g.~synchronization or arrow of time) via task-specific transforms $\mathcal{T}$:
\begin{align}
t_2(t_1) & =\mathcal{I}(t_1) \circ \mathcal{M}(t_1) \circ \mathcal{A} \circ \mathcal{T}(t_1)
\end{align}
and is dependent on the first operation.

\paragraph{Loss.}
Given a network~$\Phi$, a positive pair for the noise contrastive loss is thus given by 
\begin{align}
\textit{pos} &= (\Phi(t_1) , \Phi(t_{i}))(D),
\end{align}
with $i=1$ for inducing the various invariance hypotheses, and $i=2$ for inducing variance.
The negatives are given by the batch (of size 1024) as well as the examples of $t_2$ which are used for variance. 
We do not use a memory bank~\citep{tian2019contrastive,Wu_2018_CVPR} or another momentum network~\citep{he2019momentum} to reduce memory footprint, as we have not observed it to yield noticable gains.

By denoting the positive example of datapoint $x$ as $x'$, and the task-specific negatives by $\textit{neg}(x)$, the loss is given by
\begin{align}
\label{eq:loss}
    L(x,x')  =& 
          \log \frac{\exp(\langle \Phi(x),\Phi(x') \rangle_\tau)}
    {\exp(\langle \Phi(x),\Phi(x') \rangle_\tau)
          + \sum_{y \in \mathcal{B} + \{\textit{neg(x)}\}}\exp(\langle \Phi(x) ,\Phi(y) \rangle_\tau)},
\end{align}
 where $\langle \cdot,\!\cdot \rangle_\tau$ is the dot product of the L2-normalized embeddings multiplied by $\tau$, a temperature parameter for the cross entropy loss, as in~\citep{he2019momentum,Chen2020ASF}.
 The final loss is given by the sum of $L(x,x')$ and $L(x',x)$ and computed across all positive pairs with all $N$ noise samples for each datapoint $x$ in the batch.

\paragraph{Learning invariance gradually.}
By writing the negative gradient of this loss with regards to the sample's embedding $\Phi(x)$, \ie~the direction of a step of SGD, as done in~\citep{Chen2020ASF},
{\color{red} redo with final loss formulation}
\begin{align}
    -\nabla_{\Phi(x)} L(x) \propto 
         \Phi_(x')(1-\exp(2\langle \Phi(x),\Phi(x') \rangle_\tau)) 
          - \sum_{\alpha=1}^{N}\Phi_{jx'}\exp(\langle \Phi_{ix} ,\Phi_{jx'} \rangle_\tau)~,
\end{align}
we find that the gradient automatically reweights examples by assigning a smaller gradient to easy pairs (i.e., $\langle \Phi_{ix}, \Phi_{jx} \rangle \approx 1$) and a larger gradient to more difficult pairs.
Because we use a large augmentation space that subsumes both weaker as well as stronger transformations, our method generates a curriculum implicitly:
it will first learn to associate the easy pairs and then it will learn the more difficult pairs (\ie~heavily augmented). We confirm this hypothesis in Section~\ref{sec:curr}.

As shown in~\citep{oord2018representation,tian2019contrastive}, the negative noise  contrastive loss represents a lower bound on the mutual information between the two inputs $\Phi(x)$ and $\Phi(x')$. 
With our similarities always computed across modes, minimizing the loss thus leads to increasing (a lower bound on) the mutual information between the individually augmented modalities -- \emph{i.e.} capturing the common semantics. 
However, optimizing an estimate of the mutual information is not a necessary condition for good representations~\citep{tschannen2020on}.

==> GDT (ICCV 2021)/tabs/_HT100GDT.tex <==
\centering
% \footnotesize
% \setlength{\tabcolsep}{1.5pt}
    % \caption{\textbf{GDT on HT100M.}
    \label{tab:queryd-av}
      \begin{tabular}{ccccc  c}
      \toprule
        & DS & TR & TS & Mod. & \textbf{Acc} \\ %& $\mathbf{R@1}$ \\
        \midrule
        \multicolumn{6}{l}{\textit{SimCLR-like}} \\
        (a) & \vv & \cc & \cc  & V & $36.1$ \\ %& $5.2$ \\
        \midrule
         \multicolumn{6}{l}{\textit{Video-text cross-modal}} \\
        (b) & \vv & \cc & \cc  & VT  & $59.2$ \\ %& $6.3$ \\
        (c) & \vv & \vv & \cc  & VT  & $61.5$  \\ %& $9.9$ \\
        (d) & \vv & \cc & \vv  & VT  & $62.9$  \\ %& $7.9$ \\
        (e) & \vv & \vv & \ii  & VT  & $63.8$    \\ %& $XX$ \\ 
        (f) & \vv & \ii & \vv  & VT  & $\bf{64.4}$    \\ %& $XX$ \\
        (g) & \vv & \vv & \vv  & VT  & $\bf{64.4}$    \\ %& $XX$ \\ 
        \bottomrule
    \end{tabular}


==> GDT (ICCV 2021)/tabs/_abl-negs.tex <==

\setlength{\tabcolsep}{3pt}
\caption{\textbf{Number of negatives.}}
   \centering
  \footnotesize
  \begin{tabular}{l c c @{\hskip 5pt} c c}% c}
  \toprule
     \textbf{\#Negs} &  \multicolumn{2}{c}{\textbf{UCF}} & \multicolumn{2}{c}{\textbf{HMDB}} \\
    % &  50 & 100 & 50 & 100 \\
    Epochs & 50 & 100  & 50 & 100  \\
    \midrule 
        32  & $83.9$ & $\ul{87.1}$ & $\ul{52.1}$ & $53.8$  \\
        1024  & $\ul{84.8}$ & $86.5$ & $51.5$ & $\ul{55.6}$ \\ 
    \bottomrule
  \end{tabular}
  \vspace{5pt}
  \label{tab:ablation:temp}

==> GDT (ICCV 2021)/tabs/_abl-tau.tex <==

\setlength{\tabcolsep}{3pt}
\caption{\textbf{Tau, \textbf{$\tau$}.}}
  \centering
  \footnotesize
  \begin{tabular}{l c c @{\hskip 5pt} c c}
  \toprule
      \textbf{Tau} & \multicolumn{2}{c}{\textbf{UCF}} & \multicolumn{2}{c}{\textbf{HMDB}} \\
    % & 50 & 100  & 50 & 100  \\
    Epochs & 50 & 100  & 50 & 100  \\
    \midrule %\midrule
    % {50: 42.68, 100: 44.39, 150: 44.79, 200: 43.14}
          $0.2^{-1}$  & $84.4$ & $85.8$ & $51.2$ & $53.7$  \\
          $0.07^{-1}$ & $\ul{84.8}$ & $\ul{86.5}$ & $\ul{51.5}$ & $\ul{55.6}$   \\
          % seed = epoch % 5 variant ?
    \bottomrule
  \end{tabular}
  \vspace{5pt}
  \label{tab:ablation:tau}

==> GDT (ICCV 2021)/tabs/_audio-results.tex <==
%\begin{table}[t]
\footnotesize
%\scriptsize
\setlength{\tabcolsep}{1pt}
\captionof{table}{\textbf{Audio classification.} 
Downstream task accuracies on standard audio classification  benchmarks. For ESC-50 and DCASE2014, we report top-1 accuracy. 
%Methods with $^*$ use full-finetuning of their encoder network. %, $\star$ is concurrent. 
\label{tab:audio}}
% \vspace{.5em}
\begin{tabular}{l c cc} 
\toprule
\textbf{Method}    \\
                                 & \textbf{Data} & \textbf{DCASE}  & \textbf{ESC-50 } \\
\midrule
Human \citep{esc50}                     & --      & 81.3  \\
Supervised \citep{VGGSound}             & --      & --    \\
\midrule
ConvRBM \citep{sailor2017}          & None    & --      & 86.5 \\
AVTS \citep{avts}                 & K-400      & 91      & 76.7 \\
% DMC \citep{hu2018deep}            & K-400      & --      & 82.6 \\
XDC \cite{alwassel2019self}       & K-400      & --      & 78.5 \\
AVID \citep{morgado2020avid}      & K-400      &\ul{93}  &\bf{79.1} \\
\midrule
\textbf{GDT} (ours)               & K-400      &\bf{XX}  &\ul{XX}\\
\bottomrule
\end{tabular} 
%\end{table}

% %\begin{table}[t]
% \footnotesize
% %\scriptsize
% \setlength{\tabcolsep}{1pt}
% \captionof{table}{\textbf{Audio classification.} 
% Downstream task accuracies on standard audio classification  benchmarks. For ESC-50 and DCASE2014, we report top-1 accuracy and for VGG-Sound, mAP. 
% %Methods with $^*$ use full-finetuning of their encoder network. %, $\star$ is concurrent. 
% \label{tab:audio}}
% % \vspace{.5em}
% \begin{tabular}{l ccc} 
% \toprule
% \textbf{Method}    \\
%                                           & \textbf{DCASE}  & \textbf{ESC-50 }& \textbf{VGG-S}\\
% \midrule
% Human \citep{esc50}                     & --      & 81.3 & -- \\
% Supervised \citep{VGGSound}             & --      & --       & \ul{51.6}     \\
% \midrule
% %Autoencoder \citep{aytar2016soundnet} & - &   39.9         \\
% %Random Forest \citep{esc50}           & - &   44.3         \\
% %Piczak ConvNet \citep{Piczak2015}     & - &   64.5       \\
% %RNH \citep{rnh2013}                   &72 & -                  \\
% %Ensemble \citep{stowell2015}          &77 &   -                \\
% ConvRBM \citep{sailor2017}               &--        & 86.5   & --      \\
% %SoundNet \citep{aytar2016soundnet}      &88       & 74.2          \\
% %L3-Net \citep{arandjelovic17look}       &93       & 79.3          \\
% AVTS \citep{avts}                        &94       & 82.3   & --       \\
% DMC \citep{hu2018deep}                  &--       & 82.6   & --       \\
% XDC \cite{alwassel2019self}             &95       & 84.8   & --       \\
% AVID \citep{morgado2020avid}            &\ul{96}  &\bf{89.2}  & --    \\
% \midrule
% \textbf{GDT} (ours)                    &\bf{98}  &\ul{88.5}     & \bf{54.8}  \\
% \bottomrule
% \end{tabular} 
% %\end{table}

==> GDT (ICCV 2021)/tabs/_retrieval_and_fewshot.tex <==
% \setlength{\tabcolsep}{2pt}
\centering
%  \scriptsize
\midsepremove
% \footnotesize
\caption{\textbf{Video retrieval and Few Shot Learning.} Retrieval accuracy in (\%) via nearest neighbors at various levels of neighborhood sizes and few shot learning accuracy (\%) via  a $k$-nearest neighbor on frozen representations. \label{tab:few-shot-ret} }
\vspace{1mm}
\begin{tabular}{c l c c @{\hskip 7pt} c c}
\toprule
& & \multicolumn{2}{c}{\textbf{HMDB}} & \multicolumn{2}{c}{\textbf{UCF}} \\
& & 1 & 5 & 1 & 5   \\
\midrule
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textit{kNN}}}}  
&\hphantom{x} Random  & 3.0  & 3.5  & 2.3  & 4.6     \\
&\hphantom{x}  3DRot~\citep{jing2018self} & -- & --   & 15.0 & 31.5  \\
\cmidrule{2-6}
& \hphantom{x} \textbf{GDT (ours)} & \bf{14.3} & \bf{15.4}  & \bf{26.7} & \bf{44.6}  \\
\midrule
&\hphantom{x} SP-Net~\citep{benaim2020speednet}                 & - & - & 13.0 & 28.1   \\
% &\hphantom{x} VCOP~\citep{clip_order}                    & 7.6 & 22.9  & 14.1 & 30.3 \\
&\hphantom{x} VCP~\citep{luo2020video}                   & 7.6 & 24.4 & 18.6 & 33.6 \\
&\hphantom{x} M-DPC~\citep{Han_2020}                             & 7.7 & 25.7 & 20.2 & 40.4 \\
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textit{Retrieval}}}}&\hphantom{x} 
VSP~\citep{cho2020selfsupervised}                   & 10.3 & 26.6 & 24.6 & 41.9 \\
&\hphantom{x} CoCLR~\citep{Han2020SelfsupervisedCF}               & 23.2 & 43.2 & 53.3 & 69.4   \\
&\hphantom{x} SeLaVi~\citep{asano2020labelling}                   & 24.8 & 47.6 & 52.0 & 68.6    \\
\cmidrule{2-6}
&\hphantom{x} \textbf{GDT (ours)} & \textbf{26.1} & \textbf{51.7} & \textbf{62.8} & \textbf{79.0}  \\
\bottomrule
\end{tabular}
\midsepdefault

% \setlength{\tabcolsep}{2pt}
% \centering
% %  \scriptsize
% \footnotesize
% \caption{\textbf{Video retrieval and Few Shot Learning.} Retrieval accuracy in (\%) via nearest neighbors at various levels of neighborhood sizes and few shot learning accuracy (\%) via training a $k$-nearest neighbor classifier on fixed representations. \label{tab:few-shot-ret} }
% \vspace{1mm}
% \begin{tabular}{c l c c c @{\hskip 5pt} c c c}
% \toprule
% & & \multicolumn{3}{c}{\textbf{HMDB}} & \multicolumn{3}{c}{\textbf{UCF}} \\
% & & 1 & 5  & 20 & 1 & 5 & 20   \\
% \midrule
% \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textit{Few-shot}}}}  
% &\hphantom{x} Random  & 3.0  & 3.5   & 4.5  & 2.3  & 4.6  & 6.8    \\
% &\hphantom{x}  3DRot~\citep{jing2018self} & -- & -- & --   & 15.0 & 31.5  & 47.1  \\
% \cmidrule{2-8}
% & \hphantom{x} \textbf{GDT (ours)} & \bf{14.3} & \bf{15.4}  & \bf{24.7}  & \bf{26.7} & \bf{44.6}   & \bf{57.4}  \\
% \midrule
% \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textit{Retrieval}}}}&\hphantom{x}
% SP-Net~\citep{benaim2020speednet}                 & - & - & - & 13.0 & 28.1 & 49.5    \\
% &\hphantom{x} VCOP~\citep{clip_order}                                      & 7.6 & 22.9 & 48.8  & 14.1 & 30.3 & 51.1   \\
% &\hphantom{x} VCP~\citep{cho2020selfsupervised}                   & 7.6 & 24.4 & 53.6 & 18.6 & 33.6 & 53.5    \\
% &\hphantom{x} M-DPC~\citep{Han_2020}                             & 7.7 & 25.7 & 57.7 & 20.2 & 40.4 & 64.7    \\
% &\hphantom{x} VSP~\citep{cho2020selfsupervised}                   & 10.3 & 26.6 & 54.6 & 24.6 & 41.9 & 76.9    \\
% &\hphantom{x} CoCLR~\citep{Han2020SelfsupervisedCF}               & 23.2 & 43.2 & 65.5 & 53.3 & 69.4 & 82.0    \\
% &\hphantom{x} SeLaVi~\citep{asano2020labelling}                   & 24.8 & 47.6 & 75.5 & 52.0 & 68.6 & 84.5    \\
% % &\hphantom{x} CoCLR~\citep{Han2020SelfsupervisedCF}               & 26.1 & 45.8 & 69.7 & 55.9 & 70.8 & 82.5    \\
% \cmidrule{2-8}
% &\hphantom{x} \textbf{GDT (ours)} & \textbf{26.1} & \textbf{51.7} & \textbf{75.1} & \textbf{62.8} & \textbf{79.0}  & \textbf{90.4}  \\
% \bottomrule
% \end{tabular}


==> GDT (ICCV 2021)/tabs/appx-ablations.tex <==
\begin{table*}[b]
\caption{\textbf{NCE loss computation parameters.} Top-1 accuracies (as \%) on downstream video classification tasks are shown after $50$ and $100$ epochs of pretext training.}\label{tab:ablation-appx}
\centering
	\begin{subtable}[b]{.33\linewidth}\centering
		{\input{tabs/_abl-tau}}	
	\end{subtable}
	\qquad
	\begin{subtable}[b]{.33\linewidth}\centering
		{\input{tabs/_abl-negs}}	
	\end{subtable}
\end{table*}

==> GDT (ICCV 2021)/tabs/appx-retrieval.tex <==
 \begin{table}[htb]
\setlength{\tabcolsep}{3pt}
\centering
\caption{\textbf{Full retrieval table.}\label{tab:ret-full}}
  \centering
  \footnotesize
  \begin{tabular}{l c c c c c @{\hskip 5pt} c c c c c}
  \toprule
      & \multicolumn{5}{c}{\textbf{HMDB}} & \multicolumn{5}{c}{\textbf{UCF}} \\
      \cmidrule(lr){2-6} \cmidrule(lr){7-11} \multicolumn{1}{r}{Recall @} & 1 & 5  & 10 & 20 & 50 & 1 & 5 & 10 & 20 & 50  \\
    \midrule %\midrule
    Supervised (Kinetics) & 49.1 & 74.4 & 83.9 & 90.6 & 96.4 & 86.9 & 94.6 & 96.5 & 98.1 & 99.0 \\
    \midrule 
    ST-Puzzle~\citep{kim2019self}             & -- & -- & -- & -- & -- & 19.7 & 28.5 & 33.5 & 40.0 & 49.4 \\
    OPN~\citep{lee2017unsupervised}           & -- & -- & -- & -- & -- & 19.9 & 28.7 & 34.0 & 40.6 & 51.6  \\
    ST Order ~\citep{buchler2018improving}    & -- & -- & -- & -- & -- & 25.7 & 36.2 & 42.2 & 49.2 & 59.5  \\
    ClipOrder~\citep{clip_order}              & 7.6 & 22.9 & 34.4 & 48.8 & 68.9 & 14.1 & 30.3 & 40.4 & 51.1 & 66.5  \\
    SpeedNet~\citep{benaim2020speednet}        & -- & -- & -- & -- & -- & 13.0 & 28.1 & 37.5 & 49.5 & 65.0  \\
    VCP~\citep{luo2020video}                  & 7.6 & 24.4 & 36.3 & 53.6 & 76.4 & 18.6 & 33.6 & 42.5 & 53.5 & 68.1  \\
    VSP~\citep{cho2020selfsupervised}         & 10.3 & 26.6 & 38.8& 54.6 & 76.8 & 24.6 & 41.9 & 51.3 & 62.7 &76.9   \\
    \midrule
    \textbf{GDT (Kinetics)} &\textbf{25.4} & \textbf{51.4} &\textbf{63.9} & \textbf{75.0} & \textbf{87.8} & \textbf{57.4} & \textbf{73.4} & \textbf{80.8} & \textbf{88.1}  & \textbf{92.9} 
     \\
    \textbf{GDT (VGG-Sound)} & \textbf{28.4} & \textbf{55.1} & \textbf{67.2} & \textbf{79.3}  & \textbf{91.1} 
    &\textbf{63.4} & \textbf{79.6} &\textbf{85.0} & \textbf{90.1} & \textbf{95.2} \\
    \textbf{GDT (Audioset)} & \textbf{30.6} & \textbf{58.0} & \textbf{69.8} & \textbf{79.9}  & \textbf{91.0} 
    &\textbf{65.9} & \textbf{82.6} &\textbf{88.2} & \textbf{92.2} & \textbf{96.6} \\
    \textbf{GDT (IG65M)} & \textbf{36.1} & \textbf{61.1} & \textbf{70.8} & \textbf{79.7}  & \textbf{92.1} 
    &\textbf{75.7} & \textbf{87.2} &\textbf{90.7} & \textbf{93.5} & \textbf{96.6} \\
    \bottomrule
  \end{tabular}
  \vspace{5pt}

 \end{table}

==> GDT (ICCV 2021)/tabs/appx-video-full-finetune.tex <==
\begin{table*}[!ht]
    \small
	\centering
	\caption{\textbf{State-of-the-art on action recognition.}
	Self-supervised and supervised methods on UCF101 and HMDB51 benchmarks.
	We follow the standard protocol and report the average top-1 accuracy over the official splits and show results for finetuning the whole network.
	Note that we find the supervised baseline to be around $6\%$ and $2\%$ better than reported in \citep{alwassel2019self} as we use a different finetuning strategy. 
	Methods with $^\dagger$ indicate the additional use of video titles as supervision.
	Methods with $^*$ use ASR generated text.
	Methods in {\color{gray} gray}  are concurrent works.
	\dontshowthisinappendix{See \cref{supp:tab:sota} in the Appendix for a full version of this table.}
	\labelswitch{tab:sota}}
	\tabcolsep=0.09cm
	\begin{tabular}{l l l @{\hskip 0.2in} c c }
		\toprule
		%\multicolumn{3}{c|}{\underline{Pretraining}} & \multicolumn{4}{c}{\underline{Evaluation}} \\
		\textbf{Method}                              & \textbf{Architecture} & \bf{Pretrain Dataset}  & %\multicolumn{2}{c}{\underline{\textbf{ft. last}}}
		\multicolumn{2}{c}{\textbf{Top-1 Acc\%}} \\
		                                             &                       &                           & HMDB\,        & UCF          \\
		\midrule 
		Full supervision                             & R(2+1)D-18            & ImageNet                  & 46.7          & 82.8         \\ 
		Full supervision~\citep{alwassel2019self}    & R(2+1)D-18            & Kinetics-400              & 65.1          & 94.2         \\   
		Full supervision (ours)                      & R(2+1)D-18            & Kinetics-400              & 70.4          & 95.0         \\
		 
		Full supervision~\citep{tran2018closer}      & R(2+1)D-34            & Kinetics-400              & 74.5          & 96.8         \\   
		\midrule 
		\textit{Using UCF}  \\ 
		Shuffle and Learn~\citep{misra2016shuffle}   & CaffeNet              & UCF                       & 18.1          & 50.2         \\   
		VGAN~\citep{vondrick2016generating}          & VGAN                  & Flickr                    & --            & 52.1         \\   
		LT-Motion~\citep{Luo_2017}                   & VGG-16                & UCF                       & --            & 53.0         \\   
		Geometry~\citep{gan2018geometry}             & CaffeNet              & UCF                       & 23.3          & 55.1         \\   
		OPN~\citep{lee2017unsupervised}              & VGG                   & UCF                       & 23.8          & 56.3         \\   
		ST Order ~\citep{buchler2018improving}       & CaffeNet              & UCF                       & 25.0          & 58.6         \\   
		CMC~\citep{tian2019contrastive}              & CaffeNet              & UCF                       & 26.7          & 59.1         \\   
		VCP~\citep{luo2020video}                     & R(2+1)D-18            & UCF                       & 32.2          & 66.3         \\   
		Cross and Learn ~\citep{Sayed_2019}          & VGG-16                & UCF                       & 33.0          & 70.5         \\   
		\midrule
		\textit{Using Kinetics}  \\
		ClipOrder~\citep{clip_order}                 & R(2+1)D-18            & Kinetics-400              & 30.9          & 72.4         \\  
        MotionPred~\citep{motion_statistics}         & C3D                   & Kinetics-400              & 33.4          & 61.2         \\    
		RotNet3D~\citep{jing2018self}                & 3D-ResNet18           & Kinetics-600              & 33.7          & 62.9         \\  
		ST-Puzzle~\citep{kim2019self}                & 3D-ResNet18           & Kinetics-400              & 33.7          & 65.8         \\  
		DPC~\citep{han2019video}                     & 3D-ResNet34           & Kinetics-400              & 35.7          & 75.7         \\  
		VPS~\citep{cho2020selfsupervised}            & R3D                   & Kinetics-400              & 36.8          & 74.8         \\  
		SpeedNet~\citep{benaim2020speednet}          & I3D                   & Kinetics-400              & 43.7          & 66.7         \\  
		AoT~\citep{wei2018learning}                  & T-CAM                 & Kinetics-400              & -             & 79.4         \\  
		CBT~\citep{sun2019contrastive}               & S3D                   & Kinetics-600              & 44.6          & 79.5         \\  
		Multisensory~\citep{owens2018audio}          & 3D-ResNet18           & Kinetics-400              & -             & 82.1         \\  
		XDC~\citep{alwassel2019self}                 & R(2+1)D-18            & Kinetics-400              & 52.6          & 86.8         \\  
		AV Sync+RotNet~\citep{xiao2020audiovisual}   & AVSlowFast            & Kinetics-400              & 54.6          & 87.0         \\  
		AVTS~\citep{avts}                            & MC3-18                & Kinetics-400              & 56.9          & 85.8         \\  
		CPD~\citep{li2020learning}$^{\dagger *}$     & 3D-Resnet50           & Kinetics-400              & 57.7          & 88.7         \\  
		AVID~\citep{morgado2020avid}                 & R(2+1)D-18            & Kinetics-400              & \ul{60.8}     & 87.5         \\
		{\color{gray}CoCLR~\citep{Han2020SelfsupervisedCF}}         & {\color{gray}S3D}         & {\color{gray}Kinetics-400}         & {\color{gray}\bf{62.9}}          & {\color{gray}\bf{90.6}}  \\
		\midrule
		\bf{\methodname~(ours)}                      & R(2+1)D-18            & Kinetics-400              & {60.0}    & \ul{89.3}     \\
		 \midrule
		% OTHER DATASETS
		 \textit{Using other datasets} \\
		 L$^3$-Net~\citep{Arandjelovic17}        & VGG-16                & AudioSet                  & 40.2          & 72.3         \\    
		 Speech2Action*~\citep{nagrani2020}          & S3D-G                 & MovieDataset              & 58.1          & -            \\    
		 DynamoNet~\citep{Diba_2019}                 & ResNext101            & Youtube8M                 & 58.6          & 87.3         \\    
		     
		 MIL-NCE~\citep{miech2019endtoend}*          & S3D                   & HowTo100M                 & 61.0          & 91.3         \\    
		 AVTS~\citep{avts}                           & MC3-18                & AudioSet                  & 61.6          & 89.0         \\
		 XDC~\citep{alwassel2019self}                & R(2+1)D-18            & AudioSet                  & 63.7          & \bf{93.0}         \\
		 AVID~\citep{morgado2020avid}                & R(2+1)D-18            & AudioSet                  & 64.7          & 91.5         \\
		 {\color{gray}MMV$^*$~\citep{alayrac2020selfsupervised}}     & {\color{gray}R(2+1)D-18} & {\color{gray}Audioset}                 & {\color{gray}\bf{70.1}} & {\color{gray}91.5}  \\
		 ELo~\citep{piergiovanni2020evolving}        & R(2+1)D-50x3          & Youtube-2M                & 67.4          & 93.8         \\   
		 XDC~\citep{alwassel2019self}                & R(2+1)D-18            & IG65M                     & 68.9          & \bf{95.5}         \\   
         {\color{gray}MMV$^*$~\citep{alayrac2020selfsupervised}}     & {\color{gray}TSM-50x2}   & {\color{gray}AudioSet+HT100M}  & {\color{gray}\bf{75.0}} & {\color{gray}\ul{95.2}}\\
		 \midrule       
		 \bf{\methodname~(ours)}                     & R(2+1)D-18            & VGGSound (170K)           & 61.9          & 89.4         \\   
		 \bf{\methodname~(ours)}                     & R(2+1)D-18            & AudioSet (1.7M)           & \ul{66.1}     & \ul{92.5}    \\   
		 \bf{\methodname~(ours)}                     & R(2+1)D-18            & IG65M                     & \ul{72.8}     & \ul{95.2}    \\   
		 \midrule
		 {\bf{\methodname~(ours)}}  (only finetune \texttt{fc}) & R(2+1)D-18    & IG65M                  & {55.1}     & {85.4}    \\   
		 %\bf{\methodname~(ours)}                     & R(2+1)D-34            & IG65M                     & \bf{xx}       & \bf{xx}      \\   
		\bottomrule       
	\end{tabular}
	\vspace{2mm}
\end{table*}

% \begin{table}[!h]
%     \small
% 	\centering
% 	\caption{\textbf{State-of-the-art on action recognition.}
% 	Self-supervised and supervised methods on UCF101 and HMDB51 benchmarks.
% 	We follow the standard protocol and report the average top-1 accuracy over the official splits and show results for finetuning the whole network.
% 	Note that we find the supervised baseline to be around $6\%$ and $2\%$ better than reported in \citep{alwassel2019self} as we use a different finetuning strategy. 
% 	Methods with $^\dagger$ indicate the additional use of video titles as supervision.
% 	Methods with $^*$ use ASR generated text.
% 	Methods in {\color{gray} gray}  are concurrent works.
% 	\dontshowthisinappendix{See \cref{supp:tab:sota} in the Appendix for a full version of this table.}
% 	\labelswitch{tab:sota}}
% 	\vspace{-0.5em}
% 	\tabcolsep=0.09cm
% 	\begin{tabular}{l l l @{\hskip 0.2in} c c }
% 		\toprule
% 		%\multicolumn{3}{c|}{\underline{Pretraining}} & \multicolumn{4}{c}{\underline{Evaluation}} \\
% 		\textbf{Method}                              & \textbf{Architecture} & \bf{Pretrain Dataset}  & %\multicolumn{2}{c}{\underline{\textbf{ft. last}}}
% 		\multicolumn{2}{c}{\textbf{Top-1 Acc\%}} \\
% 		                                             &                       &                           & HMDB\,        & UCF          \\
% 		\midrule 
% 		Full supervision                             & R(2+1)D-18            & ImageNet                  & 46.7          & 82.8         \\ 
% 		Full supervision~\citep{alwassel2019self}    & R(2+1)D-18            & Kinetics-400              & 65.1          & 94.2         \\   
% 		Full supervision (ours)                      & R(2+1)D-18            & Kinetics-400              & 70.4          & 95.0         \\
		 
% 		Full supervision~\citep{tran2018closer}      & R(2+1)D-34            & Kinetics-400              & 74.5          & 96.8         \\   
% 		\midrule 
% 		\textit{Using UCF}  \\ 
% 		Shuffle and Learn~\citep{misra2016shuffle}   & CaffeNet              & UCF                       & 18.1          & 50.2         \\   
% 		VGAN~\citep{vondrick2016generating}          & VGAN                  & Flickr                    & --            & 52.1         \\   
% 		LT-Motion~\citep{Luo_2017}                   & VGG-16                & UCF                       & --            & 53.0         \\   
% 		Geometry~\citep{gan2018geometry}             & CaffeNet              & UCF                       & 23.3          & 55.1         \\   
% 		OPN~\citep{lee2017unsupervised}              & VGG                   & UCF                       & 23.8          & 56.3         \\   
% 		ST Order ~\citep{buchler2018improving}       & CaffeNet              & UCF                       & 25.0          & 58.6         \\   
% 		CMC~\citep{tian2019contrastive}              & CaffeNet              & UCF                       & 26.7          & 59.1         \\   
% 		VCP~\citep{luo2020video}                     & R(2+1)D-18            & UCF                       & 32.2          & 66.3         \\   
% 		Cross and Learn ~\citep{Sayed_2019}          & VGG-16                & UCF                       & 33.0          & 70.5         \\   
% 		\midrule
% 		\textit{Using Kinetics}  \\
% 		ClipOrder~\citep{clip_order}                 & R(2+1)D-18            & Kinetics-400              & 30.9          & 72.4         \\  
%         MotionPred~\citep{motion_statistics}         & C3D                   & Kinetics-400              & 33.4          & 61.2         \\    
% 		RotNet3D~\citep{jing2018self}                & 3D-ResNet18           & Kinetics-600              & 33.7          & 62.9         \\  
% 		ST-Puzzle~\citep{kim2019self}                & 3D-ResNet18           & Kinetics-400              & 33.7          & 65.8         \\  
% 		DPC~\citep{han2019video}                     & 3D-ResNet34           & Kinetics-400              & 35.7          & 75.7         \\  
% 		VPS~\citep{cho2020selfsupervised}            & R3D                   & Kinetics-400              & 36.8          & 74.8         \\  
% 		SpeedNet~\citep{benaim2020speednet}          & I3D                   & Kinetics-400              & 43.7          & 66.7         \\  
% 		AoT~\citep{wei2018learning}                  & T-CAM                 & Kinetics-400              & -             & 79.4         \\  
% 		CBT~\citep{sun2019contrastive}               & S3D                   & Kinetics-600              & 44.6          & 79.5         \\  
% 		Multisensory~\citep{owens2018audio}          & 3D-ResNet18           & Kinetics-400              & -             & 82.1         \\  
% 		XDC~\citep{alwassel2019self}                 & R(2+1)D-18            & Kinetics-400              & 52.6          & 86.8         \\  
% 		AV Sync+RotNet~\citep{xiao2020audiovisual}   & AVSlowFast            & Kinetics-400              & 54.6          & 87.0         \\  
% 		AVTS~\citep{avts}                            & MC3-18                & Kinetics-400              & 56.9          & 85.8         \\  
% 		CPD~\citep{li2020learning}$^{\dagger *}$     & 3D-Resnet50           & Kinetics-400              & 57.7          & 88.7         \\  
% 		AVID~\citep{morgado2020avid}                 & R(2+1)D-18            & Kinetics-400              & \ul{60.8}     & 87.5         \\
% 		{\color{gray}CoCLR}~\citep{Han2020SelfsupervisedCF}         & S3D         & Kinetics-400         & \bf{62.9}          & \bf{90.6}  \\
% 		\midrule
% 		\bf{\methodname~(ours)}                      & R(2+1)D-18            & Kinetics-400              & {60.0}    & \ul{89.3}     \\
% 		 \midrule
% 		% OTHER DATASETS
% 		 \textit{Using other datasets} \\
% 		 L$^3$-Net~\citep{Arandjelovic17}        & VGG-16                & AudioSet                  & 40.2          & 72.3         \\    
% 		 Speech2Action*~\citep{nagrani2020}          & S3D-G                 & MovieDataset              & 58.1          & -            \\    
% 		 DynamoNet~\citep{Diba_2019}                 & ResNext101            & Youtube8M                 & 58.6          & 87.3         \\    
		     
% 		 MIL-NCE~\citep{miech2019endtoend}*          & S3D                   & HowTo100M                 & 61.0          & 91.3         \\    
% 		 AVTS~\citep{avts}                           & MC3-18                & AudioSet                  & 61.6          & 89.0         \\
% 		 XDC~\citep{alwassel2019self}                & R(2+1)D-18            & AudioSet                  & 63.7          & 93.0         \\
% 		 AVID~\citep{morgado2020avid}                & R(2+1)D-18            & AudioSet                  & 64.7          & 91.5         \\
% 		 {\color{gray}MMV}~\citep{alayrac2020selfsupervised}     & R(2+1)D-18 & Audioset                 & \bf{70.1} & 91.5  \\
% 		 ELo~\citep{piergiovanni2020evolving}        & R(2+1)D-50x3          & Youtube-2M                & 67.4          & 93.8         \\   
% 		 XDC~\citep{alwassel2019self}                & R(2+1)D-18            & IG65M                     & 68.9          & \bf{95.5}         \\   
%          {\color{gray}MMV}~\citep{alayrac2020selfsupervised}     & TSM-50x2   & AudioSet+HT100M  & \bf{75.0} & \ul{95.2}\\
% 		 \midrule       
% 		 \bf{\methodname~(ours)}                     & R(2+1)D-18            & VGGSound (170K)           & 61.9          & 89.4         \\   
% 		 \bf{\methodname~(ours)}                     & R(2+1)D-18            & AudioSet (1.7M)           & \ul{66.1}     & {92.5}    \\   
% 		 \bf{\methodname~(ours)}                     & R(2+1)D-18            & IG65M                     & \ul{72.8}     & \ul{95.2}    \\   
% 		 \midrule
% 		 {\bf{\methodname~(ours)}}  (only finetune \texttt{fc}) & R(2+1)D-18    & IG65M                  & {55.1}     & {85.4}    \\   
% 		 %\bf{\methodname~(ours)}                     & R(2+1)D-34            & IG65M                     & \bf{xx}       & \bf{xx}      \\   
% 		\bottomrule       
% 	\end{tabular}
% 	\vspace{2mm}
% \end{table}


==> GDT (ICCV 2021)/tabs/full-finetune-joined.tex <==
\centering
\begin{tabular}{l l @{\hskip 5pt} c c }
		\toprule
		%\multicolumn{3}{c|}{\underline{Pretraining}} & \multicolumn{4}{c}{\underline{Evaluation}} \\
		\textbf{Method}                              & \bf{Data}  & %\multicolumn{2}{c}{\underline{\textbf{ft. last}}}
		\multicolumn{2}{c}{\textbf{Top-1 Acc\%}} \\
		                                             &                           & HMDB\,        & UCF          \\
		\midrule 
% 		Full supervision                             & ImageNet                  & 46.7          & 82.8         \\         
      {\color{gray}Supervised~\citep{xie2018rethinking}} & {\color{gray}K-400+IN} & {\color{gray}75.9} & {\color{gray} 96.8} \\
		{\color{gray}Supervised~\citep{alwassel2019self}}    & {\color{gray}K-400}              & {\color{gray}65.1}          & {\color{gray}94.2}         \\   
 		% Supervised (ours)                      & K-400              & 70.4          & 95.0         \\
		\specialrule{.4pt}{1pt}{1pt} %\midrule
		%\textit{Using Kinetics}  \\
		AoT~\citep{wei2018learning}                  & K-400              & -             & 79.4         \\  
		MultiSensory~\citep{owens2018audio}          & K-400              & -             & 82.1         \\
		SeLaVi~\citep{asano2020labelling}            & K-400              & 47.1          & 84.2         \\  
		PEMT~\citep{lee2021parameter}                & K-400             & --             & 85.2         \\ 
		XDC~\citep{alwassel2019self}                 & K-400              & 52.6          & 86.8         \\  
		AV Sync+RotNet~\citep{xiao2020audiovisual}   & K-400              & 54.6          & 87.0         \\  
		CoCLR~\citep{Han2020SelfsupervisedCF}        & K-400              & 54.6         & 87.9\\
		SeCo~\citep{yao2021seco}                     & K-400              & 55.6          & 88.3         \\  
		AVTS~\citep{avts}                            & K-400              & 56.9          & 85.8         \\  
		CPD~\citep{li2020learning}                   & K-400              & 57.7          & 88.7        \\  
		AVID~\citep{morgado2020avid}                 & K-400              & 60.8          & 87.5         \\  
		CM-ACC~\citep{ma2021active}                  & K-400              &  61.8         & 90.2         \\
		GLCM~\citep{ma2021contrastive}               & K-400              &  61.9         & 91.2 \\
		% CoCLR~\citep{Han2020SelfsupervisedCF}        & K-400              & 62.9         & 90.6         \\  
		\bf{\methodname~(ours)}                      & K-400              & \bf{62.3}    & \bf{90.9}     \\
		 \specialrule{.4pt}{1pt}{1pt}
		 MIL-NCE~\citep{miech2019endtoend}         & HT100M                 & 61.0          & 91.3         \\
		 \bf{\methodname~(ours)}                    & HT100M            & \bf{67.4}     & \bf{94.1}    \\ 
		 \specialrule{.4pt}{1pt}{1pt}
		  XDC~\citep{alwassel2019self}                & IG65M                     & 68.9          & \bf{95.5}         \\  
		 \bf{\methodname~(ours)}                     & IG65M                     & \bf{72.8}     & \ul{95.2}    \\   
		% OTHER DATASETS
		 %\textit{Using other datasets} \\
% 		 L$^3$-Net~\citep{arandjelovic17look}        & AudioSet                  & 40.2          & 72.3         \\    
% 		 Speech2Action*~\citep{nagrani2020}          & MovieDataset              & 58.1          & -            \\    
% 		 DynamoNet~\citep{Diba_2019}                 & Youtube8M                 & 58.6          & 87.3         \\
        %\midrule
		 %AVTS~\citep{avts}                           & AS                  & 61.6          & 89.0         \\
		 %XDC~\citep{alwassel2019self}                & AS                  & 63.7          & \bf{93.0}         \\
		 %AVID~\citep{morgado2020avid}                & AS                  & 64.7          & 91.5         \\ 
		 %MMV~\citep{alayrac2020selfsupervised}       & AS                  & 70.1          & 91.5         \\ 
		 %\midrule
		 %\bf{\methodname~(ours)}                     & AS            & \bf{66.1}     & \ul{92.5}    \\   
		 % \midrule
		 %ELo~\citep{piergiovanni2020evolving}        & YT-2M                & 67.4          & 93.8         \\   
		 % XDC~\citep{alwassel2019self}                & IG65M                     & 68.9          & \bf{95.5}         \\   
% 		 \midrule   
		 % \specialrule{.4pt}{1pt}{1pt}
		 %\bf{\methodname~(ours)}                     & VGGS            & 61.9          & 89.4         \\  
		 %\bf{\methodname~(ours)}                     & IG65M                     & \bf{72.8}     & \ul{95.2}    \\   
		 %\bf{\methodname~(ours)}                     & IG65M                     & \bf{xx}       & \bf{xx}      \\   
		\bottomrule       
	\end{tabular}


==> GDT (ICCV 2021)/tabs/queryd.tex <==
\renewcommand\thesubtable{\Alph{subtable}}

\begin{table}[t] 
% \begin{wraptable}{r}{3.5cm}
% \vspace{-1em}
\centering
\caption{\textbf{GDT on video-text HT100M dataset}. We also find the positive effect of including more modalities and find non-trivial combinations of beneficial transformations previously unexplored.}\label{t:text}
	{\input{tabs/_HT100GDT}}
\end{table}
% \end{wraptable}

% for ICML:
% \begin{table}[t] 
% \vspace{-1em}
% \centering
% \caption{\textbf{GDT on video-text HT100M dataset}. We also find the positive effect of including more modalities and find non-trivial combinations of beneficial transformations previously unexplored.}\label{t:text}
% 	{\input{tabs/_HT100GDT}}
% \end{table}


==> GDT (ICCV 2021)/tabs/t1_abl_inv.tex <==
%------------------------------------------
\begin{wraptable}{r}{5.0cm} %\begin{table}
\vspace{-4.5mm}
\setlength{\tabcolsep}{3pt}
\centering
\footnotesize
\caption{Downstream action recognition results  for \textbf{different invariance ablations}.}\label{tab:ablation}
\vspace{-1mm}
\begin{tabular}{l c c c c @{\hskip 5pt} c c c c}
\toprule
 & \multicolumn{2}{c}{\textbf{HMDB}} & \multicolumn{2}{c}{\textbf{UCF}} \\
Epochs           & 50     & 100                & 50       & 100  \\
\midrule 
(a) Full          & \bf{55.1} & \bf{56.9}  & \bf{85.1} & \bf{87.9}  \\
\midrule 
(b) No $\tau$     & 32.8 & 34.8            & 74.0  & 76.2   \\
(c) No $g_v$      & 50.7 & 46.7            & 83.2  & 83.2  \\
(d) No $g_a$      & 51.5 & 55.6            & 84.8  & 86.5  \\
\bottomrule
\end{tabular}
\vspace{-18pt}
\end{wraptable} %\end{table}
%------------------------------------------

==> GDT (ICCV 2021)/tabs/t2_hypothesis-res.tex <==
\newcommand{\vv}{{\bf{d}}}%
\newcommand{\ii}{{\bf{i}}}%
\newcommand{\cc}{{$\cdot$}}%
\begin{table}
%\vspace{-0.47em}
% \centering
% \footnotesize
% \setlength{\tabcolsep}{3pt}
% \vspace{-3mm}
\centering
    \caption{\textbf{Learning hypothesis ablation.} Results on action classification performance on HMDB-51 is shown for finetuning accuracy (Acc) and frozen retrieval (recall@1) after pretraining on Kinetics-400 for 50 epochs.
    GDT can leverage signals from both \ul{i}nvariance and stronger \ul{d}istinctiveness transformation signals.
    We consider data-sampling (DS), time-reversal (TR) and time-shifting (TS).
    %hypotheses: Data-sample (DS), time-reversal (TR) and time-shift (TS).
    \label{tab:hypotheses_results}}
    % \vspace{2mm}
      \begin{tabular}{c cccc @{\hskip 5pt} cc }
      \toprule
         & DS & TR & TS & Mod. & $\mathbf{Acc.}$ & $\mathbf{R@1}$ \\
        \midrule
        \multicolumn{7}{l}{\textit{SimCLR-like: DS-distinctiveness only}}      \\
        (a) & \vv & \cc     &  \cc   &   V    & $44.6$ & $11.8$    \\ %% & 47.1 & 32.5
        (b) & \vv & \ii     &  \cc   &   V    & $36.9$ & $13.3$   \\ %% & 39.5 & 31.9
        (c) & \vv & \cc     &  \ii   &   V    & $35.9$ & $15.3$    \\ %% & 46.9 & 34.5 
        (d) & \vv & \ii     &  \ii   &   V    & $37.8$ & $13.9$    \\ %% & 46.6 & 33.4
        \midrule
        \midrule
        \multicolumn{7}{l}{\textit{Cross-modal}}\\
        (e) & \vv & \cc & \cc  & AV  & $52.4$ & $21.8$   \\
        (f) & \vv & \ii & \cc  & AV  & $58.8$ & $22.6$   \\
        (g) & \vv & \cc & \ii  & AV  & $57.4$ & $23.5$    \\
        (h) & \vv & \ii & \ii  & AV  & $59.9$ & $24.8$    \\ %% need to. change
        \midrule
        \multicolumn{7}{l}{\textit{Cross-modal +1 distinctive factor}} \\
        (i) & \vv & \vv & \cc  & AV  & $57.8$ & $26.1$ \\
        (j) & \vv & \cc & \vv  & AV  & $58.7$ & $22.1$  \\
        (k) & \vv & \vv & \ii  & AV  & $61.1$ & $25.4$ \\
        (l) & \vv & \ii & \vv  & AV &  $\bf{61.4}$ & $\bf{27.1}$ \\
        \hline
        \multicolumn{7}{l}{\textit{Cross-modal + 2 distinctive factors}} \\
        (m) & \vv & \vv & \vv  & AV & $57.2$ & $20.5$  \\ % 
        \bottomrule
    \end{tabular}
% \vspace{-5em}
\end{table}
% \end{wraptable}

% \newcommand{\vv}{{\bf{v}}}%
% \newcommand{\ii}{{\bf{i}}}%
% \newcommand{\cc}{{$\cdot$}}%
% \begin{table}
% %\vspace{-0.47em}
% \centering
% \footnotesize
% \setlength{\tabcolsep}{1pt}
% \vspace{-3mm}
%     \caption{\textbf{Learning hypothesis ablation.} Results on action classification performance on HMDB-51 is shown for finetuning accuracy (Acc) and frozen action retrieval (recall@5).
%     GDT can leverage signals from both  \ul{i}nvariance and stronger \ul{v}ariance transformation signals, that sole data-sample (DS) variance misses.
%     %hypotheses: Data-sample (DS), time-reversal (TR) and time-shift (TS).
%     \label{tab:hypotheses_results}}
%     % \vspace{-1mm}
%       \begin{tabular}{c cccc @{\hskip 5pt} cc }
%       \toprule
%          & DS & TR & TS & Mod. & \textbf{Acc} & $\mathbf{r@5}$ \\
%         \midrule
%         \multicolumn{6}{l}{\textit{SimCLR: DS-variance only}}      \\
%         (a) & \vv & \cc     &  \cc   &   V    & 47.1 & 32.5    \\
%         %%(b) & \vv & \ii     &  \cc   &   V    & 46.3 & 31.9   \\ %% need to. change
%         (b) & \vv & \ii     &  \cc   &   V    & 39.5 & 31.9   \\
%         (c) & \vv & \cc     &  \ii   &   V    & 46.9 & 34.5    \\
%         (d) & \vv & \ii     &  \ii   &   V    & 46.6 & 33.4    \\ %% need to. change
%         % (e) & \vv & \ii     &  \ii   &   VA    &  &  \\
%         \midrule
%         \midrule
%         \multicolumn{6}{l}{\textit{GDT}: 1-variance}\\
%         (e) & \vv & \cc & \cc  & AV  & $XX$ &  $XX$   \\
%         (f) & \vv & \ii & \cc  & AV  & $XX$ &  $XX$   \\
%         (g) & \vv & \cc & \ii  & AV  & $XX$ &  $XX$    \\
%         (h) & \vv & \ii & \ii  & AV  & $XX$ &  $XX$ \\ %% need to. change
%         \midrule
%         \multicolumn{6}{l}{\textit{GDT}: 2-variances} \\
%         (i) & \vv & \ii & \vv  & AV &  $XX$ &  $XX$ \\
%         (j) & \vv & \vv & \ii  & AV  & $XX$ &  $XX$ \\ %% need to. change
%         (k) & \vv & \cc & \vv  & AV  & $XX$ &  $XX$  \\
%         (l) & \vv & \vv & \cc  & AV  & $XX$ &  $XX$ \\
%         \multicolumn{6}{l}{\textit{GDT}: 3-variances} \\
%         (m) & \vv & \vv & \vv  & AV & $XX$ &  $XX$ \\ % 
%         \bottomrule
%     \end{tabular}
% % \vspace{-5em}
% \end{table}

% \newcommand{\vv}{{\bf{v}}}%
% \newcommand{\ii}{{\bf{i}}}%
% \newcommand{\cc}{{$\cdot$}}%
% \begin{wraptable}{r}{5.2cm} %\begin{table}
% %\vspace{-0.47em}
% \centering
% \footnotesize
% \setlength{\tabcolsep}{1pt}
% \vspace{-3mm}
%     \caption{\textbf{Learning hypothesis ablation.} Results on action classification performance on HMDB-51 is shown for finetuning accuracy (Acc) and frozen action retrieval (recall@5).
%     GDT can leverage signals from both  \ul{i}nvariance and stronger \ul{v}ariance transformation signals, that sole data-sample (DS) variance misses.
%     %hypotheses: Data-sample (DS), time-reversal (TR) and time-shift (TS).
%     \label{tab:hypotheses_results}}
%     % \vspace{-1mm}
%       \begin{tabular}{c cccc @{\hskip 5pt} cc }
%       \toprule
%          & DS & TR & TS & Mod. & \textbf{Acc} & $\mathbf{r@5}$ \\
%         \midrule
%         \multicolumn{6}{l}{\textit{SimCLR: DS-variance only}}      \\
%         (a) & \vv & \cc     &  \cc   &   V    & 47.1 & 32.5    \\
%         %%(b) & \vv & \ii     &  \cc   &   V    & 46.3 & 31.9   \\ %% need to. change
%         (b) & \vv & \ii     &  \cc   &   V    & 39.5 & 31.9   \\
%         (c) & \vv & \cc     &  \ii   &   V    & 46.9 & 34.5    \\
%         (d) & \vv & \ii     &  \ii   &   V    & 46.6 & 33.4    \\ %% need to. change
%         % (e) & \vv & \ii     &  \ii   &   VA    &  &  \\
%         \midrule
%         \midrule
%         \multicolumn{6}{l}{\textit{GDT}: 1-variance}\\
%         (e) & \vv & \cc & \cc  & AV  & $56.9$   & $49.3$   \\
%         (f) & \vv & \ii & \cc  & AV  & $56.1$   & $49.7$   \\
%         (g) & \vv & \cc & \ii  & AV  & $57.2$  & $45.2$    \\
%         (h) & \vv & \ii & \ii  & AV  &  $56.6$  & $44.8$ \\ %% need to. change
%         \midrule
%         \multicolumn{6}{l}{\textit{GDT}: 2-variances} \\
%         (i) & \vv & \ii & \vv  & AV & $57.5$ & $46.8$ \\
%         (j) & \vv & \vv & \ii  & AV  & $57.0$ & $46.2$ \\ %% need to. change
%         (k) & \vv & \cc & \vv  & AV  & $58.0$  & $50.2$  \\
%         (l) & \vv & \vv & \cc  & AV  & $58.2$  & $50.2$ \\
%         \multicolumn{6}{l}{\textit{GDT}: 3-variances} \\
%         (m) & \vv & \vv & \vv  & AV & $60.0$ &  $47.8$ \\ % 
%         \bottomrule
%     \end{tabular}
% % \vspace{-5em}
% \end{wraptable}

% \begin{wraptable}{r}{5.5cm} %\begin{table}
% \vspace{-1.5em}
% \centering
% \footnotesize
% \setlength{\tabcolsep}{1pt}
% \vspace{1mm}
%     \caption{Action retrieval performance on \textbf{H}MDB-51 and \textbf{U}CF-101 datasets  for different \textbf{i}nvariance or \textbf{v}ariance transformation hypotheses: Data-sample (DS), time-reversal (TR) and time-shift (TS).\label{tab:hypotheses_results}}
%     \vspace{-1mm}
%       \begin{tabular}{c cccc @{\hskip 5pt} cc }
%       \toprule
%          & DS & TR & TS & Mod. & \textbf{H} & \textbf{U} \\
%         \midrule
%         & \multicolumn{6}{l}{\textit{V-SimCLR baselines}}      \\
%         (a) & \vv & \cc     &  \cc   &   V    & 32.7 & 53.9 \\
%         (b) & \vv & \ii     &  \cc   &   V    &      &      \\
%         (c) & \vv & \cc     &  \ii   &   V    &      &      \\
%         (d) & \vv & \ii     &  \ii   &   V    &      &      \\
%         \midrule
%         & \multicolumn{6}{l}{\textit{V-SimCLR+pretext}}  \\
%         % \multicolumn{6}{l}{ these use fc-layer} \\
%         (e) & \vv & (\vv)    & \cc   & V \\
%         (f) & \vv & \cc      & (\vv) & V \\
%         \midrule
%         & \multicolumn{6}{l}{\textit{VA-SimCLR+pretext}} \\
%         %this uses another head with fc-layer
%         % \multicolumn{6}{l}{ these use fc-layer} \\
%         (g) & \vv &  \cc & \cc &    VA   \\
%         (h) & \vv & (\vv) & \cc   & VA \\
%         (i) & \vv & \cc & (\vv)   & VA \\
%         \midrule
%         \midrule
%         & \multicolumn{6}{l}{\textit{GDT: pretext-variances}} \\
%         %{pretty much our old runs, but with 2 heads} \\
%         % \vv &  \cc & \cc &    VA   \\
%         (j) & \vv & \vv & \cc  & VA \\
%         (k) & \vv & \cc & \vv  & VA \\
%         (l) & \vv & \vv & \vv  & VA \\
%         \midrule
%         & \multicolumn{6}{l}{\textit{GDT: pretext-var. and -invar.}} \\
%         % pretty much our old runs, but with 2 heads and "flip-of-coin" augmentation of TR/TS}  \\
%         (m) & \vv & \ii & \ii  & VA   \\
%         (n) & \vv & \vv & \ii  & VA \\
%         (o) & \vv & \ii & \vv  & VA \\
%         \bottomrule
%     \end{tabular}
% \vspace{-16pt}
% \end{wraptable}

% \begin{wraptable}{r}{5.5cm} %\begin{table}
% \vspace{-1.5em}
% \centering
% \footnotesize
% \setlength{\tabcolsep}{2pt}
% \vspace{1mm}
%     \caption{Downstream results action recognition   for \textbf{different transformation hypotheses}.}\label{tab:hypotheses_results}
%     \vspace{-1mm}
%       \begin{tabular}{l c c  @{\hskip 5pt} c c }
%       \toprule
%          & \multicolumn{2}{c}{\textbf{HMDB}} & \multicolumn{2}{c}{\textbf{UCF}} \\
%          \multicolumn{1}{r}{Epochs}  & 50 & 100 & 50 & 100 \\
%           \midrule
%         (a) Sample dist.  & 55.1 & 56.9 & 85.1 & 87.9  \\
%         \midrule %\midrule
%         Time shift (\textit{TS}) \\
%          (b) \quad  invariant (I)  & 54.8 & 56.1& 85.8 & 87.7  \\
%          (c) \quad  distinct (D)  & \ul{56.8} & \ul{58.2}& \ul{86.0} & \ul{86.5}  \\
%          \midrule
%         Time Reversal (\textit{TR}) \\
%          (d) \quad  invariant (I) & 53.2 & 57.2  & 86.6 & 88.1  \\
%          (e)  \quad distinct (D)  & \ul{54.7} & \ul{58.0} & \ul{87.2} & \textbf{\ul{88.5}} \\
%         \midrule
%         %(f) TS distinct, TS invariant  & \ul{56.8} & \ul{57.4} & \ul{86.7} & \ul{87.4}\\
%         %(g) TS distinct, TR distinct  & \ul{56.8} & \ul{60.0} & \ul{86.9} & \ul{87.3}\\
%         %(h) TS distinct, TR invariant & \ul{56.0} & \ul{57.5} & \ul{87.0} & \ul{88.2} \\
%         (f) \textit{TS} (D),  \textit{TS} (I)  & 56.8 & 57.4 & 86.7 & 87.4\\
%         (g) \textit{TS} (D),  \textit{TR} (D) & 56.8 & \bf{60.0} & 86.9 & 87.3 \\
%         (h) \textit{TS} (D), \textit{TR} (I)  & 56.0 & 57.5 & 87.0 & 88.2\\
%         \bottomrule
%     \end{tabular}
% \vspace{-16pt}
% \end{wraptable} %\end{table}
% % \quad

==> GDT (ICCV 2021)/tabs/t3_video-sota.tex <==
\begin{table}[t]
	\caption{\textbf{State-of-the-art on video action recognition with full-finetuning.} Self- and fully-supervisedly trained methods on UCF-101 and HMDB-51 benchmarks.
% 	We follow the standard protocol and report the average top-1 accuracy over the official splits for finetuning the whole network.
% 	Methods with $^\dagger$: use video titles as supervision, with $^*$: use ASR generated text.
	%See \cref{supp:tab:sota} for an extended version including recent/concurrent works.
	\labelswitch{tab:sota}
	}
% \footnotesize
% \setlength{\tabcolsep}{1.2pt}
    \include{tabs/full-finetune-joined}
\end{table}

==> GDT (ICCV 2021)/tabs/t45_ret-few-aud.tex <==
\begin{table}[t]
% \footnotesize
\begin{minipage}[t]{0.5\textwidth}
\centering
\input{tabs/_retrieval_and_fewshot}
\end{minipage}
\hfill
% \begin{minipage}[t]{0.5\textwidth}
% \centering
%     \input{tabs/_audio-results}	
% \end{minipage}
%  \vspace{-1em}
\end{table}

==> GDT (ICCV 2021)/tabs/t6_vggsound.tex <==
\begin{wraptable}{r}{4.5cm}
%\vspace{-0.5em}
%\begin{table}[t]
%\centering
\footnotesize
\setlength{\tabcolsep}{1.4pt}
\captionof{table}{\textbf{VGG-Sound.}
\break 
Audio classification metrics after full-finetuning. \label{tab:vggsound}
}
% \vspace{-1mm}
\begin{tabular}{l l ccc}
\toprule
\textbf{Method}                 & mAP        & AUC        & d' \\
\midrule
Supervised                      &51.6          &96.8          &2.63 \\
\textbf{GDT} (ours)             &\bf{54.8}     &\bf{97.5}     &\bf{2.77} \\
\bottomrule
\end{tabular}
 \vspace{-34pt}
\end{wraptable}



==> GDT (ICCV 2021)/vedaldi.tex <==
\newif\ifdark
\IfFileExists{/Users/vedaldi/.bash_profile}{
\immediate\write18{%
if defaults read -g AppleInterfaceStyle 2>/dev/null;
then echo \\darktrue > /tmp/displaymode.tex;
else echo \\darkfalse > /tmp/displaymode.tex; fi}
\input{/tmp/displaymode.tex}
\ifdark
\definecolor{pcolor}{HTML}{1E1E1E}
\definecolor{tcolor}{HTML}{C5C5C5}
\else
\definecolor{pcolor}{HTML}{FDF6E3}
\definecolor{tcolor}{HTML}{333333}
\fi
\pagecolor{pcolor}
\color{tcolor}
% Suppress hbadness warnings.
\hbadness=\maxdimen
\vbadness=\maxdimen
\vfuzz=30pt
\hfuzz=30pt
}{} 

==> figs/splash_source.tex <==
  \begin{figure}
   \newcommand{\Tone}{\colorbox{blue!30}{$T_1$}\xspace}
   \newcommand{\Ttwo}{\colorbox{blue!20}{$T_2$}\xspace}
   \newcommand{\Tthree}{\colorbox{blue!10}{$T_3$}\xspace}
   \newcommand{\Tfour}{\colorbox{blue!5}{$T_4$}\xspace}
   \newcommand{\Tfive}{\colorbox{red!30}{$T_5$}\xspace}
   \newcommand{\Tsix}{\colorbox{red!20}{$T_6$}\xspace}
   \newcommand{\Tseven}{\colorbox{red!10}{$T_7$}\xspace}
   \newcommand{\Teight}{\colorbox{red!5}{$T_8$}\xspace}
   \fboxsep1pt
   \footnotesize
   \begin{tikzpicture}[grow'=right,
     edge from parent/.style={draw,-latex},
     label distance = 0.1cm,
     level 1/.style = {level distance=1cm, sibling distance=4mm},
     level 2/.style = {level distance=1cm, sibling distance=8mm},
     level 3/.style = {level distance=1cm, sibling distance=4mm},
     level 4/.style = {level distance=1cm, sibling distance=4mm},
     level 5/.style = {level distance=0.5cm, sibling distance=4mm, edge from parent/.style={}},
     ]
   \node (X) {1}
   child { node[label={$t_1$}] at ($(X)+(1,+1.6)$) {$i_1$}
       child { node[label={$t_2$}]{$\tau_1$}
           child { node[label={$t_3$}]{$m_v$}
               child { node[label={$t_4$}]{$g_1$} child { node{\Tone}} }
           }
           child { node{$m_a$}
               child { 
                    child { nchild { node{\Ttwo}} } node{$g_2$}
                    child { node{\Ttwo}} }
           }
       }
       child { node{$\tau_2$}
           child { node{$m_v$}
               child { node{$g_3$} child { node{\Tthree}} }
           }
           child { node{$m_a$}
               child { node{$g_4$} child { node{\Tfour}} }
           }
       }
   }
   child { node at ($(X)+(1,0)$) {$i_2$}
       child { node{$\tau_3$}
           child { node{$m_v$}
               child { node{$g_5$} child { node{\Tfive}} }
           }
           child { node{$m_a$}
               child { node{$g_6$} child { node{\Tsix}} }
           }
       }
       child { node{$\tau_4$}
           child { node{$m_v$}
               child { node{$g_7$} child { node{\Tseven}} }
           }
           child { node{$m_a$}
               child { node{$g_8$} child { node{\Teight}} }
           }
       }
   }
   child { node at ($(X)+(1,-0.5)$) {$\dots$} }
   child { node at ($(X)+(1,-1)$) {$i_{M_i}$}
       child { node{$\dots$} }
   }
   ;
   \end{tikzpicture}
   \hfill
   \newcommand{\zp}{$\cdot$}
   \newcommand{\0}{$\cdot$}
   \newcommand{\m}{$0$}
   \newcommand{\as}{$\ast$}
   % \newcommand{\1}{\fcolorbox{LimeGreen!100}{white}{\bf{1}}}
   \newcommand{\1}{$1$}
   \newcommand{\ld}[1]{\ldelim\{{2}{*}[\parbox{2mm}{\rotatebox[origin=c]{90}{\tiny #1}}]}
   % \newcommand{\ld}[1]{}
   \begin{tabular}[b]{c@{\,}c|cccc|cccc}
       \multicolumn{2}{c}{}
       & \multicolumn{4}{c}{\tiny video $i_1$}
       & \multicolumn{4}{c}{\tiny video $i_2$} \\[-.5em]
       \multicolumn{2}{c}{}
       & \multicolumn{4}{c}{\tiny \downbracefill}
       & \multicolumn{4}{c}{\tiny \downbracefill}\\[-.5em]
       \multicolumn{2}{c}{}
       & \multicolumn{2}{c}{\tiny visual}
       & \multicolumn{2}{c}{\tiny audio}
       & \multicolumn{2}{c}{\tiny visual}
       & \multicolumn{2}{c}{\tiny audio} \\[-.5em]
       \multicolumn{2}{c}{}
       & \multicolumn{2}{c}{\downbracefill}
       & \multicolumn{2}{c}{\downbracefill}
       & \multicolumn{2}{c}{\downbracefill}
       & \multicolumn{2}{c}{\downbracefill} \\
               & $c$     & \Tone & \Tthree & \Ttwo & \Tfour & \Tfive & \Tseven & \Tsix & \Teight \\
   \cline{2-10}
   \ld{audio}  & \Ttwo   & \1    & \as     & \0    & \zp    & \m     & \zp      & \zp   & \zp  \\
               & \Tfour  & \as   & \1      & \zp   & \0     & \zp     & \m      & \zp   & \zp \\
   \ld{visual} & \Tone   & \0    & \zp     & \1    & \as    & \zp    & \zp     & \m    & \zp \\
               & \Tthree & \zp   & \0      & \as   & \1     & \zp    & \zp     & \zp    & \m \\
   \cline{2-10}
   \ld{audio}  & \Tsix   & \m    & \zp      & \zp   & \zp    & \1     & \as     & \0    & \zp \\
               & \Teight & \zp    & \m      & \zp   & \zp    & \as    & \1      & \zp   & \0 \\
   \ld{visual} & \Tfive  & \zp   & \zp     & \m     & \zp     & \0     & \zp     & \1    & \as \\
               & \Tseven & \zp   & \zp     & \zp    & \m     & \zp    & \0      & \as   & \1 \\
   \end{tabular}
   \caption{
       \textbf{Left}: Hierarchical sampling process of generalized transformations for the multimodal training study case.
       All transformations are contrastive except $t_4$ which is augmentative.
       \textbf{Right}: Subset of the $c(T,T')$ matrix illustrating its pattern.
       The matrix has a block-diagonal structure (transformations have been reordered to highlight the pattern).
       The diagonal contrasts different modalities subject to the same time shift (e.g.~\Tone vs \Ttwo), for which we assume invariance ($1$).
       Identical (e.g.~\Tone vs \Tone) or within modality (\Tone vs \Tthree) comparisons are ignored, setting $w(T,T')=0$ (denoted by a $\cdot$). % in the table).
       The major off-diagonal blocks are set to $0$ as we assume sample distinctiveness (e.g.~\Tone vs \Tsix). %, except for within modality comparisons that we still ignore.
       Contrasting time shifts (e.g.~\Tone vs \Tfour) can be used for invariance, distinctiveness or ignored (baseline), so $\ast \in \{+1,0,\cdot\}$.
   }\label{f:theory}
   \end{figure}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{d}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> scratch.tex <==

\subsection{The general case: contrastive and augmentative transformations}

In order to instantiate~\cref{e:contrastive}, we require not only a definition of the function $c(T,T')$, but also a way of sampling transformations in the batch.
Differently from most learning formulations, in contrastive learning, one \emph{must} ensure that the batch contains transformations that can be meaningfully contrasted, so transformations cannot be sampled independently.

We propose the following \emph{hierarchical} sampling scheme.
Each generalized transformation $T=t_M \circ \dots \circ t_1$ is constructed as a sequence of $M$ transformations $t_m$.
First, we sample  $K_1$ versions of transformation $t_1$; then, for each sample $t_1$, we sample $K_2$ versions of transformation $t_2$ and so on, obtaining a total of $K=\prod_{m=1}^M K_m$ different transformations $T$ for the batch.

We distinguish between two types of transformations, depending on how we sample them.
For a \emph{contrastive transformation} $t_m$, we always sample \emph{two or more versions} of the same transformation, i.e.~$K_m \geq 2$.
For an \emph{augmentative transformation}, we only sample a single version, i.e.~$K_m=1$.
As the name suggests, contrastive transformations lead to explicit comparisons in the loss~\cref{e:contrastive}, whereas augmentative ones do not.\todo{This distinction actually does not make sense. Will likely remove.}

Given two generalized transformations $T=t_M\circ\dots\circ t_1$ and $T'=t'_M\circ\dots\circ t'_1$ sampled in this manner, we must also define $c(T,T')$.
For individual transformations, we set:
\begin{equation}
c(t_m,t_m')
=
\begin{cases}
1, & \text{if $t_m$ is augmentative or invariant contrastive},\\
2\delta_{t_m=t_m'}-1, & \text{if $t_m$ is distinctive contrastive.}
\end{cases}
\end{equation}
Then, if any $c(t_m,t_m')=-1$, we set $c(T,T')=-1$ for the overall transformation, otherwise we set $c(T,T')=1$.
In practice, we consider slightly refined definitions of $c(T,T')$ to allow for some comparisons to be ignored ($c(T,T')=0$), as suggested above and further detailed below.

\subsection{Learning hypotheses}
\begin{figure}[!tb]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/GDT_template.pdf}
    \caption{\textbf{The GDT loss template.}
    xxx.
    }\label{fig:template}
\end{figure}

Next, we describe the learning hypotheses explored in the paper.
These correspond to different definitions of the function $c(T,T')$, coding for invariance or distinctiveness to various transformations.
The function defaults to $c(T,T')=1$ (invariance), with the following modifications:

\paragraph{Sample distinctiveness.}

The representation must distinguish different videos, so that $i \not = i' \Rightarrow c(T,T')=0$.
This is the baseline on which the other hypotheses build upon.

\paragraph{Modality invariance (AV correspondence).}

The representation must be invariant to the selected modality, so $c(T,T')$ is not affected by $m$ or $m'$.
Combined with sample distinctiveness, this means that the representation must be able to identify the same video from either the visual or audio components.
Stated differently, the representation must be able to put in correspondence visual and audio tracks from the same video.

\paragraph{Augmentation invariance.}

The representation should be invariant to data augmentation.
Hence $c(T,T')$ is not affected by $t$ or $t'$.

\paragraph{Time shift invariance/distinctiveness (synchronization).}

The representation might be either invariant or distinctive to a temporal shift.
The latter, captured by $\tau \not= \tau' \Rightarrow c(T,T')=0$, means that the representation can tell if two clips from the same video are synchronized or not.
Combined with modality invariance, this also means deciding if the visual and audio components are in sync.

\paragraph{Time reversal invariance/distinctiveness (arrow of time).}

Similar to before, in order to train a representation sensitive to time reversal, we set $r \not= r' \Rightarrow c(T,T')=0$.

Distinctiveness to the arrow of time~\citep{wei2018learning} and synchronization~\citep{avts,owens2018audio,arandjelovic2018objects} were explored before, albeit in a different setup that requires either a binary classifier or a curriculum; furthermore, here we also test whether invariance to either effects is preferable to distinctivenesses as a learning cue.

{\color{red} motivation: need to also explain how our formulation can encode for combination of hypotheses and why the GDT formation is advantageous / key}

{\color{red} need to also explain how our formulation can encompass other papers: 3D Rotnet, Jigsaw, Sync, AVC, in a table -> extensibility}

{\color{red} also need to concretize notation to hypothesis table}

\section{Multi-modal self-supervision}

We apply our framework to multi-modal self-supervision where the data $x$ are \emph{videos}.
We learn representations using invariance or distinctiveness to several types of transformations, with each setting corresponding to a different \textit{learning hypothesis}.
This requires to decide how transformations $T$ are sampled in the contrastive loss~\cref{e:contrastive} and which transformation pairs $c(T,T')$ are considered positive or negative, thus leading to different invariance/distinctiveness requirements.

\subsection{Sampling transformation}

First, we discuss how transformations are sampled.
In order for the batch to contain a mix of positive and negative transformation pairs, we sample them in pairs.
Specifically, we start by sampling $K$ generalized transformations $T_1,\dots,T_m$ i.i.d.~at random.
Then, for each $T_m$, we randomly sample a second transformation $T_m' | T_m$ condition on the first.
This second, related transformation $T_m'$ does \emph{not} necessarily constitute a positive pairing with $T_m$; instead, we will choose $c(T_m,T_m')=1$ for invariance or $c(T_m,T_m')=0$ for distinctiveness.

In more detail, let the pair of transformations be the tuples $T_m= A_k \circ H_k$ and we will focus on formulating different choices of $H_k = (i,\tau,m,t,r)$ and $H_k'=(i',\tau',m',r')$ constructed as follows.

\paragraph{Sample selection.}
$H_k$ selects first a random video $x_i$ from the dataset $D$.
The paired transformation $H'_k$ always selects the same sample $i'=i$.\footnote{While we do not explore this case here, it is meaningful to also consider pairs where $i'\not=i$ --- this could be used, for example, to test whether two different images are rotated by different amounts, similar to RotNet.}

\paragraph{Temporal clipping.}
After selecting a video, $H_k$ extracts a 1s clip $x_{i\tau}$ from it, where the the starting time $\tau$ is selected uniformly at random.
$H'_k$ then picks either the same start time $\tau=\tau'$ or another uniformly randomly start time. % $\tau' \sim \mathcal{N}(\tau,\sigma^2)$.

\paragraph{Modality slicing.}
Next, $H_k$ slices a modality $m(x_{i\tau})$ at random, where $m\in\mathcal{M}$ extracts either the visual $v_{i\tau}$ or the audio $a_{i\tau}$ component from the video, as explained before.
$H'_k$ either samples a modality $m'$ independently of $m$, or always picks the opposite modality $m'\not =m$.

\paragraph{Augmentation and normalization.}
Following video selection, clipping and slicing, we apply a random augmentation.
For the visual component, $H_k$ extracts a fixed-size tensor $t(v_{i\tau})$ where $t$ picks a random spatial crop and resizes it to a fixed resolution.
For the audio component, $t(a_{i\tau})$ is a spectrogram representation of the audio signal followed by SpecAugment~\cite{Park_2019}.
The transformation $t'$ in $T'_k$ is sampled in the same way, independently of $t$.

\paragraph{Time reversal.}
Finally, $H_k$ applies a time reversal operator $r\in\mathcal{R}=\{r_0, r_1\}$, where $r_0$ is the identity (do nothing) and $r_1$ flips the time dimension of its input tensor.
The transformation $r'$ in $H'_k$ is sampled independently.

\subsection{Learning hypotheses}
\begin{figure}[!tb]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/GDT_template.pdf}
    \caption{\textbf{The GDT loss template.}
    xxx.
    }\label{fig:template}
\end{figure}

Next, we describe the learning hypotheses explored in the paper.
These correspond to different definitions of the function $c(T,T')$, coding for invariance or distinctiveness to various transformations.
The function defaults to $c(T,T')=1$ (invariance), with the following modifications:

\paragraph{Sample distinctiveness.}

The representation must distinguish different videos, so that $i \not = i' \Rightarrow c(T,T')=0$.
This is the baseline on which the other hypotheses build upon.

\paragraph{Modality invariance (AV correspondence).}

The representation must be invariant to the selected modality, so $c(T,T')$ is not affected by $m$ or $m'$.
Combined with sample distinctiveness, this means that the representation must be able to identify the same video from either the visual or audio components.
Stated differently, the representation must be able to put in correspondence visual and audio tracks from the same video.

\paragraph{Augmentation invariance.}

The representation should be invariant to data augmentation.
Hence $c(T,T')$ is not affected by $t$ or $t'$.

\paragraph{Time shift invariance/distinctiveness (synchronization).}

The representation might be either invariant or distinctive to a temporal shift.
The latter, captured by $\tau \not= \tau' \Rightarrow c(T,T')=0$, means that the representation can tell if two clips from the same video are synchronized or not.
Combined with modality invariance, this also means deciding if the visual and audio components are in sync.

\paragraph{Time reversal invariance/distinctiveness (arrow of time).}

Similar to before, in order to train a representation sensitive to time reversal we set $r \not= r' \Rightarrow c(T,T')=0$.

Distinctiveness to the arrow of time~\citep{wei2018learning} and synchronization~\citep{avts,owens2018audio,arandjelovic2018objects} were explored before, albeit in a different setup that requires either a binary classifier or a curriculum; furthermore, here we also test whether invariance to either effects is preferable to distinctivenesses as a learning cue.

Another line of work in self-supervision uses multiple data modalities instead of using only images.
In this case, the task is to predict one modality from the other, such as predicting properties of the audio track in a video from images extracted from it~\citep{owens2016ambient}.
Cross-modal self-supervision is, in practice, also very powerful, although in these cases, data augmentations have been considered as useful but not key elements of the formulations.

In this paper, we argue that transformations are in fact \emph{central} to self-supervision.
% By this, we mean that the specific learning formulation, contrastive or not, is not as crucial.
We develop a clear framework for semantics preserving data augmentations for multi-modal training.
In particular, we view multi-modal training as a \emph{special case} of data transformation and thus, any recent method in self-supervised learning can be applied to this case without changes.

This can be explained succinctly as follows.
In self-supervision in the image domain, one starts from an image $x$ and generates a second, congruous image $t(x)$ by applying a nuisance transformation $t$ to $x$.
These transformations leave the semantic content mostly intact but can introduce noise as variance or make the task more difficult by masking parts of the inputs.
The goal is then to learn a representation $\Phi$ which is approximately invariant to $t$,
i.e.~$\Phi(x) \approx \Phi(t(x))$.
The latter must be paired with a constraint that the representation should also be distinctive, i.e.~$\Phi(x)\not=\Phi(x')$ if $x$ and $x'$ are different images.

In multi-modal learning, one starts instead from composite data $z=(a,v)$.
For example, $a$ could be the audio stream and $v$ the video stream in a video.
Then, instead of directly learning to predict the audio $a$ from the video $v$ (or vice-versa), which is an ill-posed problem, one might instead wish to learn  a pair of representations $\Phi_\mathrm{a}(a) \approx \Phi_\mathrm{v}(v)$, one for each stream.
In this case, distinctiveness means that  $\Phi_\mathrm{a}(a) \not= \Phi_\mathrm{v}(v')$ if $(a,v)\not=(a',v')$ are two different videos.

It is then easy to combine these two approaches under the same formulation as shown in Figure~\ref{fig:splash}.
The first step is to consider transformations $t(x)$ applied to the composite data.
These \emph{generalized transformations} play two roles: (a) to \emph{slice} (selecting \emph{which} modality to observe) and (b) to \emph{augment} (applying a random perturbation to the modality) the data.
The second step is to consider a representation $\Phi$ that can take as input any modality.
This is trivially achieved by considering a pair of networks $\Phi =(\Phi_\mathrm{a},\Phi_\mathrm{v})$ as before, with the convention that $\Phi(t(x))$ amounts to running either $\Phi_\mathrm{a}$ or $\Phi_\mathrm{v}$ depending on which modality is sliced by $t$.

Since transformations on videos can be applied in the time dimension as well, this results in a \emph{combinatorial} space of possible transformations that can be used to slice and augment multi-modal data.
A second contribution of the paper is to study this space, demonstrating the power of searching for better sets of transformations.
We show empirically the power of these intuitions by building them into MoCo~\citep{he2019momentum}, an off-the-shelf self-supervised method for learning from static images, extending it to a state-of-the-art method for learning from multi-modal data.

\subsection{Semantic video augmentations \label{sec:transforms}}
\begin{figure}[!tb]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/aug.pdf}
    \caption{\textbf{GDT augmentation space for videos.} For visual clips, we apply cropping, flipping and temporal jittering. 
    For auditory clips, we use SpecAugment~\cite{Park_2019} along with temporal jittering. 
    In addition, both clips can be independently sampled yielding asynchronization.}
    \label{fig:transformation}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%% 
\paragraph{Implementation.}
For learning robust representations, the applied within-modal augmentations are shown in Figure~\ref{fig:transformation}. 

For $\mathcal{A}_\mathrm{a}$, the audio-level augmentations, we use one second clips using log mel bank features with 40 MEL filters and 99 audio frames and apply SpecAugment~\citep{Park_2019}.

The visual augmentations $\mathcal{A}_\mathrm{v}$ are borrowed from~\citep{avts} and consist of first sampling one second of video at the original frame rate, applying a resizing to $(128\times171)$, random cropping to $(112\times112)$ and random horizontal flipping. 
For both modalities, we explore the effect of sampling clips from the source videos at different times each epoch, which we refer to as temporal jittering. 
We show examples of how these transformations affect the input in Figure~\ref{fig:transformation}.

\subsection{Generalized Data Transformations}
%While previous works have utilized hand-crafted losses for videos such as colorization~\citep{vondrick2018tracking} or detecting rotations in clips~\citep{jing2018self}, we apply a contrastive loss function, which has recently been shown to yield good performance for images and videos~\citep{sohn2016improved,he2019momentum,Wu_2018_CVPR,oord2018representation,Chen2020ASF,miech2019endtoend,han2019video,sun2019contrastive,li2020learning} without the need to implicitly specify what information needs to be discarded via a designed task.

For training our network in a self-supervised manner, we utilize the above semantics preserving video augmentations and combine them with various other task-specific transforms $\mathcal{T}$, which we will call \textit{learning hypotheses}. 
Each hypothesis constitutes a prior on what the network should learn via specifying desirable invariances or variances.
As such, they can encode previously proposed pretext tasks and we select a subset of those to include in our framework:
\begin{itemize}
   \item  Audio-Visual correspondence: this is our basecase and the transformation is the identity function, $\mathcal{T}(z)=z$, where $z$ is the audio or video input.
   \item  (In)Variance to temporal synchronization. The transformation asynchronizes the input: $\mathcal{T}(z(t_n))= z(t_m), t_m\neq t_n$.
   \item  (In)Variance to the arrow of time. The transformation reverses the arrow of time. $\mathcal{T}(\vec{z})=\cev{z}$, where $\cev{z}$ represents the reversing of the frames for visual input and the left-right flipping of the spectrogram for audio.
\end{itemize}
Note that we do not only choose the hypotheses chosen in previous works (variant to arrow of time ~\citep{wei2018learning}, variant to synchronization ~\citep{avts, owens2018audio}), but also their reversals to investigate the performance when treating these task-specific transforms as semantics preserving augmentations.

For each of these hypotheses, applying them as a desired variance requires treating them differently than the augmentations described in Sec~\ref{sec:transforms}.
While the papers that have proposed these tasks use binary classifiers~\citep{wei2018learning,arandjelovic17look, owens2018audio} or margin constrastive losses~\cite{avts}, we accommodate these various hypotheses in a noise contrastive loss formulation~\citep{gutmann2010noise, Wu_2018_CVPR,tian2019contrastive,Chen2020ASF,he2019momentum,misra2019selfsupervised,henaff2019data,hjelm2018learning} by specifying the positives and the negatives accordingly, as shown in Table~\ref{tab:hypotheses}.
\input{tabs/pos-neg}

\paragraph{Two sets of composed transforms.}
Given the within-modality augmentations $\mathcal{A}$, we construct two composed transformations:

First, the base set of augmented data can be defined as applying an operator 
\begin{align}
t_1 & =\mathcal{I} \circ \mathcal{M} \circ \mathcal{A}
\end{align}
on the dataset $D$,
where $\mathcal{I}$ selects a source video with a random index and $\mathcal{M}$ select the modality.
The second transformation $t_2$ can be used to define additional variances (e.g.~synchronization or arrow of time) via task-specific transforms $\mathcal{T}$:
\begin{align}
t_2(t_1) & =\mathcal{I}(t_1) \circ \mathcal{M}(t_1) \circ \mathcal{A} \circ \mathcal{T}(t_1)
\end{align}
and is dependent on the first operation.

\paragraph{Loss.}
Given a network~$\Phi$, a positive pair for the noise contrastive loss is thus given by 
\begin{align}
\textit{pos} &= (\Phi(t_1) , \Phi(t_{i}))(D),
\end{align}
with $i=1$ for inducing the various invariance hypotheses, and $i=2$ for inducing variance.
The negatives are given by the batch (of size 1024) as well as the examples of $t_2$ which are used for variance. 
We do not use a memory bank~\citep{tian2019contrastive,Wu_2018_CVPR} or another momentum network~\citep{he2019momentum} to reduce memory footprint, as we have not observed it to yield noticable gains.

By denoting the positive example of datapoint $x$ as $x'$, and the task-specific negatives by $\textit{neg}(x)$, the loss is given by
\begin{align}
\label{eq:loss}
    L(x,x')  =& 
          \log \frac{\exp(\langle \Phi(x),\Phi(x') \rangle_\tau)}
    {\exp(\langle \Phi(x),\Phi(x') \rangle_\tau)
          + \sum_{y \in \mathcal{B} + \{\textit{neg(x)}\}}\exp(\langle \Phi(x) ,\Phi(y) \rangle_\tau)},
\end{align}
 where $\langle \cdot,\!\cdot \rangle_\tau$ is the dot product of the L2-normalized embeddings multiplied by $\tau$, a temperature parameter for the cross entropy loss, as in~\citep{he2019momentum,Chen2020ASF}.
 The final loss is given by the sum of $L(x,x')$ and $L(x',x)$ and computed across all positive pairs with all $N$ noise samples for each datapoint $x$ in the batch.

\paragraph{Learning invariance gradually.}
By writing the negative gradient of this loss with regards to the sample's embedding $\Phi(x)$, \ie~the direction of a step of SGD, as done in~\citep{Chen2020ASF},
{\color{red} redo with final loss formulation}
\begin{align}
    -\nabla_{\Phi(x)} L(x) \propto 
         \Phi_(x')(1-\exp(2\langle \Phi(x),\Phi(x') \rangle_\tau)) 
          - \sum_{\alpha=1}^{N}\Phi_{jx'}\exp(\langle \Phi_{ix} ,\Phi_{jx'} \rangle_\tau)~,
\end{align}
we find that the gradient automatically reweights examples by assigning a smaller gradient to easy pairs (i.e., $\langle \Phi_{ix}, \Phi_{jx} \rangle \approx 1$) and a larger gradient to more difficult pairs.
Because we use a large augmentation space that subsumes both weaker as well as stronger transformations, our method generates a curriculum implicitly:
it will first learn to associate the easy pairs and then it will learn the more difficult pairs (\ie~heavily augmented). We confirm this hypothesis in Section~\ref{sec:curr}.

As shown in~\citep{oord2018representation,tian2019contrastive}, the negative noise  contrastive loss represents a lower bound on the mutual information between the two inputs $\Phi(x)$ and $\Phi(x')$. 
With our similarities always computed across modes, minimizing the loss thus leads to increasing (a lower bound on) the mutual information between the individually augmented modalities -- \emph{i.e.} capturing the common semantics. 
However, optimizing an estimate of the mutual information is not a necessary condition for good representations~\citep{tschannen2020on}.

==> tabs/_abl-negs.tex <==

\setlength{\tabcolsep}{3pt}
\caption{\textbf{Number of negatives.}}
   \centering
  \footnotesize
  \begin{tabular}{l c c @{\hskip 5pt} c c}% c}
  \toprule
     \textbf{\#Negs} &  \multicolumn{2}{c}{\textbf{UCF}} & \multicolumn{2}{c}{\textbf{HMDB}} \\
    % &  50 & 100 & 50 & 100 \\
    Epochs & 50 & 100  & 50 & 100  \\
    \midrule 
        32  & $83.9$ & $\ul{87.1}$ & $\ul{52.1}$ & $53.8$  \\
        1024  & $\ul{84.8}$ & $86.5$ & $51.5$ & $\ul{55.6}$ \\ 
    \bottomrule
  \end{tabular}
  \vspace{5pt}
  \label{tab:ablation:temp}

==> tabs/_abl-tau.tex <==

\setlength{\tabcolsep}{3pt}
\caption{\textbf{Tau, \textbf{$\tau$}.}}
  \centering
  \footnotesize
  \begin{tabular}{l c c @{\hskip 5pt} c c}
  \toprule
      \textbf{Tau} & \multicolumn{2}{c}{\textbf{UCF}} & \multicolumn{2}{c}{\textbf{HMDB}} \\
    % & 50 & 100  & 50 & 100  \\
    Epochs & 50 & 100  & 50 & 100  \\
    \midrule %\midrule
    % {50: 42.68, 100: 44.39, 150: 44.79, 200: 43.14}
          $0.2^{-1}$  & $84.4$ & $85.8$ & $51.2$ & $53.7$  \\
          $0.07^{-1}$ & $\ul{84.8}$ & $\ul{86.5}$ & $\ul{51.5}$ & $\ul{55.6}$   \\
          % seed = epoch % 5 variant ?
    \bottomrule
  \end{tabular}
  \vspace{5pt}
  \label{tab:ablation:tau}

==> tabs/_audio-results.tex <==
%\begin{table}[t]
\footnotesize
%\scriptsize
\setlength{\tabcolsep}{1pt}
\captionof{table}{\textbf{Audio classification.} 
Downstream task accuracies on standard audio classification  benchmarks. For ESC-50 and DCASE2014, we report top-1 accuracy. 
%Methods with $^*$ use full-finetuning of their encoder network. %, $\star$ is concurrent. 
\label{tab:audio}}
% \vspace{.5em}
\begin{tabular}{l c cc} 
\toprule
\textbf{Method}    \\
                                 & \textbf{Data} & \textbf{DCASE}  & \textbf{ESC-50 } \\
\midrule
Human \citep{esc50}                     & --      & 81.3  \\
Supervised \citep{VGGSound}             & --      & --    \\
\midrule
ConvRBM \citep{sailor2017}          & None    & --      & 86.5 \\
AVTS \citep{avts}                 & K-400      & 91      & 76.7 \\
% DMC \citep{hu2018deep}            & K-400      & --      & 82.6 \\
XDC \cite{alwassel2019self}       & K-400      & --      & 78.5 \\
AVID \citep{morgado2020avid}      & K-400      &\ul{93}  &\bf{79.1} \\
\midrule
\textbf{GDT} (ours)               & K-400      &\bf{XX}  &\ul{XX}\\
\bottomrule
\end{tabular} 
%\end{table}

% %\begin{table}[t]
% \footnotesize
% %\scriptsize
% \setlength{\tabcolsep}{1pt}
% \captionof{table}{\textbf{Audio classification.} 
% Downstream task accuracies on standard audio classification  benchmarks. For ESC-50 and DCASE2014, we report top-1 accuracy and for VGG-Sound, mAP. 
% %Methods with $^*$ use full-finetuning of their encoder network. %, $\star$ is concurrent. 
% \label{tab:audio}}
% % \vspace{.5em}
% \begin{tabular}{l ccc} 
% \toprule
% \textbf{Method}    \\
%                                           & \textbf{DCASE}  & \textbf{ESC-50 }& \textbf{VGG-S}\\
% \midrule
% Human \citep{esc50}                     & --      & 81.3 & -- \\
% Supervised \citep{VGGSound}             & --      & --       & \ul{51.6}     \\
% \midrule
% %Autoencoder \citep{aytar2016soundnet} & - &   39.9         \\
% %Random Forest \citep{esc50}           & - &   44.3         \\
% %Piczak ConvNet \citep{Piczak2015}     & - &   64.5       \\
% %RNH \citep{rnh2013}                   &72 & -                  \\
% %Ensemble \citep{stowell2015}          &77 &   -                \\
% ConvRBM \citep{sailor2017}               &--        & 86.5   & --      \\
% %SoundNet \citep{aytar2016soundnet}      &88       & 74.2          \\
% %L3-Net \citep{arandjelovic17look}       &93       & 79.3          \\
% AVTS \citep{avts}                        &94       & 82.3   & --       \\
% DMC \citep{hu2018deep}                  &--       & 82.6   & --       \\
% XDC \cite{alwassel2019self}             &95       & 84.8   & --       \\
% AVID \citep{morgado2020avid}            &\ul{96}  &\bf{89.2}  & --    \\
% \midrule
% \textbf{GDT} (ours)                    &\bf{98}  &\ul{88.5}     & \bf{54.8}  \\
% \bottomrule
% \end{tabular} 
% %\end{table}

==> tabs/appx-ablations.tex <==
\begin{table*}[b]
\caption{\textbf{NCE loss computation parameters.} Top-1 accuracies (as \%) on downstream video classification tasks are shown after $50$ and $100$ epochs of pretext training.}\label{tab:ablation-appx}
\centering
	\begin{subtable}[b]{.33\linewidth}\centering
		{\input{tabs/_abl-tau}}	
	\end{subtable}
	\qquad
	\begin{subtable}[b]{.33\linewidth}\centering
		{\input{tabs/_abl-negs}}	
	\end{subtable}
\end{table*}

==> tabs/appx-retrieval.tex <==
 \begin{table}[htb]
\setlength{\tabcolsep}{3pt}
\centering
\caption{\textbf{Full retrieval table.}\label{tab:ret-full}}
  \centering
  \footnotesize
  \begin{tabular}{l c c c c c @{\hskip 5pt} c c c c c}
  \toprule
      & \multicolumn{5}{c}{\textbf{HMDB}} & \multicolumn{5}{c}{\textbf{UCF}} \\
      \cmidrule(lr){2-6} \cmidrule(lr){7-11} \multicolumn{1}{r}{Recall @} & 1 & 5  & 10 & 20 & 50 & 1 & 5 & 10 & 20 & 50  \\
    \midrule %\midrule
    Supervised (Kinetics) & 49.1 & 74.4 & 83.9 & 90.6 & 96.4 & 86.9 & 94.6 & 96.5 & 98.1 & 99.0 \\
    \midrule 
    ST-Puzzle~\citep{kim2019self}             & -- & -- & -- & -- & -- & 19.7 & 28.5 & 33.5 & 40.0 & 49.4 \\
    OPN~\citep{lee2017unsupervised}           & -- & -- & -- & -- & -- & 19.9 & 28.7 & 34.0 & 40.6 & 51.6  \\
    ST Order ~\citep{buchler2018improving}    & -- & -- & -- & -- & -- & 25.7 & 36.2 & 42.2 & 49.2 & 59.5  \\
    ClipOrder~\citep{clip_order}              & 7.6 & 22.9 & 34.4 & 48.8 & 68.9 & 14.1 & 30.3 & 40.4 & 51.1 & 66.5  \\
    SpeedNet~\citep{benaim2020speednet}        & -- & -- & -- & -- & -- & 13.0 & 28.1 & 37.5 & 49.5 & 65.0  \\
    VCP~\citep{luo2020video}                  & 7.6 & 24.4 & 36.3 & 53.6 & 76.4 & 18.6 & 33.6 & 42.5 & 53.5 & 68.1  \\
    VSP~\citep{cho2020selfsupervised}         & 10.3 & 26.6 & 38.8& 54.6 & 76.8 & 24.6 & 41.9 & 51.3 & 62.7 &76.9   \\
    \midrule
    \textbf{GDT (Kinetics)} &\textbf{25.4} & \textbf{51.4} &\textbf{63.9} & \textbf{75.0} & \textbf{87.8} & \textbf{57.4} & \textbf{73.4} & \textbf{80.8} & \textbf{88.1}  & \textbf{92.9} 
     \\
    \textbf{GDT (VGG-Sound)} & \textbf{28.4} & \textbf{55.1} & \textbf{67.2} & \textbf{79.3}  & \textbf{91.1} 
    &\textbf{63.4} & \textbf{79.6} &\textbf{85.0} & \textbf{90.1} & \textbf{95.2} \\
    \textbf{GDT (Audioset)} & \textbf{30.6} & \textbf{58.0} & \textbf{69.8} & \textbf{79.9}  & \textbf{91.0} 
    &\textbf{65.9} & \textbf{82.6} &\textbf{88.2} & \textbf{92.2} & \textbf{96.6} \\
    \textbf{GDT (IG65M)} & \textbf{36.1} & \textbf{61.1} & \textbf{70.8} & \textbf{79.7}  & \textbf{92.1} 
    &\textbf{75.7} & \textbf{87.2} &\textbf{90.7} & \textbf{93.5} & \textbf{96.6} \\
    \bottomrule
  \end{tabular}
  \vspace{5pt}

 \end{table}

==> tabs/appx-video-full-finetune.tex <==
\begin{table*}[!ht]
    \small
	\centering
	\caption{\textbf{State-of-the-art on action recognition.}
	Self-supervised and supervised methods on UCF101 and HMDB51 benchmarks.
	We follow the standard protocol and report the average top-1 accuracy over the official splits and show results for finetuning the whole network.
	Note that we find the supervised baseline to be around $6\%$ and $2\%$ better than reported in \citep{alwassel2019self} as we use a different finetuning strategy. 
	Methods with $^\dagger$ indicate the additional use of video titles as supervision.
	Methods with $^*$ use ASR generated text.
	Methods in {\color{gray} gray}  are concurrent works.
	\dontshowthisinappendix{See \cref{supp:tab:sota} in the Appendix for a full version of this table.}
	\labelswitch{tab:sota}}
	\tabcolsep=0.09cm
	\begin{tabular}{l l l @{\hskip 0.2in} c c }
		\toprule
		%\multicolumn{3}{c|}{\underline{Pretraining}} & \multicolumn{4}{c}{\underline{Evaluation}} \\
		\textbf{Method}                              & \textbf{Architecture} & \bf{Pretrain Dataset}  & %\multicolumn{2}{c}{\underline{\textbf{ft. last}}}
		\multicolumn{2}{c}{\textbf{Top-1 Acc\%}} \\
		                                             &                       &                           & HMDB\,        & UCF          \\
		\midrule 
		Full supervision                             & R(2+1)D-18            & ImageNet                  & 46.7          & 82.8         \\ 
		Full supervision~\citep{alwassel2019self}    & R(2+1)D-18            & Kinetics-400              & 65.1          & 94.2         \\   
		Full supervision (ours)                      & R(2+1)D-18            & Kinetics-400              & 70.4          & 95.0         \\
		 
		Full supervision~\citep{tran2018closer}      & R(2+1)D-34            & Kinetics-400              & 74.5          & 96.8         \\   
		\midrule 
		\textit{Using UCF}  \\ 
		Shuffle and Learn~\citep{misra2016shuffle}   & CaffeNet              & UCF                       & 18.1          & 50.2         \\   
		VGAN~\citep{vondrick2016generating}          & VGAN                  & Flickr                    & --            & 52.1         \\   
		LT-Motion~\citep{Luo_2017}                   & VGG-16                & UCF                       & --            & 53.0         \\   
		Geometry~\citep{gan2018geometry}             & CaffeNet              & UCF                       & 23.3          & 55.1         \\   
		OPN~\citep{lee2017unsupervised}              & VGG                   & UCF                       & 23.8          & 56.3         \\   
		ST Order ~\citep{buchler2018improving}       & CaffeNet              & UCF                       & 25.0          & 58.6         \\   
		CMC~\citep{tian2019contrastive}              & CaffeNet              & UCF                       & 26.7          & 59.1         \\   
		VCP~\citep{luo2020video}                     & R(2+1)D-18            & UCF                       & 32.2          & 66.3         \\   
		Cross and Learn ~\citep{Sayed_2019}          & VGG-16                & UCF                       & 33.0          & 70.5         \\   
		\midrule
		\textit{Using Kinetics}  \\
		ClipOrder~\citep{clip_order}                 & R(2+1)D-18            & Kinetics-400              & 30.9          & 72.4         \\  
        MotionPred~\citep{motion_statistics}         & C3D                   & Kinetics-400              & 33.4          & 61.2         \\    
		RotNet3D~\citep{jing2018self}                & 3D-ResNet18           & Kinetics-600              & 33.7          & 62.9         \\  
		ST-Puzzle~\citep{kim2019self}                & 3D-ResNet18           & Kinetics-400              & 33.7          & 65.8         \\  
		DPC~\citep{han2019video}                     & 3D-ResNet34           & Kinetics-400              & 35.7          & 75.7         \\  
		VPS~\citep{cho2020selfsupervised}            & R3D                   & Kinetics-400              & 36.8          & 74.8         \\  
		SpeedNet~\citep{benaim2020speednet}          & I3D                   & Kinetics-400              & 43.7          & 66.7         \\  
		AoT~\citep{wei2018learning}                  & T-CAM                 & Kinetics-400              & -             & 79.4         \\  
		CBT~\citep{sun2019contrastive}               & S3D                   & Kinetics-600              & 44.6          & 79.5         \\  
		Multisensory~\citep{owens2018audio}          & 3D-ResNet18           & Kinetics-400              & -             & 82.1         \\  
		XDC~\citep{alwassel2019self}                 & R(2+1)D-18            & Kinetics-400              & 52.6          & 86.8         \\  
		AV Sync+RotNet~\citep{xiao2020audiovisual}   & AVSlowFast            & Kinetics-400              & 54.6          & 87.0         \\  
		AVTS~\citep{avts}                            & MC3-18                & Kinetics-400              & 56.9          & 85.8         \\  
		CPD~\citep{li2020learning}$^{\dagger *}$     & 3D-Resnet50           & Kinetics-400              & 57.7          & 88.7         \\  
		AVID~\citep{morgado2020avid}                 & R(2+1)D-18            & Kinetics-400              & \ul{60.8}     & 87.5         \\
		{\color{gray}CoCLR~\citep{Han2020SelfsupervisedCF}}         & {\color{gray}S3D}         & {\color{gray}Kinetics-400}         & {\color{gray}\bf{62.9}}          & {\color{gray}\bf{90.6}}  \\
		\midrule
		\bf{\methodname~(ours)}                      & R(2+1)D-18            & Kinetics-400              & {60.0}    & \ul{89.3}     \\
		 \midrule
		% OTHER DATASETS
		 \textit{Using other datasets} \\
		 L$^3$-Net~\citep{Arandjelovic17}        & VGG-16                & AudioSet                  & 40.2          & 72.3         \\    
		 Speech2Action*~\citep{nagrani2020}          & S3D-G                 & MovieDataset              & 58.1          & -            \\    
		 DynamoNet~\citep{Diba_2019}                 & ResNext101            & Youtube8M                 & 58.6          & 87.3         \\    
		     
		 MIL-NCE~\citep{miech2019endtoend}*          & S3D                   & HowTo100M                 & 61.0          & 91.3         \\    
		 AVTS~\citep{avts}                           & MC3-18                & AudioSet                  & 61.6          & 89.0         \\
		 XDC~\citep{alwassel2019self}                & R(2+1)D-18            & AudioSet                  & 63.7          & \bf{93.0}         \\
		 AVID~\citep{morgado2020avid}                & R(2+1)D-18            & AudioSet                  & 64.7          & 91.5         \\
		 {\color{gray}MMV$^*$~\citep{alayrac2020selfsupervised}}     & {\color{gray}R(2+1)D-18} & {\color{gray}Audioset}                 & {\color{gray}\bf{70.1}} & {\color{gray}91.5}  \\
		 ELo~\citep{piergiovanni2020evolving}        & R(2+1)D-50x3          & Youtube-2M                & 67.4          & 93.8         \\   
		 XDC~\citep{alwassel2019self}                & R(2+1)D-18            & IG65M                     & 68.9          & \bf{95.5}         \\   
         {\color{gray}MMV$^*$~\citep{alayrac2020selfsupervised}}     & {\color{gray}TSM-50x2}   & {\color{gray}AudioSet+HT100M}  & {\color{gray}\bf{75.0}} & {\color{gray}\ul{95.2}}\\
		 \midrule       
		 \bf{\methodname~(ours)}                     & R(2+1)D-18            & VGGSound (170K)           & 61.9          & 89.4         \\   
		 \bf{\methodname~(ours)}                     & R(2+1)D-18            & AudioSet (1.7M)           & \ul{66.1}     & \ul{92.5}    \\   
		 \bf{\methodname~(ours)}                     & R(2+1)D-18            & IG65M                     & \ul{72.8}     & \ul{95.2}    \\   
		 \midrule
		 {\bf{\methodname~(ours)}}  (only finetune \texttt{fc}) & R(2+1)D-18    & IG65M                  & {55.1}     & {85.4}    \\   
		 %\bf{\methodname~(ours)}                     & R(2+1)D-34            & IG65M                     & \bf{xx}       & \bf{xx}      \\   
		\bottomrule       
	\end{tabular}
	\vspace{2mm}
\end{table*}

% \begin{table}[!h]
%     \small
% 	\centering
% 	\caption{\textbf{State-of-the-art on action recognition.}
% 	Self-supervised and supervised methods on UCF101 and HMDB51 benchmarks.
% 	We follow the standard protocol and report the average top-1 accuracy over the official splits and show results for finetuning the whole network.
% 	Note that we find the supervised baseline to be around $6\%$ and $2\%$ better than reported in \citep{alwassel2019self} as we use a different finetuning strategy. 
% 	Methods with $^\dagger$ indicate the additional use of video titles as supervision.
% 	Methods with $^*$ use ASR generated text.
% 	Methods in {\color{gray} gray}  are concurrent works.
% 	\dontshowthisinappendix{See \cref{supp:tab:sota} in the Appendix for a full version of this table.}
% 	\labelswitch{tab:sota}}
% 	\vspace{-0.5em}
% 	\tabcolsep=0.09cm
% 	\begin{tabular}{l l l @{\hskip 0.2in} c c }
% 		\toprule
% 		%\multicolumn{3}{c|}{\underline{Pretraining}} & \multicolumn{4}{c}{\underline{Evaluation}} \\
% 		\textbf{Method}                              & \textbf{Architecture} & \bf{Pretrain Dataset}  & %\multicolumn{2}{c}{\underline{\textbf{ft. last}}}
% 		\multicolumn{2}{c}{\textbf{Top-1 Acc\%}} \\
% 		                                             &                       &                           & HMDB\,        & UCF          \\
% 		\midrule 
% 		Full supervision                             & R(2+1)D-18            & ImageNet                  & 46.7          & 82.8         \\ 
% 		Full supervision~\citep{alwassel2019self}    & R(2+1)D-18            & Kinetics-400              & 65.1          & 94.2         \\   
% 		Full supervision (ours)                      & R(2+1)D-18            & Kinetics-400              & 70.4          & 95.0         \\
		 
% 		Full supervision~\citep{tran2018closer}      & R(2+1)D-34            & Kinetics-400              & 74.5          & 96.8         \\   
% 		\midrule 
% 		\textit{Using UCF}  \\ 
% 		Shuffle and Learn~\citep{misra2016shuffle}   & CaffeNet              & UCF                       & 18.1          & 50.2         \\   
% 		VGAN~\citep{vondrick2016generating}          & VGAN                  & Flickr                    & --            & 52.1         \\   
% 		LT-Motion~\citep{Luo_2017}                   & VGG-16                & UCF                       & --            & 53.0         \\   
% 		Geometry~\citep{gan2018geometry}             & CaffeNet              & UCF                       & 23.3          & 55.1         \\   
% 		OPN~\citep{lee2017unsupervised}              & VGG                   & UCF                       & 23.8          & 56.3         \\   
% 		ST Order ~\citep{buchler2018improving}       & CaffeNet              & UCF                       & 25.0          & 58.6         \\   
% 		CMC~\citep{tian2019contrastive}              & CaffeNet              & UCF                       & 26.7          & 59.1         \\   
% 		VCP~\citep{luo2020video}                     & R(2+1)D-18            & UCF                       & 32.2          & 66.3         \\   
% 		Cross and Learn ~\citep{Sayed_2019}          & VGG-16                & UCF                       & 33.0          & 70.5         \\   
% 		\midrule
% 		\textit{Using Kinetics}  \\
% 		ClipOrder~\citep{clip_order}                 & R(2+1)D-18            & Kinetics-400              & 30.9          & 72.4         \\  
%         MotionPred~\citep{motion_statistics}         & C3D                   & Kinetics-400              & 33.4          & 61.2         \\    
% 		RotNet3D~\citep{jing2018self}                & 3D-ResNet18           & Kinetics-600              & 33.7          & 62.9         \\  
% 		ST-Puzzle~\citep{kim2019self}                & 3D-ResNet18           & Kinetics-400              & 33.7          & 65.8         \\  
% 		DPC~\citep{han2019video}                     & 3D-ResNet34           & Kinetics-400              & 35.7          & 75.7         \\  
% 		VPS~\citep{cho2020selfsupervised}            & R3D                   & Kinetics-400              & 36.8          & 74.8         \\  
% 		SpeedNet~\citep{benaim2020speednet}          & I3D                   & Kinetics-400              & 43.7          & 66.7         \\  
% 		AoT~\citep{wei2018learning}                  & T-CAM                 & Kinetics-400              & -             & 79.4         \\  
% 		CBT~\citep{sun2019contrastive}               & S3D                   & Kinetics-600              & 44.6          & 79.5         \\  
% 		Multisensory~\citep{owens2018audio}          & 3D-ResNet18           & Kinetics-400              & -             & 82.1         \\  
% 		XDC~\citep{alwassel2019self}                 & R(2+1)D-18            & Kinetics-400              & 52.6          & 86.8         \\  
% 		AV Sync+RotNet~\citep{xiao2020audiovisual}   & AVSlowFast            & Kinetics-400              & 54.6          & 87.0         \\  
% 		AVTS~\citep{avts}                            & MC3-18                & Kinetics-400              & 56.9          & 85.8         \\  
% 		CPD~\citep{li2020learning}$^{\dagger *}$     & 3D-Resnet50           & Kinetics-400              & 57.7          & 88.7         \\  
% 		AVID~\citep{morgado2020avid}                 & R(2+1)D-18            & Kinetics-400              & \ul{60.8}     & 87.5         \\
% 		{\color{gray}CoCLR}~\citep{Han2020SelfsupervisedCF}         & S3D         & Kinetics-400         & \bf{62.9}          & \bf{90.6}  \\
% 		\midrule
% 		\bf{\methodname~(ours)}                      & R(2+1)D-18            & Kinetics-400              & {60.0}    & \ul{89.3}     \\
% 		 \midrule
% 		% OTHER DATASETS
% 		 \textit{Using other datasets} \\
% 		 L$^3$-Net~\citep{Arandjelovic17}        & VGG-16                & AudioSet                  & 40.2          & 72.3         \\    
% 		 Speech2Action*~\citep{nagrani2020}          & S3D-G                 & MovieDataset              & 58.1          & -            \\    
% 		 DynamoNet~\citep{Diba_2019}                 & ResNext101            & Youtube8M                 & 58.6          & 87.3         \\    
		     
% 		 MIL-NCE~\citep{miech2019endtoend}*          & S3D                   & HowTo100M                 & 61.0          & 91.3         \\    
% 		 AVTS~\citep{avts}                           & MC3-18                & AudioSet                  & 61.6          & 89.0         \\
% 		 XDC~\citep{alwassel2019self}                & R(2+1)D-18            & AudioSet                  & 63.7          & 93.0         \\
% 		 AVID~\citep{morgado2020avid}                & R(2+1)D-18            & AudioSet                  & 64.7          & 91.5         \\
% 		 {\color{gray}MMV}~\citep{alayrac2020selfsupervised}     & R(2+1)D-18 & Audioset                 & \bf{70.1} & 91.5  \\
% 		 ELo~\citep{piergiovanni2020evolving}        & R(2+1)D-50x3          & Youtube-2M                & 67.4          & 93.8         \\   
% 		 XDC~\citep{alwassel2019self}                & R(2+1)D-18            & IG65M                     & 68.9          & \bf{95.5}         \\   
%          {\color{gray}MMV}~\citep{alayrac2020selfsupervised}     & TSM-50x2   & AudioSet+HT100M  & \bf{75.0} & \ul{95.2}\\
% 		 \midrule       
% 		 \bf{\methodname~(ours)}                     & R(2+1)D-18            & VGGSound (170K)           & 61.9          & 89.4         \\   
% 		 \bf{\methodname~(ours)}                     & R(2+1)D-18            & AudioSet (1.7M)           & \ul{66.1}     & {92.5}    \\   
% 		 \bf{\methodname~(ours)}                     & R(2+1)D-18            & IG65M                     & \ul{72.8}     & \ul{95.2}    \\   
% 		 \midrule
% 		 {\bf{\methodname~(ours)}}  (only finetune \texttt{fc}) & R(2+1)D-18    & IG65M                  & {55.1}     & {85.4}    \\   
% 		 %\bf{\methodname~(ours)}                     & R(2+1)D-34            & IG65M                     & \bf{xx}       & \bf{xx}      \\   
% 		\bottomrule       
% 	\end{tabular}
% 	\vspace{2mm}
% \end{table}


==> tabs/t1_abl_inv.tex <==
%------------------------------------------
\begin{wraptable}{r}{5.0cm} %\begin{table}
\vspace{-4.5mm}
\setlength{\tabcolsep}{3pt}
\centering
\footnotesize
\caption{Downstream action recognition results  for \textbf{different invariance ablations}.}\label{tab:ablation}
\vspace{-1mm}
\begin{tabular}{l c c c c @{\hskip 5pt} c c c c}
\toprule
 & \multicolumn{2}{c}{\textbf{HMDB}} & \multicolumn{2}{c}{\textbf{UCF}} \\
Epochs           & 50     & 100                & 50       & 100  \\
\midrule 
(a) Full          & \bf{55.1} & \bf{56.9}  & \bf{85.1} & \bf{87.9}  \\
\midrule 
(b) No $\tau$     & 32.8 & 34.8            & 74.0  & 76.2   \\
(c) No $g_v$      & 50.7 & 46.7            & 83.2  & 83.2  \\
(d) No $g_a$      & 51.5 & 55.6            & 84.8  & 86.5  \\
\bottomrule
\end{tabular}
\vspace{-18pt}
\end{wraptable} %\end{table}
%------------------------------------------

==> tabs/t6_vggsound.tex <==
\begin{wraptable}{r}{4.5cm}
%\vspace{-0.5em}
%\begin{table}[t]
%\centering
\footnotesize
\setlength{\tabcolsep}{1.4pt}
\captionof{table}{\textbf{VGG-Sound.}
\break 
Audio classification metrics after full-finetuning. \label{tab:vggsound}
}
% \vspace{-1mm}
\begin{tabular}{l l ccc}
\toprule
\textbf{Method}                 & mAP        & AUC        & d' \\
\midrule
Supervised                      &51.6          &96.8          &2.63 \\
\textbf{GDT} (ours)             &\bf{54.8}     &\bf{97.5}     &\bf{2.77} \\
\bottomrule
\end{tabular}
 \vspace{-34pt}
\end{wraptable}


